ECRM: Efficient Fault Tolerance for Recommendation Model Training via Erasure Coding

Deep-learning-based recommendation models (DLRMs) are widely deployed to serve personalized content to users. DLRMs are large in size due to their use of large embedding tables, and are trained by distributing the model across the memory of tens or hundreds of servers. Server failures are common in such large distributed systems and must be mitigated to enable training to progress. Checkpointing is the primary approach used for fault tolerance in these systems, but incurs significant training-time overhead both during normal operation and when recovering from failures. As these overheads increase with DLRM size, checkpointing is slated to become an even larger overhead for future DLRMs, which are expected to grow in size. This calls for rethinking fault tolerance in DLRM training. We present ECRM, a DLRM training system that achieves efficient fault tolerance using erasure coding. ECRM chooses which DLRM parameters to encode, correctly and efficiently updates parities, and enables training to proceed without any pauses, while maintaining consistency of the recovered parameters. We implement ECRM atop XDL, an open-source, industrial-scale DLRM training system. Compared to checkpointing, ECRM reduces training-time overhead for large DLRMs by up to 88%, recovers from failures up to 10.3$\times$ faster, and allows training to proceed during recovery. These results show the promise of erasure coding in imparting efficient fault tolerance to training current and future DLRMs.

==> figures/evaluation/data/normal/criteo-4x/progress.tex <==
\addplot [semithick, color0, mark=square*, mark size=1.5, mark options={solid,fill=white}, mark repeat=60,mark phase=0]
table {%
0 892928
0.333333333333333 9924608
0.666666666666667 18669568
1 27209728
1.33333333333333 35692544
1.66666666666667 44109824
2 52486144
2.33333333333333 60809216
2.66666666666667 69111808
3 77408256
3.33333333333333 85651456
3.66666666666667 93859840
4 102014976
4.33333333333333 110163968
4.66666666666667 118343680
5 126466048
5.33333333333333 134647808
5.66666666666667 142802944
6 150988800
6.33333333333333 159154176
6.66666666666667 167331840
7 175495168
7.33333333333333 183660544
7.66666666666667 191850496
8 200003584
8.33333333333333 208119808
8.66666666666667 216231936
9 224378880
9.33333333333333 232544256
9.66666666666667 240656384
10 248707072
10.3333333333333 256745472
10.6666666666667 264814592
11 272805888
11.3333333333333 280811520
11.6666666666667 288831488
12 296914944
12.3333333333333 304955392
12.6666666666667 312983552
13 321003520
13.3333333333333 329013248
13.6666666666667 336992256
14 344950784
14.3333333333333 352907264
14.6666666666667 360933376
15 368920576
15.3333333333333 376934400
15.6666666666667 384956416
16 393000960
16.3333333333333 401022976
16.6666666666667 409022464
17 416985088
17.3333333333333 424960000
17.6666666666667 432971776
18 440948736
18.3333333333333 448921600
18.6666666666667 456898560
19 464867328
19.3333333333333 472791040
19.6666666666667 480716800
20 488697856
20.3333333333333 496656384
20.6666666666667 504621056
21 512612352
21.3333333333333 520611840
21.6666666666667 528582656
22 536545280
22.3333333333333 544538624
22.6666666666667 552495104
23 560453632
23.3333333333333 568432640
23.6666666666667 576401408
24 584355840
24.3333333333333 592312320
24.6666666666667 600360960
25 608360448
25.3333333333333 616310784
25.6666666666667 624271360
26 632256512
26.3333333333333 640192512
26.6666666666667 648097792
27 656013312
27.3333333333333 663973888
27.6666666666667 671922176
28 679870464
28.3333333333333 687828992
28.6666666666667 695771136
29 703723520
29.3333333333333 711663616
29.6666666666667 719675392
30 727633920
30.3333333333333 735576064
30.6666666666667 743534592
31 751525888
31.3333333333333 759480320
31.6666666666667 767457280
32 775473152
32.3333333333333 783486976
32.6666666666667 791453696
33 799416320
33.3333333333333 807389184
33.6666666666667 815456256
34 823402496
34.3333333333333 831363072
34.6666666666667 839333888
35 847310848
35.3333333333333 855224320
35.6666666666667 863129600
36 871077888
36.3333333333333 879017984
36.6666666666667 886972416
37 894937088
37.3333333333333 902885376
37.6666666666667 910809088
38 918784000
38.3333333333333 926746624
38.6666666666667 934729728
39 942690304
39.3333333333333 950659072
39.6666666666667 958728192
40 966715392
40.3333333333333 974706688
40.6666666666667 982681600
41 990674944
41.3333333333333 998672384
41.6666666666667 1006628864
42 1014601728
42.3333333333333 1022595072
42.6666666666667 1030539264
43 1038454784
43.3333333333333 1046392832
43.6666666666667 1054369792
44 1062336512
44.3333333333333 1070327808
44.6666666666667 1078312960
45 1086308352
45.3333333333333 1094266880
45.6666666666667 1102239744
46 1110218752
46.3333333333333 1118191616
46.6666666666667 1126258688
47 1134204928
47.3333333333333 1142165504
47.6666666666667 1150136320
48 1158113280
48.3333333333333 1166026752
48.6666666666667 1173932032
49 1181880320
49.3333333333333 1189820416
49.6666666666667 1197774848
50 1205739520
50.3333333333333 1213687808
50.6666666666667 1221611520
51 1229586432
51.3333333333333 1237549056
51.6666666666667 1245532160
52 1253492736
52.3333333333333 1261461504
52.6666666666667 1269499904
53 1277444096
53.3333333333333 1285359616
53.6666666666667 1293297664
54 1301274624
54.3333333333333 1309241344
54.6666666666667 1317232640
55 1325217792
55.3333333333333 1333213184
55.6666666666667 1341171712
56 1349144576
56.3333333333333 1357123584
56.6666666666667 1365096448
57 1373163520
57.3333333333333 1381109760
57.6666666666667 1389070336
58 1397041152
58.3333333333333 1405018112
58.6666666666667 1412931584
59 1420836864
59.3333333333333 1428764672
59.6666666666667 1436809216
60 1444777984
60.3333333333333 1452701696
60.6666666666667 1460627456
61 1468608512
61.3333333333333 1476567040
61.6666666666667 1484531712
62 1492523008
62.3333333333333 1500522496
62.6666666666667 1508493312
63 1516455936
63.3333333333333 1524449280
63.6666666666667 1532405760
64 1540454400
64.3333333333333 1548453888
64.6666666666667 1556404224
65 1564364800
65.3333333333333 1572349952
65.6666666666667 1580285952
66 1588191232
66.3333333333333 1596119040
66.6666666666667 1604163584
67 1612132352
67.3333333333333 1620056064
67.6666666666667 1627981824
68 1635962880
68.3333333333333 1643921408
68.6666666666667 1651886080
69 1659877376
69.3333333333333 1667876864
69.6666666666667 1675847680
70 1683810304
70.3333333333333 1691803648
70.6666666666667 1699760128
71 1707808768
71.3333333333333 1715808256
71.6666666666667 1723758592
72 1731719168
72.3333333333333 1739704320
72.6666666666667 1747652608
73 1755623424
73.3333333333333 1763600384
73.6666666666667 1771513856
74 1779429376
74.3333333333333 1787398144
74.6666666666667 1795436544
75 1803380736
75.3333333333333 1811296256
75.6666666666667 1819234304
76 1827211264
76.3333333333333 1835177984
76.6666666666667 1843169280
77 1851154432
77.3333333333333 1859149824
77.6666666666667 1867108352
78 1875081216
78.3333333333333 1883060224
78.6666666666667 1891033088
79 1899100160
79.3333333333333 1907085312
79.6666666666667 1915080704
80 1923039232
80.3333333333333 1931012096
80.6666666666667 1938991104
81 1946963968
81.3333333333333 1955031040
81.6666666666667 1962977280
82 1970937856
82.3333333333333 1978908672
82.6666666666667 1986885632
83 1994799104
83.3333333333333 2002704384
83.6666666666667 2010632192
84 2018676736
84.3333333333333 2026645504
84.6666666666667 2034569216
85 2042494976
85.3333333333333 2050476032
85.6666666666667 2058434560
86 2066417664
86.3333333333333 2074365952
86.6666666666667 2082336768
87 2090313728
87.3333333333333 2098227200
87.6666666666667 2106142720
88 2114111488
88.3333333333333 2122149888
88.6666666666667 2130094080
89 2138009600
89.3333333333333 2145947648
89.6666666666667 2153924608
90 2161891328
90.3333333333333 2169882624
90.6666666666667 2177867776
91 2185863168
91.3333333333333 2193821696
91.6666666666667 2201794560
92 2209773568
92.3333333333333 2217746432
92.6666666666667 2225801216
93 2233759744
93.3333333333333 2241724416
93.6666666666667 2249715712
94 2257715200
94.3333333333333 2265686016
94.6666666666667 2273648640
95 2281641984
95.3333333333333 2289598464
95.6666666666667 2297647104
96 2305646592
96.3333333333333 2313646080
96.6666666666667 2321616896
97 2329579520
97.3333333333333 2337572864
97.6666666666667 2345529344
98 2353577984
98.3333333333333 2361577472
98.6666666666667 2369527808
99 2377488384
99.3333333333333 2385455104
99.6666666666667 2393397248
100 2401441792
100.333333333333 2409410560
100.666666666667 2417334272
101 2425260032
101.333333333333 2433241088
101.666666666667 2441199616
102 2449164288
102.333333333333 2457155584
102.666666666667 2465155072
103 2473125888
103.333333333333 2481088512
103.666666666667 2489081856
104 2497038336
104.333333333333 2505086976
104.666666666667 2513086464
105 2521036800
105.333333333333 2528997376
105.666666666667 2536982528
106 2544922624
106.333333333333 2552860672
106.666666666667 2560837632
107 2568804352
107.333333333333 2576795648
107.666666666667 2584780800
108 2592776192
108.333333333333 2600734720
108.666666666667 2608707584
109 2616686592
109.333333333333 2624659456
109.666666666667 2632726528
110 2640672768
110.333333333333 2648633344
110.666666666667 2656604160
111 2664581120
111.333333333333 2672494592
111.666666666667 2680410112
112 2688378880
112.333333333333 2696417280
112.666666666667 2704386048
113 2712344576
113.333333333333 2720317440
113.666666666667 2728296448
114 2736269312
114.333333333333 2744336384
114.666666666667 2752321536
115 2760316928
115.333333333333 2768275456
115.666666666667 2776248320
116 2784227328
116.333333333333 2792200192
116.666666666667 2800267264
117 2808213504
117.333333333333 2816174080
117.666666666667 2824144896
118 2832121856
118.333333333333 2840035328
118.666666666667 2847940608
119 2855868416
119.333333333333 2863855616
119.666666666667 2871832576
120 2879758336
120.333333333333 2887739392
120.666666666667 2895697920
121 2903662592
121.333333333333 2911653888
121.666666666667 2919653376
122 2927624192
122.333333333333 2935586816
122.666666666667 2943580160
123 2951536640
123.333333333333 2959585280
123.666666666667 2967584768
124 2975535104
124.333333333333 2983495680
124.666666666667 2991480832
125 2999416832
125.333333333333 3007322112
125.666666666667 3015249920
126 3023269888
126.333333333333 3031216128
126.666666666667 3039176704
127 3047147520
127.333333333333 3055124480
127.666666666667 3063037952
128 3070953472
128.333333333333 3078922240
128.666666666667 3086960640
129 3094904832
129.333333333333 3102820352
129.666666666667 3110758400
130 3118735360
130.333333333333 3126702080
130.666666666667 3134693376
131 3142678528
131.333333333333 3150673920
131.666666666667 3158632448
132 3166605312
132.333333333333 3174584320
132.666666666667 3182520320
133 3190425600
133.333333333333 3198341120
133.666666666667 3206309888
134 3214348288
134.333333333333 3222292480
134.666666666667 3230208000
135 3238146048
135.333333333333 3246123008
135.666666666667 3254089728
136 3262081024
136.333333333333 3270066176
136.666666666667 3278061568
137 3286020096
137.333333333333 3293992960
137.666666666667 3301971968
138 3309944832
138.333333333333 3318011904
138.666666666667 3325958144
139 3333918720
139.333333333333 3341957120
139.666666666667 3349956608
140 3357906944
140.333333333333 3365867520
140.666666666667 3373852672
141 3381788672
141.333333333333 3389693952
141.666666666667 3397609472
142 3405570048
142.333333333333 3413518336
142.666666666667 3421466624
143 3429425152
143.333333333333 3437367296
143.666666666667 3445319680
144 3453259776
144.333333333333 3461271552
144.666666666667 3469230080
145 3477172224
145.333333333333 3485130752
145.666666666667 3493122048
146 3501101056
146.333333333333 3509059584
146.666666666667 3517032448
147 3525011456
147.333333333333 3532984320
147.666666666667 3541051392
148 3549036544
148.333333333333 3557031936
148.666666666667 3564990464
149 3572963328
149.333333333333 3580942336
149.666666666667 3588915200
150 3596982272
150.333333333333 3604928512
150.666666666667 3612889088
151 3620859904
151.333333333333 3628836864
151.666666666667 3636750336
152 3644655616
152.333333333333 3652583424
152.666666666667 3660568576
153 3668559872
153.333333333333 3676545024
153.666666666667 3684540416
154 3692498944
154.333333333333 3700471808
154.666666666667 3708450816
155 3716423680
155.333333333333 3724490752
155.666666666667 3732475904
156 3740471296
156.333333333333 3748429824
156.666666666667 3756402688
157 3764381696
157.333333333333 3772354560
157.666666666667 3780421632
158 3788367872
158.333333333333 3796328448
158.666666666667 3804299264
159 3812276224
159.333333333333 3820212224
159.666666666667 3828160512
160 3836108800
160.333333333333 3844067328
160.666666666667 3852009472
161 3859961856
161.333333333333 3867901952
161.666666666667 3875913728
162 3883872256
162.333333333333 3891814400
162.666666666667 3899772928
163 3907764224
163.333333333333 3915718656
163.666666666667 3923695616
164 3931711488
164.333333333333 3939725312
164.666666666667 3947692032
165 3955654656
165.333333333333 3963627520
165.666666666667 3971694592
166 3979649024
166.333333333333 3987572736
166.666666666667 3995498496
167 4003479552
167.333333333333 4011438080
167.666666666667 4019421184
168 4027369472
168.333333333333 4035340288
168.666666666667 4043317248
169 4051230720
169.333333333333 4059146240
169.666666666667 4067115008
170 4075153408
170.333333333333 4083097600
170.666666666667 4091013120
171 4098951168
171.333333333333 4106928128
171.666666666667 4114894848
172 4122886144
172.333333333333 4130871296
172.666666666667 4138870784
173 4146866176
173.333333333333 4154824704
173.666666666667 4162797568
174 4170776576
174.333333333333 4178749440
174.666666666667 4186816512
175 4194801664
175.333333333333 4202797056
175.666666666667 4210755584
176 4218728448
176.333333333333 4226707456
176.666666666667 4234680320
177 4242747392
177.333333333333 4250693632
177.666666666667 4258654208
178 4266625024
178.333333333333 4274601984
178.666666666667 4282515456
179 4290420736
179.333333333333 4298381312
179.666666666667 4306325504
180 4314241024
180.333333333333 4322179072
180.666666666667 4330156032
181 4338122752
181.333333333333 4346114048
181.666666666667 4354099200
182 4362094592
182.333333333333 4370053120
182.666666666667 4378025984
183 4386004992
183.333333333333 4393977856
183.666666666667 4402032640
184 4409991168
184.333333333333 4417955840
184.666666666667 4425947136
185 4433946624
185.333333333333 4441917440
185.666666666667 4449880064
186 4457916416
186.333333333333 4465885184
186.666666666667 4473808896
187 4481734656
187.333333333333 4489715712
187.666666666667 4497674240
188 4505638912
188.333333333333 4513630208
188.666666666667 4521629696
189 4529600512
189.333333333333 4537563136
189.666666666667 4545556480
190 4553512960
190.333333333333 4561561600
190.666666666667 4569538560
191 4577505280
191.333333333333 4585496576
191.666666666667 4593481728
192 4601477120
192.333333333333 4609435648
192.666666666667 4617396224
193 4625395712
193.333333333333 4633366528
193.666666666667 4641329152
194 4649322496
194.333333333333 4657278976
194.666666666667 4665327616
195 4673327104
195.333333333333 4681277440
195.666666666667 4689238016
196 4697223168
196.333333333333 4705159168
196.666666666667 4713099264
197 4721053696
197.333333333333 4729018368
197.666666666667 4736966656
198 4744890368
198.333333333333 4752865280
198.666666666667 4760827904
199 4768811008
199.333333333333 4776790016
199.666666666667 4784769024
200 4792741888
200.333333333333 4800808960
200.666666666667 4808794112
201 4816789504
201.333333333333 4824748032
201.666666666667 4832720896
202 4840699904
202.333333333333 4848672768
202.666666666667 4856739840
203 4864686080
203.333333333333 4872646656
203.666666666667 4880617472
204 4888594432
204.333333333333 4896507904
204.666666666667 4904413184
205 4912373760
205.333333333333 4920317952
205.666666666667 4928233472
206 4936177664
206.333333333333 4944177152
206.666666666667 4952147968
207 4960110592
207.333333333333 4968103936
207.666666666667 4976060416
208 4984109056
208.333333333333 4992108544
208.666666666667 5000058880
209 5008019456
209.333333333333 5016004608
209.666666666667 5023940608
210 5031845888
210.333333333333 5039761408
210.666666666667 5047730176
211 5055653888
211.333333333333 5063579648
211.666666666667 5071560704
212 5079519232
212.333333333333 5087483904
212.666666666667 5095489536
213 5103448064
213.333333333333 5111420928
213.666666666667 5119399936
214 5127372800
214.333333333333 5135439872
214.666666666667 5143425024
215 5151420416
215.333333333333 5159378944
215.666666666667 5167351808
216 5175330816
216.333333333333 5183303680
216.666666666667 5191370752
217 5199316992
217.333333333333 5207277568
217.666666666667 5215248384
218 5223225344
218.333333333333 5231138816
218.666666666667 5239044096
219 5247004672
219.333333333333 5254977536
219.666666666667 5262913536
220 5270853632
220.333333333333 5278808064
220.666666666667 5286772736
221 5294721024
221.333333333333 5302644736
221.666666666667 5310619648
222 5318582272
222.333333333333 5326565376
222.666666666667 5334525952
223 5342461952
223.333333333333 5350455296
223.666666666667 5358422016
224 5366386688
224.333333333333 5374365696
224.666666666667 5382404096
225 5390395392
225.333333333333 5398349824
225.666666666667 5406306304
226 5414287360
226.333333333333 5422264320
226.666666666667 5430177792
227 5438083072
227.333333333333 5446043648
227.666666666667 5453987840
228 5461903360
228.333333333333 5469841408
228.666666666667 5477818368
229 5485785088
229.333333333333 5493776384
229.666666666667 5501761536
230 5509756928
230.333333333333 5517715456
230.666666666667 5525688320
231 5533667328
231.333333333333 5541640192
231.666666666667 5549694976
232 5557653504
232.333333333333 5565618176
232.666666666667 5573599232
233 5581561856
233.333333333333 5589555200
233.666666666667 5597511680
234 5605560320
234.333333333333 5613559808
234.666666666667 5621510144
235 5629470720
235.333333333333 5637455872
235.666666666667 5645391872
236 5653297152
236.333333333333 5661224960
236.666666666667 5669269504
237 5677238272
237.333333333333 5685161984
237.666666666667 5693087744
238 5701068800
238.333333333333 5709027328
238.666666666667 5716992000
239 5724983296
239.333333333333 5732966400
239.666666666667 5740939264
240 5748932608
240.333333333333 5756876800
240.666666666667 5764792320
241 5772730368
241.333333333333 5780707328
241.666666666667 5788674048
242 5796665344
242.333333333333 5804650496
242.666666666667 5812645888
243 5820604416
243.333333333333 5828577280
243.666666666667 5836548096
244 5844514816
244.333333333333 5852485632
244.666666666667 5860462592
245 5868410880
245.333333333333 5876373504
245.666666666667 5884346368
246 5892378624
246.333333333333 5900369920
246.666666666667 5908355072
247 5916350464
247.333333333333 5924308992
247.666666666667 5932281856
248 5940260864
248.333333333333 5948233728
248.666666666667 5956300800
249 5964247040
249.333333333333 5972207616
249.666666666667 5980178432
250 5988155392
250.333333333333 5996068864
250.666666666667 6003984384
251 6011953152
251.333333333333 6019952640
251.666666666667 6027902976
252 6035863552
252.333333333333 6043848704
252.666666666667 6051801088
253 6059724800
253.333333333333 6067699712
253.666666666667 6075662336
254 6083645440
254.333333333333 6091624448
254.666666666667 6099603456
255 6107576320
255.333333333333 6115643392
255.666666666667 6123628544
256 6131623936
256.333333333333 6139582464
256.666666666667 6147555328
257 6155534336
257.333333333333 6163507200
257.666666666667 6171574272
258 6179520512
258.333333333333 6187481088
258.666666666667 6195451904
259 6203428864
259.333333333333 6211377152
259.666666666667 6219337728
260 6227322880
260.333333333333 6235258880
260.666666666667 6243164160
261 6251079680
261.333333333333 6259040256
261.666666666667 6266988544
262 6274936832
262.333333333333 6282895360
262.666666666667 6290837504
263 6298789888
263.333333333333 6306729984
263.666666666667 6314741760
264 6322700288
264.333333333333 6330642432
264.666666666667 6338686976
265 6346655744
265.333333333333 6354579456
265.666666666667 6362505216
266 6370463744
266.333333333333 6378436608
266.666666666667 6386429952
267 6394374144
267.333333333333 6402289664
267.666666666667 6410227712
268 6418204672
268.333333333333 6426171392
268.666666666667 6434162688
269 6442147840
269.333333333333 6450143232
269.666666666667 6458101760
270 6466074624
270.333333333333 6474053632
270.666666666667 6482026496
271 6490093568
271.333333333333 6498039808
271.666666666667 6506000384
272 6513971200
272.333333333333 6521948160
272.666666666667 6529861632
273 6537777152
273.333333333333 6545745920
273.666666666667 6553669632
274 6561595392
274.333333333333 6569580544
274.666666666667 6577575936
275 6585534464
275.333333333333 6593507328
275.666666666667 6601486336
276 6609459200
276.333333333333 6617526272
276.666666666667 6625472512
277 6633433088
277.333333333333 6641403904
277.666666666667 6649380864
278 6657294336
278.333333333333 6665199616
278.666666666667 6673160192
279 6681104384
279.333333333333 6689032192
279.666666666667 6697025536
280 6704982016
280.333333333333 6713030656
280.666666666667 6721030144
281 6729029632
281.333333333333 6737000448
281.666666666667 6744963072
282 6752956416
282.333333333333 6760912896
282.666666666667 6768961536
283 6776961024
283.333333333333 6784911360
283.666666666667 6792871936
284 6800857088
284.333333333333 6808793088
284.666666666667 6816698368
285 6824613888
285.333333333333 6832582656
285.666666666667 6840506368
286 6844471296
};
\addlegendentry{\noFT}
\addplot [semithick, color2, mark=triangle*, mark size=2.0, mark options={solid,fill=white}, mark repeat=60,mark phase=45]
table {%
0 0
0.333333333333333 0
0.666666666666667 0
1 0
1.33333333333333 8009728
1.66666666666667 16058368
2 24004608
2.33333333333333 31950848
2.66666666666667 39870464
3 47763456
3.33333333333333 55613440
3.66666666666667 63440896
4 71278592
4.33333333333333 79122432
4.66666666666667 86974464
5 94826496
5.33333333333333 102651904
5.66666666666667 110393344
6 118145024
6.33333333333333 125896704
6.66666666666667 133695488
7 141457408
7.33333333333333 149219328
7.66666666666667 157005824
8 164812800
8.33333333333333 172619776
8.66666666666667 180385792
9 188151808
9.33333333333333 195911680
9.66666666666667 203618304
10 211314688
10.3333333333333 219031552
10.6666666666667 226820096
11 234479616
11.3333333333333 242194432
11.6666666666667 249907200
12 257634304
12.3333333333333 265318400
12.6666666666667 273063936
13 280819712
13.3333333333333 288550912
13.6666666666667 296218624
14 303867904
14.3333333333333 311554048
14.6666666666667 319211520
15 326885376
15.3333333333333 334600192
15.6666666666667 342321152
16 349984768
16.3333333333333 357609472
16.6666666666667 365297664
17 372940800
17.3333333333333 380735488
17.6666666666667 388392960
18 396056576
18.3333333333333 403666944
18.6666666666667 411308032
19 418961408
19.3333333333333 426655744
19.6666666666667 434358272
20 442064896
20.3333333333333 449794048
20.6666666666667 457541632
21 465211392
21.3333333333333 472936448
21.6666666666667 480591872
22 488265728
22.3333333333333 495933440
22.6666666666667 503529472
23 511150080
23.3333333333333 518768640
23.6666666666667 526446592
24 534106112
24.3333333333333 541831168
24.6666666666667 549525504
25 557236224
25.3333333333333 564908032
25.6666666666667 572571648
26 580237312
26.3333333333333 587884544
26.6666666666667 595437568
27 603047936
27.3333333333333 610658304
27.6666666666667 618311680
28 626001920
28.3333333333333 633640960
28.6666666666667 641245184
29 648869888
29.3333333333333 656506880
29.6666666666667 664143872
30 671817728
30.3333333333333 679481344
30.6666666666667 687126528
31 694835200
31.3333333333333 702504960
31.6666666666667 710115328
32 717746176
32.3333333333333 725407744
32.6666666666667 733061120
33 740792320
33.3333333333333 748511232
33.6666666666667 756215808
34 763887616
34.3333333333333 771561472
34.6666666666667 779235328
35 786880512
35.3333333333333 794458112
35.6666666666667 802056192
36 809674752
36.3333333333333 817321984
36.6666666666667 824991744
37 832616448
37.3333333333333 840216576
37.6666666666667 847851520
38 855465984
38.3333333333333 863096832
38.6666666666667 870774784
39 878487552
39.3333333333333 886190080
39.6666666666667 893902848
40 901662720
40.3333333333333 909332480
40.6666666666667 917057536
41 924706816
41.3333333333333 932376576
41.6666666666667 940048384
42 947648512
42.3333333333333 955283456
42.6666666666667 962902016
43 970592256
43.3333333333333 978251776
43.6666666666667 985958400
44 993671168
44.3333333333333 1001371648
44.6666666666667 1009047552
45 1016723456
45.3333333333333 1024393216
45.6666666666667 1032015872
46 1039665152
46.3333333333333 1047326720
46.6666666666667 1055027200
47 1062729728
47.3333333333333 1070442496
47.6666666666667 1078157312
48 1085911040
48.3333333333333 1093582848
48.6666666666667 1101316096
49 1108961280
49.3333333333333 1116639232
49.6666666666667 1124302848
50 1131907072
50.3333333333333 1139554304
50.6666666666667 1147174912
51 1154852864
51.3333333333333 1162500096
51.6666666666667 1170206720
52 1177884672
52.3333333333333 1185529856
52.6666666666667 1193240576
53 1200936960
53.3333333333333 1208676352
53.6666666666667 1216352256
54 1224011776
54.3333333333333 1231661056
54.6666666666667 1239310336
55 1246922752
55.3333333333333 1254481920
55.6666666666667 1262067712
56 1269723136
56.3333333333333 1277368320
56.6666666666667 1285042176
57 1292638208
57.3333333333333 1300271104
57.6666666666667 1307871232
58 1315538944
58.3333333333333 1323177984
58.6666666666667 1330849792
59 1338435584
59.3333333333333 1346091008
59.6666666666667 1353691136
60 1361338368
60.3333333333333 1369001984
60.6666666666667 1376669696
61 1384302592
61.3333333333333 1391972352
61.6666666666667 1399687168
62 1407309824
62.3333333333333 1414912000
62.6666666666667 1422594048
63 1430224896
63.3333333333333 1437935616
63.6666666666667 1445627904
64 1453357056
64.3333333333333 1461028864
64.6666666666667 1468700672
65 1476370432
65.3333333333333 1484122112
65.6666666666667 1491800064
66 1499551744
66.3333333333333 1507207168
66.6666666666667 1514876928
67 1522542592
67.3333333333333 1530146816
67.6666666666667 1537777664
68 1545385984
68.3333333333333 1553057792
68.6666666666667 1560709120
69 1568444416
69.3333333333333 1576146944
69.6666666666667 1583841280
70 1591515136
70.3333333333333 1599199232
70.6666666666667 1606871040
71 1614491648
71.3333333333333 1622145024
71.6666666666667 1629771776
72 1637478400
72.3333333333333 1645182976
72.6666666666667 1652922368
73 1660628992
73.3333333333333 1668302848
73.6666666666667 1675984896
74 1683630080
74.3333333333333 1691308032
74.6666666666667 1698938880
75 1706571776
75.3333333333333 1714214912
75.6666666666667 1721890816
76 1729527808
76.3333333333333 1737236480
76.6666666666667 1744920576
77 1752649728
77.3333333333333 1760319488
77.6666666666667 1767985152
78 1775636480
78.3333333333333 1783267328
78.6666666666667 1790922752
79 1798574080
79.3333333333333 1806190592
79.6666666666667 1813827584
80 1821462528
80.3333333333333 1829146624
80.6666666666667 1836847104
81 1844563968
81.3333333333333 1852286976
81.6666666666667 1860032512
82 1867710464
82.3333333333333 1875431424
82.6666666666667 1883092992
83 1890768896
83.3333333333333 1898424320
83.6666666666667 1906051072
84 1913688064
84.3333333333333 1921312768
84.6666666666667 1928998912
85 1936635904
85.3333333333333 1944293376
85.6666666666667 1951997952
86 1959706624
86.3333333333333 1967409152
86.6666666666667 1975083008
87 1982756864
87.3333333333333 1990420480
87.6666666666667 1998049280
88 2005692416
88.3333333333333 2013329408
88.6666666666667 2021029888
89 2028750848
89.3333333333333 2036490240
89.6666666666667 2044200960
90 2051878912
90.3333333333333 2059556864
90.6666666666667 2067222528
91 2074904576
91.3333333333333 2082506752
91.6666666666667 2090137600
92 2097702912
92.3333333333333 2105303040
92.6666666666667 2112954368
93 2120603648
93.3333333333333 2128273408
93.6666666666667 2135853056
94 2143479808
94.3333333333333 2151090176
94.6666666666667 2158739456
95 2166382592
95.3333333333333 2174085120
95.6666666666667 2181726208
96 2189402112
96.3333333333333 2197112832
96.6666666666667 2204762112
97 2212368384
97.3333333333333 2220046336
97.6666666666667 2227668992
98 2235385856
98.3333333333333 2243080192
98.6666666666667 2250735616
99 2258386944
99.3333333333333 2266071040
99.6666666666667 2273710080
100 2281367552
100.333333333333 2289078272
100.666666666667 2296711168
101 2304301056
101.333333333333 2311983104
101.666666666667 2319599616
102 2327318528
102.333333333333 2335004672
102.666666666667 2342715392
103 2350387200
103.333333333333 2358042624
103.666666666667 2365693952
104 2373349376
104.333333333333 2380965888
104.666666666667 2388545536
105 2396160000
105.333333333333 2403837952
105.666666666667 2411489280
106 2419204096
106.333333333333 2426873856
106.666666666667 2434506752
107 2442217472
107.333333333333 2449917952
107.666666666667 2457657344
108 2465337344
108.333333333333 2473005056
108.666666666667 2480660480
109 2488299520
109.333333333333 2495926272
109.666666666667 2503497728
110 2511099904
110.333333333333 2518761472
110.666666666667 2526398464
111 2534072320
111.333333333333 2541662208
111.666666666667 2549307392
112 2556993536
112.333333333333 2564618240
112.666666666667 2572316672
113 2579996672
113.333333333333 2587684864
113.666666666667 2595346432
114 2603075584
114.333333333333 2610776064
114.666666666667 2618480640
115 2626162688
115.333333333333 2633832448
115.666666666667 2641485824
116 2649116672
116.333333333333 2656679936
116.666666666667 2664282112
117 2671872000
117.333333333333 2679517184
117.666666666667 2687166464
118 2694795264
118.333333333333 2702397440
118.666666666667 2710052864
119 2717759488
119.333333333333 2725462016
119.666666666667 2733205504
120 2740881408
120.333333333333 2748547072
120.666666666667 2756208640
121 2763853824
121.333333333333 2771515392
121.666666666667 2779160576
122 2786768896
122.333333333333 2794407936
122.666666666667 2802055168
123 2809747456
123.333333333333 2817445888
123.666666666667 2825166848
124 2832898048
124.333333333333 2840641536
124.666666666667 2848309248
125 2856042496
125.333333333333 2863714304
125.666666666667 2871326720
126 2878976000
126.333333333333 2886617088
126.666666666667 2894354432
127 2902067200
127.333333333333 2909806592
127.666666666667 2917515264
128 2925193216
128.333333333333 2932883456
128.666666666667 2940536832
129 2948218880
129.333333333333 2955831296
129.666666666667 2963433472
130 2970994688
130.333333333333 2978588672
130.666666666667 2986258432
131 2993899520
131.333333333333 3001563136
131.666666666667 3009175552
132 3016890368
132.333333333333 3024580608
132.666666666667 3032270848
133 3039934464
133.333333333333 3047616512
133.666666666667 3055239168
134 3062845440
134.333333333333 3070461952
134.666666666667 3078144000
135 3085776896
135.333333333333 3093485568
135.666666666667 3101175808
136 3108907008
136.333333333333 3116593152
136.666666666667 3124248576
137 3131914240
137.333333333333 3139559424
137.666666666667 3147218944
138 3154872320
138.333333333333 3162492928
138.666666666667 3170105344
139 3177764864
139.333333333333 3185418240
139.666666666667 3193051136
140 3200706560
140.333333333333 3208378368
140.666666666667 3216107520
141 3223775232
141.333333333333 3231451136
141.666666666667 3239129088
142 3246735360
142.333333333333 3254372352
142.666666666667 3262001152
143 3269685248
143.333333333333 3277340672
143.666666666667 3285067776
144 3292778496
144.333333333333 3300483072
144.666666666667 3308140544
145 3315810304
145.333333333333 3323455488
145.666666666667 3331117056
146 3338846208
146.333333333333 3346544640
146.666666666667 3354241024
147 3361921024
147.333333333333 3369582592
147.666666666667 3377246208
148 3384891392
148.333333333333 3392546816
148.666666666667 3400204288
149 3407841280
149.333333333333 3415461888
149.666666666667 3423137792
150 3430828032
150.333333333333 3438557184
150.666666666667 3446272000
151 3454007296
151.333333333333 3461711872
151.666666666667 3469361152
152 3477059584
152.333333333333 3484663808
152.666666666667 3492259840
153 3499872256
153.333333333333 3507546112
153.666666666667 3515187200
154 3522885632
154.333333333333 3530569728
154.666666666667 3538253824
155 3545907200
155.333333333333 3553617920
155.666666666667 3561330688
156 3569018880
156.333333333333 3576694784
156.666666666667 3584368640
157 3592032256
157.333333333333 3599673344
157.666666666667 3607228416
158 3614826496
158.333333333333 3622443008
158.666666666667 3630102528
159 3637764096
159.333333333333 3645421568
159.666666666667 3653079040
160 3660738560
160.333333333333 3668340736
160.666666666667 3675940864
161 3683596288
161.333333333333 3691270144
161.666666666667 3698892800
162 3706540032
162.333333333333 3714217984
162.666666666667 3721951232
163 3729608704
163.333333333333 3737278464
163.666666666667 3744942080
164 3752529920
164.333333333333 3760160768
164.666666666667 3767783424
165 3775451136
165.333333333333 3783163904
165.666666666667 3790874624
166 3798605824
166.333333333333 3806310400
166.666666666667 3813996544
167 3821676544
167.333333333333 3829280768
167.666666666667 3836891136
168 3844530176
168.333333333333 3852218368
168.666666666667 3859853312
169 3867561984
169.333333333333 3875237888
169.666666666667 3882926080
170 3890569216
170.333333333333 3898284032
170.666666666667 3905986560
171 3913689088
171.333333333333 3921358848
171.666666666667 3929012224
172 3936624640
172.333333333333 3944237056
172.666666666667 3951863808
173 3959537664
173.333333333333 3967184896
173.666666666667 3974885376
174 3982587904
174.333333333333 3990321152
174.666666666667 3997997056
175 4005648384
175.333333333333 4013314048
175.666666666667 4020975616
176 4028596224
176.333333333333 4036214784
176.666666666667 4043880448
177 4051591168
177.333333333333 4059320320
177.666666666667 4067047424
178 4074776576
178.333333333333 4082491392
178.666666666667 4090071040
179 4097734656
179.333333333333 4105381888
179.666666666667 4113031168
180 4120635392
180.333333333333 4128354304
180.666666666667 4136028160
181 4143718400
181.333333333333 4151379968
181.666666666667 4159064064
182 4166672384
182.333333333333 4174274560
182.666666666667 4181907456
183 4189575168
183.333333333333 4197251072
183.666666666667 4204951552
184 4212662272
184.333333333333 4220403712
184.666666666667 4228075520
185 4235767808
185.333333333333 4243445760
185.666666666667 4251156480
186 4258830336
186.333333333333 4266500096
186.666666666667 4274167808
187 4281817088
187.333333333333 4289433600
187.666666666667 4296986624
188 4304584704
188.333333333333 4312246272
188.666666666667 4319885312
189 4327550976
189.333333333333 4335124480
189.666666666667 4342749184
190 4350349312
190.333333333333 4358023168
190.666666666667 4365672448
191 4373350400
191.333333333333 4380942336
191.666666666667 4388577280
192 4396335104
192.333333333333 4404037632
192.666666666667 4411748352
193 4419465216
193.333333333333 4427247616
193.666666666667 4434903040
194 4442609664
194.333333333333 4450330624
194.666666666667 4458070016
195 4465737728
195.333333333333 4473479168
195.666666666667 4481224704
196 4488960000
196.333333333333 4496629760
196.666666666667 4504260608
197 4511950848
197.333333333333 4519596032
197.666666666667 4527269888
198 4534984704
198.333333333333 4542703616
198.666666666667 4550418432
199 4558096384
199.333333333333 4565768192
199.666666666667 4573429760
200 4581064704
200.333333333333 4588617728
200.666666666667 4596232192
201 4603848704
201.333333333333 4611504128
201.666666666667 4619153408
202 4626784256
202.333333333333 4634386432
202.666666666667 4642033664
203 4649668608
203.333333333333 4657293312
203.666666666667 4664958976
204 4672598016
204.333333333333 4680212480
204.666666666667 4687912960
205 4695644160
205.333333333333 4703375360
205.666666666667 4711059456
206 4718714880
206.333333333333 4726388736
206.666666666667 4734038016
207 4741654528
207.333333333333 4749221888
207.666666666667 4756824064
208 4764483584
208.333333333333 4772110336
208.666666666667 4779776000
209 4787343360
209.333333333333 4794978304
209.666666666667 4802670592
210 4810303488
210.333333333333 4818014208
210.666666666667 4825702400
211 4833398784
211.333333333333 4841056256
211.666666666667 4848779264
212 4856434688
212.333333333333 4864098304
212.666666666667 4871759872
213 4879360000
213.333333333333 4886925312
213.666666666667 4894527488
214 4902125568
214.333333333333 4909780992
214.666666666667 4917444608
215 4925083648
215.333333333333 4932722688
215.666666666667 4940402688
216 4948135936
216.333333333333 4955793408
216.666666666667 4963465216
217 4971141120
217.333333333333 4978733056
217.666666666667 4986365952
218 4993986560
218.333333333333 5001662464
218.666666666667 5009315840
219 5016983552
219.333333333333 5024563200
219.666666666667 5032206336
220 5039810560
220.333333333333 5047463936
220.666666666667 5055123456
221 5062805504
221.333333333333 5070389248
221.666666666667 5078018048
222 5085769728
222.333333333333 5093484544
222.666666666667 5101185024
223 5108871168
223.333333333333 5116534784
223.666666666667 5124182016
224 5131814912
224.333333333333 5139392512
224.666666666667 5147002880
225 5154619392
225.333333333333 5162242048
225.666666666667 5169895424
226 5177540608
226.333333333333 5185265664
226.666666666667 5192998912
227 5200734208
227.333333333333 5208455168
227.666666666667 5216141312
228 5223845888
228.333333333333 5231523840
228.666666666667 5239201792
229 5246812160
229.333333333333 5254424576
229.666666666667 5261991936
230 5269602304
230.333333333333 5277274112
230.666666666667 5284909056
231 5292599296
231.333333333333 5300199424
231.666666666667 5307852800
232 5315522560
232.333333333333 5323212800
232.666666666667 5330874368
233 5338535936
233.333333333333 5346156544
233.666666666667 5353766912
234 5361377280
234.333333333333 5369055232
234.666666666667 5376733184
235 5384450048
235.333333333333 5392173056
235.666666666667 5399934976
236 5407600640
236.333333333333 5415290880
236.666666666667 5422954496
237 5430552576
237.333333333333 5438175232
237.666666666667 5445785600
238 5453459456
238.333333333333 5461114880
238.666666666667 5468717056
239 5476384768
239.333333333333 5484062720
239.666666666667 5491699712
240 5499310080
240.333333333333 5506959360
240.666666666667 5514661888
241 5522356224
241.333333333333 5530097664
241.666666666667 5537785856
242 5545453568
242.333333333333 5553108992
242.666666666667 5560758272
243 5568407552
243.333333333333 5576083456
243.666666666667 5583702016
244 5591361536
244.333333333333 5599000576
244.666666666667 5606690816
245 5614391296
245.333333333333 5622083584
245.666666666667 5629739008
246 5637330944
246.333333333333 5644967936
246.666666666667 5652598784
247 5660289024
247.333333333333 5667942400
247.666666666667 5675550720
248 5683224576
248.333333333333 5690894336
248.666666666667 5698504704
249 5706108928
249.333333333333 5713737728
249.666666666667 5721448448
250 5729157120
250.333333333333 5736884224
250.666666666667 5744560128
251 5752227840
251.333333333333 5759901696
251.666666666667 5767548928
252 5775163392
252.333333333333 5782781952
252.666666666667 5790418944
253 5798094848
253.333333333333 5805729792
253.666666666667 5813442560
254 5821130752
254.333333333333 5828857856
254.666666666667 5836544000
255 5844215808
255.333333333333 5851881472
255.666666666667 5859516416
256 5867239424
256.333333333333 5874933760
256.666666666667 5882671104
257 5890349056
257.333333333333 5898012672
257.666666666667 5905678336
258 5913315328
258.333333333333 5920968704
258.666666666667 5928613888
259 5936236544
259.333333333333 5943916544
259.666666666667 5951576064
260 5959290880
260.333333333333 5966999552
260.666666666667 5974687744
261 5982361600
261.333333333333 5990039552
261.666666666667 5997690880
262 6005295104
262.333333333333 6012919808
262.666666666667 6020562944
263 6028253184
263.333333333333 6035957760
263.666666666667 6043674624
264 6051397632
264.333333333333 6059153408
264.666666666667 6066808832
265 6074542080
265.333333333333 6082189312
265.666666666667 6089797632
266 6097481728
266.333333333333 6105200640
266.666666666667 6112913408
267 6120652800
267.333333333333 6128361472
267.666666666667 6136025088
268 6143721472
268.333333333333 6151419904
268.666666666667 6159124480
269 6166804480
269.333333333333 6174461952
269.666666666667 6182119424
270 6189756416
270.333333333333 6197327872
270.666666666667 6204923904
271 6212542464
271.333333333333 6220208128
271.666666666667 6227869696
272 6235541504
272.333333333333 6243258368
272.666666666667 6250960896
273 6258632704
273.333333333333 6266331136
273.666666666667 6273986560
274 6281672704
274.333333333333 6289287168
274.666666666667 6296895488
275 6304528384
275.333333333333 6312200192
275.666666666667 6319831040
276 6327539712
276.333333333333 6335236096
276.666666666667 6342952960
277 6350645248
277.333333333333 6358290432
277.666666666667 6365962240
278 6373634048
278.333333333333 6381262848
278.666666666667 6388856832
279 6396506112
279.333333333333 6404159488
279.666666666667 6411888640
280 6419597312
280.333333333333 6427293696
280.666666666667 6434965504
281 6442639360
281.333333333333 6450309120
281.666666666667 6457956352
282 6465615872
282.333333333333 6473267200
282.666666666667 6480896000
283 6488516608
283.333333333333 6496176128
283.666666666667 6503876608
284 6511597568
284.333333333333 6519277568
284.666666666667 6526881792
285 6534504448
};
\addlegendentry{\sysKFour}
\addplot [semithick, color1, mark=*, mark size=1.5, mark options={solid,fill=white}, mark repeat=60,mark phase=30]
table {%
0 3207168
0.333333333333333 9842688
0.666666666666667 17862656
1 25892864
1.33333333333333 33904640
1.66666666666667 41893888
2 49854464
2.33333333333333 57819136
2.66666666666667 65794048
3 73771008
3.33333333333333 81737728
3.66666666666667 89739264
4 97710080
4.33333333333333 105664512
4.66666666666667 113647616
5 121604096
5.33333333333333 129587200
5.66666666666667 137500672
6 145483776
6.33333333333333 153434112
6.66666666666667 161409024
7 169398272
7.33333333333333 177362944
7.66666666666667 185300992
8 193294336
8.33333333333333 201252864
8.66666666666667 209213440
9 217163776
9.33333333333333 225140736
9.66666666666667 233084928
10 241022976
10.3333333333333 248975360
10.6666666666667 256940032
11 264916992
11.3333333333333 272877568
11.6666666666667 280827904
12 288786432
12.3333333333333 296718336
12.6666666666667 304666624
13 312627200
13.3333333333333 320591872
13.6666666666667 328574976
14 336531456
14.3333333333333 344473600
14.6666666666667 352423936
15 360329216
15.3333333333333 368273408
15.6666666666667 376203264
16 384161792
16.3333333333333 392085504
16.6666666666667 400025600
17 408006656
17.3333333333333 415954944
17.6666666666667 423909376
18 431867904
18.3333333333333 439810048
18.6666666666667 447774720
19 455729152
19.3333333333333 463685632
19.6666666666667 471615488
20 479543296
20.3333333333333 487497728
20.6666666666667 495452160
21 503410688
21.3333333333333 511361024
21.6666666666667 519333888
22 527292416
22.3333333333333 535255040
22.6666666666667 543199232
23 551139328
23.3333333333333 559106048
23.6666666666667 567037952
24 574984192
24.3333333333333 582942720
24.6666666666667 590895104
25 598861824
25.3333333333333 606791680
25.6666666666667 614748160
26 622716928
26.3333333333333 630675456
26.6666666666667 638627840
27 646557696
27.3333333333333 654520320
27.6666666666667 662478848
28 670433280
28.3333333333333 678389760
28.6666666666667 686362624
29 694310912
29.3333333333333 702271488
29.6666666666667 710219776
30 718178304
30.3333333333333 722161664
30.6666666666667 722161664
31 722161664
31.3333333333333 722161664
31.6666666666667 722161664
32 722161664
32.3333333333333 722161664
32.6666666666667 722161664
33 722161664
33.3333333333333 722161664
33.6666666666667 722161664
34 722161664
34.3333333333333 722161664
34.6666666666667 722161664
35 722161664
35.3333333333333 722161664
35.6666666666667 722161664
36 722161664
36.3333333333333 722161664
36.6666666666667 722161664
37 722161664
37.3333333333333 722161664
37.6666666666667 722161664
38 722161664
38.3333333333333 722161664
38.6666666666667 722161664
39 722161664
39.3333333333333 722161664
39.6666666666667 722161664
40 726149120
40.3333333333333 734101504
40.6666666666667 742045696
41 749989888
41.3333333333333 757938176
41.6666666666667 765896704
42 773842944
42.3333333333333 781817856
42.6666666666667 789753856
43 797696000
43.3333333333333 805644288
43.6666666666667 813627392
44 821612544
44.3333333333333 829589504
44.6666666666667 837515264
45 845438976
45.3333333333333 853377024
45.6666666666667 861347840
46 869302272
46.3333333333333 877256704
46.6666666666667 885219328
47 893175808
47.3333333333333 901132288
47.6666666666667 909080576
48 917045248
48.3333333333333 925009920
48.6666666666667 932943872
49 940912640
49.3333333333333 948867072
49.6666666666667 956817408
50 964763648
50.3333333333333 972734464
50.6666666666667 980707328
51 988659712
51.3333333333333 996612096
51.6666666666667 1004578816
52 1012541440
52.3333333333333 1020481536
52.6666666666667 1028411392
53 1036380160
53.3333333333333 1044326400
53.6666666666667 1052248064
54 1060194304
54.3333333333333 1068158976
54.6666666666667 1076101120
55 1084055552
55.3333333333333 1092003840
55.6666666666667 1099945984
56 1107904512
56.3333333333333 1115877376
56.6666666666667 1123833856
57 1131780096
57.3333333333333 1139744768
57.6666666666667 1147703296
58 1155647488
58.3333333333333 1163636736
58.6666666666667 1171570688
59 1179516928
59.3333333333333 1187442688
59.6666666666667 1195390976
60 1203337216
60.3333333333333 1211289600
60.6666666666667 1219225600
61 1227155456
61.3333333333333 1235107840
61.6666666666667 1243068416
62 1251024896
62.3333333333333 1258977280
62.6666666666667 1266913280
63 1274826752
63.3333333333333 1282785280
63.6666666666667 1290723328
64 1298671616
64.3333333333333 1306632192
64.6666666666667 1314564096
65 1322524672
65.3333333333333 1330470912
65.6666666666667 1338454016
66 1346416640
66.3333333333333 1354393600
66.6666666666667 1362350080
67 1370335232
67.3333333333333 1378304000
67.6666666666667 1386260480
68 1394219008
68.3333333333333 1402181632
68.6666666666667 1410129920
69 1418039296
69.3333333333333 1426020352
69.6666666666667 1433960448
70 1441910784
70.3333333333333 1449900032
70.6666666666667 1449900032
71 1449900032
71.3333333333333 1449900032
71.6666666666667 1449900032
72 1449900032
72.3333333333333 1449900032
72.6666666666667 1449900032
73 1449900032
73.3333333333333 1449900032
73.6666666666667 1449900032
74 1449900032
74.3333333333333 1449900032
74.6666666666667 1449900032
75 1449900032
75.3333333333333 1449900032
75.6666666666667 1449900032
76 1449900032
76.3333333333333 1449900032
76.6666666666667 1449900032
77 1449900032
77.3333333333333 1449900032
77.6666666666667 1449900032
78 1449900032
78.3333333333333 1449900032
78.6666666666667 1449900032
79 1449900032
79.3333333333333 1449900032
79.6666666666667 1449900032
80 1449900032
80.3333333333333 1453873152
80.6666666666667 1461835776
81 1469767680
81.3333333333333 1477722112
81.6666666666667 1485666304
82 1493600256
82.3333333333333 1501556736
82.6666666666667 1509513216
83 1517451264
83.3333333333333 1525430272
83.6666666666667 1533360128
84 1541300224
84.3333333333333 1549250560
84.6666666666667 1557196800
85 1565155328
85.3333333333333 1573076992
85.6666666666667 1581025280
86 1588996096
86.3333333333333 1596930048
86.6666666666667 1604872192
87 1612828672
87.3333333333333 1620813824
87.6666666666667 1628774400
88 1636749312
88.3333333333333 1644713984
88.6666666666667 1652672512
89 1660608512
89.3333333333333 1668544512
89.6666666666667 1676490752
90 1684441088
90.3333333333333 1692372992
90.6666666666667 1700315136
91 1708257280
91.3333333333333 1716187136
91.6666666666667 1724129280
92 1732057088
92.3333333333333 1740011520
92.6666666666667 1747953664
93 1755899904
93.3333333333333 1763846144
93.6666666666667 1771780096
94 1779738624
94.3333333333333 1787688960
94.6666666666667 1795649536
95 1803618304
95.3333333333333 1811556352
95.6666666666667 1819551744
96 1827543040
96.3333333333333 1835526144
96.6666666666667 1843492864
97 1851437056
97.3333333333333 1859389440
97.6666666666667 1867327488
98 1875300352
98.3333333333333 1883265024
98.6666666666667 1891215360
99 1899169792
99.3333333333333 1907118080
99.6666666666667 1915080704
100 1923053568
100.333333333333 1931018240
100.666666666667 1938982912
101 1946931200
101.333333333333 1954895872
101.666666666667 1962838016
102 1970788352
102.333333333333 1978740736
102.666666666667 1986699264
103 1994653696
103.333333333333 2002610176
103.666666666667 2010570752
104 2018506752
104.333333333333 2026440704
104.666666666667 2034382848
105 2042296320
105.333333333333 2050265088
105.666666666667 2058199040
106 2066157568
106.333333333333 2074128384
106.666666666667 2082062336
107 2090020864
107.333333333333 2097963008
107.666666666667 2105948160
108 2113910784
108.333333333333 2121879552
108.666666666667 2129844224
109 2137819136
109.333333333333 2145796096
109.666666666667 2153748480
110 2161704960
110.333333333333 2169663488
110.666666666667 2177619968
111 2177619968
111.333333333333 2177619968
111.666666666667 2177619968
112 2177619968
112.333333333333 2177619968
112.666666666667 2177619968
113 2177619968
113.333333333333 2177619968
113.666666666667 2177619968
114 2177619968
114.333333333333 2177619968
114.666666666667 2177619968
115 2177619968
115.333333333333 2177619968
115.666666666667 2177619968
116 2177619968
116.333333333333 2177619968
116.666666666667 2177619968
117 2177619968
117.333333333333 2177619968
117.666666666667 2177619968
118 2177619968
118.333333333333 2177619968
118.666666666667 2177619968
119 2177619968
119.333333333333 2177619968
119.666666666667 2177619968
120 2177619968
120.333333333333 2177619968
120.666666666667 2177619968
121 2177619968
121.333333333333 2177619968
121.666666666667 2181578752
122 2189537280
122.333333333333 2197487616
122.666666666667 2205431808
123 2213382144
123.333333333333 2221320192
123.666666666667 2229264384
124 2237196288
124.333333333333 2245154816
124.666666666667 2253137920
125 2261088256
125.333333333333 2269038592
125.666666666667 2276974592
126 2284935168
126.333333333333 2292873216
126.666666666667 2300846080
127 2308798464
127.333333333333 2316754944
127.666666666667 2324682752
128 2332637184
128.333333333333 2340603904
128.666666666667 2348578816
129 2356547584
129.333333333333 2364467200
129.666666666667 2372417536
130 2380351488
130.333333333333 2388312064
130.666666666667 2396256256
131 2404231168
131.333333333333 2412201984
131.666666666667 2420152320
132 2428096512
132.333333333333 2436059136
132.666666666667 2444015616
133 2451965952
133.333333333333 2459910144
133.666666666667 2467878912
134 2475841536
134.333333333333 2483802112
134.666666666667 2491768832
135 2499702784
135.333333333333 2507663360
135.666666666667 2515595264
136 2523551744
136.333333333333 2531497984
136.666666666667 2539468800
137 2547421184
137.333333333333 2555367424
137.666666666667 2563321856
138 2571282432
138.333333333333 2579257344
138.666666666667 2587217920
139 2595162112
139.333333333333 2603100160
139.666666666667 2611073024
140 2619004928
140.333333333333 2626967552
140.666666666667 2634901504
141 2642841600
141.333333333333 2650808320
141.666666666667 2658744320
142 2666721280
142.333333333333 2674690048
142.666666666667 2682681344
143 2690633728
143.333333333333 2698573824
143.666666666667 2706524160
144 2714462208
144.333333333333 2722428928
144.666666666667 2730362880
145 2738313216
145.333333333333 2746271744
145.666666666667 2754220032
146 2762174464
146.333333333333 2770145280
146.666666666667 2778095616
147 2786043904
147.333333333333 2793977856
147.666666666667 2801922048
148 2809905152
148.333333333333 2817851392
148.666666666667 2825805824
149 2833772544
149.333333333333 2841731072
149.666666666667 2849671168
150 2857639936
150.333333333333 2865594368
150.666666666667 2873542656
151 2881507328
151.333333333333 2889449472
151.666666666667 2897395712
152 2905344000
152.333333333333 2909306880
152.666666666667 2909306880
153 2909306880
153.333333333333 2909306880
153.666666666667 2909306880
154 2909306880
154.333333333333 2909306880
154.666666666667 2909306880
155 2909306880
155.333333333333 2909306880
155.666666666667 2909306880
156 2909306880
156.333333333333 2909306880
156.666666666667 2909306880
157 2909306880
157.333333333333 2909306880
157.666666666667 2909306880
158 2909306880
158.333333333333 2909306880
158.666666666667 2909306880
159 2909306880
159.333333333333 2909306880
159.666666666667 2909306880
160 2909306880
160.333333333333 2909306880
160.666666666667 2909306880
161 2909306880
161.333333333333 2909306880
161.666666666667 2917259264
162 2925205504
162.333333333333 2933159936
162.666666666667 2941104128
163 2949060608
163.333333333333 2957002752
163.666666666667 2964922368
164 2972887040
164.333333333333 2980823040
164.666666666667 2988771328
165 2996723712
165.333333333333 3004655616
165.666666666667 3012593664
166 3020546048
166.333333333333 3028510720
166.666666666667 3036467200
167 3044440064
167.333333333333 3052394496
167.666666666667 3060375552
168 3068350464
168.333333333333 3076294656
168.666666666667 3084255232
169 3092187136
169.333333333333 3100135424
169.666666666667 3108096000
170 3116042240
170.333333333333 3123970048
170.666666666667 3131926528
171 3139868672
171.333333333333 3147816960
171.666666666667 3155793920
172 3163744256
172.333333333333 3171700736
172.666666666667 3179640832
173 3187605504
173.333333333333 3195557888
173.666666666667 3203518464
174 3211433984
174.333333333333 3219404800
174.666666666667 3227357184
175 3235301376
175.333333333333 3243223040
175.666666666667 3251181568
176 3259140096
176.333333333333 3267086336
176.666666666667 3275057152
177 3282995200
177.333333333333 3290935296
177.666666666667 3298873344
178 3306858496
178.333333333333 3314808832
178.666666666667 3322773504
179 3330734080
179.333333333333 3338711040
179.666666666667 3346679808
180 3354648576
180.333333333333 3362607104
180.666666666667 3370584064
181 3378532352
181.333333333333 3386460160
181.666666666667 3394420736
182 3402377216
182.333333333333 3410315264
182.666666666667 3418277888
183 3426232320
183.333333333333 3434178560
183.666666666667 3442141184
184 3450073088
184.333333333333 3458027520
184.666666666667 3465990144
185 3473954816
185.333333333333 3481901056
185.666666666667 3489859584
186 3497822208
186.333333333333 3505774592
186.666666666667 3513718784
187 3521703936
187.333333333333 3529658368
187.666666666667 3537584128
188 3545552896
188.333333333333 3553513472
188.666666666667 3561461760
189 3569428480
189.333333333333 3577389056
189.666666666667 3585337344
190 3593297920
190.333333333333 3601238016
190.666666666667 3609169920
191 3617130496
191.333333333333 3625091072
191.666666666667 3633033216
192 3637006336
192.333333333333 3637006336
192.666666666667 3637006336
193 3637006336
193.333333333333 3637006336
193.666666666667 3637006336
194 3637006336
194.333333333333 3637006336
194.666666666667 3637006336
195 3637006336
195.333333333333 3637006336
195.666666666667 3637006336
196 3637006336
196.333333333333 3637006336
196.666666666667 3637006336
197 3637006336
197.333333333333 3637006336
197.666666666667 3637006336
198 3637006336
198.333333333333 3637006336
198.666666666667 3637006336
199 3637006336
199.333333333333 3637006336
199.666666666667 3637006336
200 3637006336
200.333333333333 3637006336
200.666666666667 3637006336
201 3637006336
201.333333333333 3637006336
201.666666666667 3637006336
202 3637006336
202.333333333333 3640997888
202.666666666667 3648968704
203 3656923136
203.333333333333 3664857088
203.666666666667 3672844288
204 3680800768
204.333333333333 3688747008
204.666666666667 3696717824
205 3704668160
205.333333333333 3712598016
205.666666666667 3720560640
206 3728504832
206.333333333333 3736446976
206.666666666667 3744393216
207 3752355840
207.333333333333 3760310272
207.666666666667 3768272896
208 3776272384
208.333333333333 3784230912
208.666666666667 3792189440
209 3800152064
209.333333333333 3808124928
209.666666666667 3816079360
210 3823998976
210.333333333333 3831959552
210.666666666667 3839916032
211 3847849984
211.333333333333 3855802368
211.666666666667 3863758848
212 3871705088
212.333333333333 3879653376
212.666666666667 3887591424
213 3895562240
213.333333333333 3903506432
213.666666666667 3911464960
214 3919411200
214.333333333333 3927398400
214.666666666667 3935375360
215 3943333888
215.333333333333 3951316992
215.666666666667 3959277568
216 3967281152
216.333333333333 3975233536
216.666666666667 3983169536
217 3991123968
217.333333333333 3999066112
217.666666666667 4007018496
218 4014964736
218.333333333333 4022900736
218.666666666667 4030861312
219 4038813696
219.333333333333 4046774272
219.666666666667 4054726656
220 4062683136
220.333333333333 4070639616
220.666666666667 4078589952
221 4086550528
221.333333333333 4094478336
221.666666666667 4102426624
222 4110376960
222.333333333333 4118329344
222.666666666667 4126285824
223 4134264832
223.333333333333 4142254080
223.666666666667 4150202368
224 4158191616
224.333333333333 4166166528
224.666666666667 4174143488
225 4182095872
225.333333333333 4190038016
225.666666666667 4197994496
226 4205942784
226.333333333333 4213911552
226.666666666667 4221865984
227 4229806080
227.333333333333 4237725696
227.666666666667 4245661696
228 4253605888
228.333333333333 4261566464
228.666666666667 4269500416
229 4277448704
229.333333333333 4285390848
229.666666666667 4293330944
230 4301275136
230.333333333333 4309231616
230.666666666667 4317171712
231 4325115904
231.333333333333 4333068288
231.666666666667 4340998144
232 4348936192
232.333333333333 4356876288
232.666666666667 4364828672
233 4364828672
233.333333333333 4364828672
233.666666666667 4364828672
234 4364828672
234.333333333333 4364828672
234.666666666667 4364828672
235 4364828672
235.333333333333 4364828672
235.666666666667 4364828672
236 4364828672
236.333333333333 4364828672
236.666666666667 4364828672
237 4364828672
237.333333333333 4364828672
237.666666666667 4364828672
238 4364828672
238.333333333333 4364828672
238.666666666667 4364828672
239 4364828672
239.333333333333 4364828672
239.666666666667 4364828672
240 4364828672
240.333333333333 4364828672
240.666666666667 4364828672
241 4364828672
241.333333333333 4364828672
241.666666666667 4364828672
242 4364828672
242.333333333333 4364828672
242.666666666667 4364828672
243 4364828672
243.333333333333 4368824320
243.666666666667 4376791040
244 4384772096
244.333333333333 4392747008
244.666666666667 4400691200
245 4408678400
245.333333333333 4416643072
245.666666666667 4424595456
246 4432533504
246.333333333333 4440475648
246.666666666667 4448417792
247 4456368128
247.333333333333 4464308224
247.666666666667 4472293376
248 4480256000
248.333333333333 4488224768
248.666666666667 4496168960
249 4504107008
249.333333333333 4512047104
249.666666666667 4519989248
250 4527923200
250.333333333333 4535902208
250.666666666667 4543846400
251 4551782400
251.333333333333 4559765504
251.666666666667 4567734272
252 4575723520
252.333333333333 4583690240
252.666666666667 4591624192
253 4599584768
253.333333333333 4607526912
253.666666666667 4615456768
254 4623425536
254.333333333333 4631345152
254.666666666667 4639287296
255 4647262208
255.333333333333 4655212544
255.666666666667 4663140352
256 4671121408
256.333333333333 4679065600
256.666666666667 4687003648
257 4694984704
257.333333333333 4702935040
257.666666666667 4710893568
258 4718835712
258.333333333333 4726784000
258.666666666667 4734722048
259 4742660096
259.333333333333 4750651392
259.666666666667 4758605824
260 4766582784
260.333333333333 4774543360
260.666666666667 4782485504
261 4790450176
261.333333333333 4798398464
261.666666666667 4806356992
262 4814290944
262.333333333333 4822231040
262.666666666667 4830185472
263 4838133760
263.333333333333 4846090240
263.666666666667 4854022144
264 4861984768
264.333333333333 4869943296
264.666666666667 4877860864
265 4885815296
265.333333333333 4893757440
265.666666666667 4901687296
266 4909633536
266.333333333333 4917581824
266.666666666667 4925526016
267 4933462016
267.333333333333 4941428736
267.666666666667 4949411840
268 4957362176
268.333333333333 4965322752
268.666666666667 4973254656
269 4981194752
269.333333333333 4989190144
269.666666666667 4997134336
270 5005082624
270.333333333333 5013008384
270.666666666667 5020962816
271 5028925440
271.333333333333 5036879872
271.666666666667 5044826112
272 5052805120
272.333333333333 5060749312
272.666666666667 5068732416
273 5076697088
273.333333333333 5084676096
273.666666666667 5092636672
274 5092636672
274.333333333333 5092636672
274.666666666667 5092636672
275 5092636672
275.333333333333 5092636672
275.666666666667 5092636672
276 5092636672
276.333333333333 5092636672
276.666666666667 5092636672
277 5092636672
277.333333333333 5092636672
277.666666666667 5092636672
278 5092636672
278.333333333333 5092636672
278.666666666667 5092636672
279 5092636672
279.333333333333 5092636672
279.666666666667 5092636672
280 5092636672
280.333333333333 5092636672
280.666666666667 5092636672
281 5092636672
281.333333333333 5092636672
281.666666666667 5092636672
282 5092636672
282.333333333333 5092636672
282.666666666667 5092636672
283 5092636672
283.333333333333 5092636672
283.666666666667 5092636672
284 5100601344
284.333333333333 5108555776
284.666666666667 5116534784
285 5124487168
285.333333333333 5132419072
285.666666666667 5140367360
286 5148325888
286.333333333333 5156251648
286.666666666667 5164216320
287 5172170752
287.333333333333 5180133376
287.666666666667 5188081664
288 5196052480
288.333333333333 5204015104
288.666666666667 5211947008
289 5219909632
289.333333333333 5227864064
289.666666666667 5235806208
290 5243758592
290.333333333333 5251700736
290.666666666667 5259655168
291 5267611648
291.333333333333 5275572224
291.666666666667 5283553280
292 5291511808
292.333333333333 5299476480
292.666666666667 5307432960
293 5315389440
293.333333333333 5323333632
293.666666666667 5331261440
294 5339226112
294.333333333333 5347141632
294.666666666667 5355087872
295 5363038208
295.333333333333 5370978304
295.666666666667 5378932736
296 5386878976
296.333333333333 5394819072
296.666666666667 5402777600
297 5410740224
297.333333333333 5418723328
297.666666666667 5426706432
298 5434638336
298.333333333333 5442625536
298.666666666667 5450612736
299 5458597888
299.333333333333 5466554368
299.666666666667 5474506752
300 5482481664
300.333333333333 5490407424
300.666666666667 5498353664
301 5506308096
301.333333333333 5514252288
301.666666666667 5522198528
302 5530114048
302.333333333333 5538078720
302.666666666667 5546018816
303 5553973248
303.333333333333 5561931776
303.666666666667 5569890304
304 5577848832
304.333333333333 5585815552
304.666666666667 5593769984
305 5601695744
305.333333333333 5609674752
305.666666666667 5617635328
306 5625546752
306.333333333333 5633480704
306.666666666667 5641426944
307 5649369088
307.333333333333 5657325568
307.666666666667 5665255424
308 5673191424
308.333333333333 5681158144
308.666666666667 5689118720
309 5697067008
309.333333333333 5705039872
309.666666666667 5713010688
310 5720936448
310.333333333333 5728892928
310.666666666667 5736841216
311 5744769024
311.333333333333 5752733696
311.666666666667 5760665600
312 5768630272
312.333333333333 5776578560
312.666666666667 5784535040
313 5792460800
313.333333333333 5800388608
313.666666666667 5808361472
314 5816295424
314.333333333333 5824260096
314.666666666667 5824260096
315 5824260096
315.333333333333 5824260096
315.666666666667 5824260096
316 5824260096
316.333333333333 5824260096
316.666666666667 5824260096
317 5824260096
317.333333333333 5824260096
317.666666666667 5824260096
318 5824260096
318.333333333333 5824260096
318.666666666667 5824260096
319 5824260096
319.333333333333 5824260096
319.666666666667 5824260096
320 5824260096
320.333333333333 5824260096
320.666666666667 5824260096
321 5824260096
321.333333333333 5824260096
321.666666666667 5824260096
322 5824260096
322.333333333333 5824260096
322.666666666667 5824260096
323 5824260096
323.333333333333 5824260096
323.666666666667 5824260096
};
\addlegendentry{\ckptThirty}
\addplot [semithick, color3,  mark=diamond*, mark size=2.0, mark options={solid,fill=white}, mark repeat=60,mark phase=15]
table {%
0 0
0.333333333333333 710656
0.666666666666667 9043968
1 17166336
1.33333333333333 25198592
1.66666666666667 33159168
2 41105408
2.33333333333333 48994304
2.66666666666667 56821760
3 64636928
3.33333333333333 72497152
3.66666666666667 80328704
4 88190976
4.33333333333333 95971328
4.66666666666667 103749632
5 111519744
5.33333333333333 119250944
5.66666666666667 127027200
6 134778880
6.33333333333333 142565376
6.66666666666667 150317056
7 158081024
7.33333333333333 165795840
7.66666666666667 173516800
8 181260288
8.33333333333333 188987392
8.66666666666667 196720640
9 204412928
9.33333333333333 212150272
9.66666666666667 219867136
10 227532800
10.3333333333333 235198464
10.6666666666667 242841600
11 250497024
11.3333333333333 258181120
11.6666666666667 265863168
12 273514496
12.3333333333333 281194496
12.6666666666667 288882688
13 296560640
13.3333333333333 304281600
13.6666666666667 311967744
14 319633408
14.3333333333333 327313408
14.6666666666667 334981120
15 342691840
15.3333333333333 350365696
15.6666666666667 358041600
16 365744128
16.3333333333333 373411840
16.6666666666667 381104128
17 388751360
17.3333333333333 396435456
17.6666666666667 404088832
18 411729920
18.3333333333333 419368960
18.6666666666667 427053056
19 434696192
19.3333333333333 442349568
19.6666666666667 450002944
20 457654272
20.3333333333333 465340416
20.6666666666667 473018368
21 480665600
21.3333333333333 488316928
21.6666666666667 495974400
22 503623680
22.3333333333333 511258624
22.6666666666667 518891520
23 526548992
23.3333333333333 534183936
23.6666666666667 541790208
24 549439488
24.3333333333333 557066240
24.6666666666667 564678656
25 572321792
25.3333333333333 579958784
25.6666666666667 587610112
26 595232768
26.3333333333333 602861568
26.6666666666667 610494464
27 618127360
27.3333333333333 625795072
27.6666666666667 633432064
28 641069056
28.3333333333333 648691712
28.6666666666667 656312320
29 663947264
29.3333333333333 671551488
29.6666666666667 679178240
30 686813184
30.3333333333333 694470656
30.6666666666667 702113792
31 709775360
31.3333333333333 717418496
31.6666666666667 725082112
32 732729344
32.3333333333333 740356096
32.6666666666667 748027904
33 755679232
33.3333333333333 763340800
33.6666666666667 771010560
34 778670080
34.3333333333333 786333696
34.6666666666667 793933824
35 801589248
35.3333333333333 809246720
35.6666666666667 816898048
36 824571904
36.3333333333333 832225280
36.6666666666667 839903232
37 847579136
37.3333333333333 855238656
37.6666666666667 862877696
38 870555648
38.3333333333333 878231552
38.6666666666667 885919744
39 893558784
39.3333333333333 901230592
39.6666666666667 908926976
40 916633600
40.3333333333333 924325888
40.6666666666667 932005888
41 939681792
41.3333333333333 947351552
41.6666666666667 955039744
42 962734080
42.3333333333333 970412032
42.6666666666667 978096128
43 985778176
43.3333333333333 993445888
43.6666666666667 1001093120
44 1008750592
44.3333333333333 1016410112
44.6666666666667 1024040960
45 1031686144
45.3333333333333 1039310848
45.6666666666667 1046976512
46 1054619648
46.3333333333333 1062242304
46.6666666666667 1069887488
47 1077495808
47.3333333333333 1085120512
47.6666666666667 1092763648
48 1100412928
48.3333333333333 1108064256
48.6666666666667 1115686912
49 1123307520
49.3333333333333 1130942464
49.6666666666667 1138593792
50 1146232832
50.3333333333333 1153914880
50.6666666666667 1161590784
51 1169242112
51.3333333333333 1176909824
51.6666666666667 1184565248
52 1192198144
52.3333333333333 1199841280
52.6666666666667 1207474176
53 1215139840
53.3333333333333 1222780928
53.6666666666667 1230409728
54 1238063104
54.3333333333333 1245673472
54.6666666666667 1253300224
55 1260943360
55.3333333333333 1268600832
55.6666666666667 1276246016
56 1283870720
56.3333333333333 1291505664
56.6666666666667 1299156992
57 1306796032
57.3333333333333 1314439168
57.6666666666667 1322055680
58 1329690624
58.3333333333333 1337317376
58.6666666666667 1344944128
59 1352597504
59.3333333333333 1360242688
59.6666666666667 1367871488
60 1375488000
60.3333333333333 1383102464
60.6666666666667 1390735360
61 1398345728
61.3333333333333 1405976576
61.6666666666667 1413611520
62 1421275136
62.3333333333333 1428914176
62.6666666666667 1436569600
63 1444212736
63.3333333333333 1451880448
63.6666666666667 1459558400
64 1467246592
64.3333333333333 1474924544
64.6666666666667 1482604544
65 1490253824
65.3333333333333 1497929728
65.6666666666667 1505589248
66 1513224192
66.3333333333333 1520871424
66.6666666666667 1528553472
67 1536208896
67.3333333333333 1543870464
67.6666666666667 1551515648
68 1559152640
68.3333333333333 1566822400
68.6666666666667 1574510592
69 1582163968
69.3333333333333 1589833728
69.6666666666667 1597487104
70 1605142528
70.3333333333333 1612765184
70.6666666666667 1620387840
71 1628002304
71.3333333333333 1635639296
71.6666666666667 1643249664
72 1650876416
72.3333333333333 1658521600
72.6666666666667 1666183168
73 1673820160
73.3333333333333 1681485824
73.6666666666667 1689133056
74 1696806912
74.3333333333333 1704491008
74.6666666666667 1712179200
75 1719857152
75.3333333333333 1727545344
75.6666666666667 1735184384
76 1742850048
76.3333333333333 1750507520
76.6666666666667 1758171136
77 1765808128
77.3333333333333 1773430784
77.6666666666667 1781094400
78 1788733440
78.3333333333333 1796397056
78.6666666666667 1804060672
79 1811722240
79.3333333333333 1819392000
79.6666666666667 1827004416
80 1834661888
80.3333333333333 1842317312
80.6666666666667 1849966592
81 1857640448
81.3333333333333 1865302016
81.6666666666667 1872975872
82 1880651776
82.3333333333333 1888307200
82.6666666666667 1895952384
83 1903638528
83.3333333333333 1911271424
83.6666666666667 1918889984
84 1926537216
84.3333333333333 1934157824
84.6666666666667 1941776384
85 1949407232
85.3333333333333 1957054464
85.6666666666667 1964699648
86 1972326400
86.3333333333333 1979947008
86.6666666666667 1987567616
87 1995208704
87.3333333333333 2002878464
87.6666666666667 2010527744
88 2018168832
88.3333333333333 2025781248
88.6666666666667 2033383424
89 2041026560
89.3333333333333 2048630784
89.6666666666667 2056271872
90 2063884288
90.3333333333333 2071529472
90.6666666666667 2079150080
91 2086776832
91.3333333333333 2094415872
91.6666666666667 2102046720
92 2109693952
92.3333333333333 2117314560
92.6666666666667 2124949504
93 2132596736
93.3333333333333 2140248064
93.6666666666667 2147885056
94 2155515904
94.3333333333333 2163150848
94.6666666666667 2170783744
95 2178410496
95.3333333333333 2186078208
95.6666666666667 2193719296
96 2201352192
96.3333333333333 2208972800
96.6666666666667 2216665088
97 2224365568
97.3333333333333 2232035328
97.6666666666667 2239709184
98 2247395328
98.3333333333333 2255056896
98.6666666666667 2262714368
99 2270371840
99.3333333333333 2278029312
99.6666666666667 2285668352
100 2293309440
100.333333333333 2300948480
100.666666666667 2308605952
101 2316247040
101.333333333333 2323869696
101.666666666667 2331514880
102 2339129344
102.333333333333 2346754048
102.666666666667 2354395136
103 2362048512
103.333333333333 2369691648
103.666666666667 2377324544
104 2384943104
104.333333333333 2392571904
104.666666666667 2400208896
105 2407868416
105.333333333333 2415491072
105.666666666667 2423134208
106 2430760960
106.333333333333 2438385664
106.666666666667 2446049280
107 2453671936
107.333333333333 2461313024
107.666666666667 2468937728
108 2476564480
108.333333333333 2484219904
108.666666666667 2491895808
109 2499510272
109.333333333333 2507137024
109.666666666667 2514792448
110 2522443776
110.333333333333 2530097152
110.666666666667 2537748480
111 2545387520
111.333333333333 2553030656
111.666666666667 2560665600
112 2568337408
112.333333333333 2575972352
112.666666666667 2583597056
113 2591252480
113.333333333333 2598862848
113.666666666667 2606489600
114 2614136832
114.333333333333 2621777920
114.666666666667 2629419008
115 2637037568
115.333333333333 2644666368
115.666666666667 2652303360
116 2659950592
116.333333333333 2667601920
116.666666666667 2675228672
117 2682857472
117.333333333333 2690478080
117.666666666667 2698115072
118 2705786880
118.333333333333 2713436160
118.666666666667 2721067008
119 2728695808
119.333333333333 2736357376
119.666666666667 2744006656
120 2751670272
120.333333333333 2759301120
120.666666666667 2766936064
121 2774583296
121.333333333333 2782238720
121.666666666667 2789883904
122 2797500416
122.333333333333 2805141504
122.666666666667 2812764160
123 2820388864
123.333333333333 2828058624
123.666666666667 2835738624
124 2843412480
124.333333333333 2851090432
124.666666666667 2858756096
125 2866417664
125.333333333333 2874097664
125.666666666667 2881742848
126 2889383936
126.333333333333 2897049600
126.666666666667 2904731648
127 2912360448
127.333333333333 2920026112
127.666666666667 2927689728
128 2935343104
128.333333333333 2943039488
128.666666666667 2950694912
129 2958354432
129.333333333333 2966020096
129.666666666667 2973648896
130 2981289984
130.333333333333 2988920832
130.666666666667 2996541440
131 3004172288
131.333333333333 3011809280
131.666666666667 3019460608
132 3027081216
132.333333333333 3034728448
132.666666666667 3042365440
133 3049984000
133.333333333333 3057635328
133.666666666667 3065307136
134 3072919552
134.333333333333 3080558592
134.666666666667 3088171008
135 3095793664
135.333333333333 3103395840
135.666666666667 3111010304
136 3118667776
136.333333333333 3126321152
136.666666666667 3133992960
137 3141611520
137.333333333333 3149254656
137.666666666667 3156875264
138 3164504064
138.333333333333 3172155392
138.666666666667 3179804672
139 3187499008
139.333333333333 3195150336
139.666666666667 3202793472
140 3210463232
140.333333333333 3218108416
140.666666666667 3225745408
141 3233400832
141.333333333333 3241056256
141.666666666667 3248693248
142 3256320000
142.333333333333 3263965184
142.666666666667 3271596032
143 3279233024
143.333333333333 3286863872
143.666666666667 3294494720
144 3302129664
144.333333333333 3309789184
144.666666666667 3317420032
145 3325063168
145.333333333333 3332685824
145.666666666667 3340312576
146 3347957760
146.333333333333 3355613184
146.666666666667 3363305472
147 3370948608
147.333333333333 3378608128
147.666666666667 3386277888
148 3393912832
148.333333333333 3401553920
148.666666666667 3409201152
149 3416848384
149.333333333333 3424487424
149.666666666667 3432110080
150 3439771648
150.333333333333 3447447552
150.666666666667 3455100928
151 3462768640
151.333333333333 3470462976
151.666666666667 3478169600
152 3485855744
152.333333333333 3493543936
152.666666666667 3501215744
153 3508889600
153.333333333333 3516585984
153.666666666667 3524284416
154 3531952128
154.333333333333 3539638272
154.666666666667 3547318272
155 3554990080
155.333333333333 3562635264
155.666666666667 3570298880
156 3577952256
156.333333333333 3585583104
156.666666666667 3593205760
157 3600846848
157.333333333333 3608526848
157.666666666667 3616149504
158 3623780352
158.333333333333 3631392768
158.666666666667 3639021568
159 3646636032
159.333333333333 3654260736
159.666666666667 3661918208
160 3669569536
160.333333333333 3677214720
160.666666666667 3684866048
161 3692513280
161.333333333333 3700164608
161.666666666667 3707832320
162 3715512320
162.333333333333 3723180032
162.666666666667 3730857984
163 3738525696
163.333333333333 3746203648
163.666666666667 3753873408
164 3761522688
164.333333333333 3769182208
164.666666666667 3776849920
165 3784503296
165.333333333333 3792138240
165.666666666667 3799762944
166 3807369216
166.333333333333 3815010304
166.666666666667 3822612480
167 3830245376
167.333333333333 3837896704
167.666666666667 3845556224
168 3853205504
168.333333333333 3860871168
168.666666666667 3868512256
169 3876171776
169.333333333333 3883845632
169.666666666667 3891531776
170 3899160576
170.333333333333 3906818048
170.666666666667 3914438656
171 3922077696
171.333333333333 3929706496
171.666666666667 3937331200
172 3944970240
172.333333333333 3952648192
172.666666666667 3960268800
173 3967905792
173.333333333333 3975522304
173.666666666667 3983140864
174 3990751232
174.333333333333 3998363648
174.666666666667 4006012928
175 4013670400
175.333333333333 4021325824
175.666666666667 4028950528
176 4036587520
176.333333333333 4044204032
176.666666666667 4051836928
177 4059465728
177.333333333333 4067088384
177.666666666667 4074729472
178 4082407424
178.333333333333 4090028032
178.666666666667 4097650688
179 4105295872
179.333333333333 4112955392
179.666666666667 4120619008
180 4128278528
180.333333333333 4135911424
180.666666666667 4143554560
181 4151185408
181.333333333333 4158851072
181.666666666667 4166490112
182 4174112768
182.333333333333 4181760000
182.666666666667 4189378560
183 4197015552
183.333333333333 4204662784
183.666666666667 4212252672
184 4219887616
184.333333333333 4227518464
184.666666666667 4235182080
185 4242831360
185.333333333333 4250488832
185.666666666667 4258142208
186 4265816064
186.333333333333 4273463296
186.666666666667 4281088000
187 4288747520
187.333333333333 4296382464
187.666666666667 4304050176
188 4311715840
188.333333333333 4319379456
188.666666666667 4327047168
189 4334667776
189.333333333333 4342312960
189.666666666667 4349970432
190 4357611520
190.333333333333 4365246464
190.666666666667 4372908032
191 4380542976
191.333333333333 4388165632
191.666666666667 4395806720
192 4403417088
192.333333333333 4411058176
192.666666666667 4418727936
193 4426412032
193.333333333333 4434085888
193.666666666667 4441774080
194 4449421312
194.333333333333 4457091072
194.666666666667 4464744448
195 4472375296
195.333333333333 4480028672
195.666666666667 4487729152
196 4495380480
196.333333333333 4503042048
196.666666666667 4510689280
197 4518330368
197.333333333333 4525965312
197.666666666667 4533630976
198 4541265920
198.333333333333 4548884480
198.666666666667 4556533760
199 4564154368
199.333333333333 4571774976
199.666666666667 4579418112
200 4587063296
200.333333333333 4594704384
200.666666666667 4602320896
201 4609945600
201.333333333333 4617580544
201.666666666667 4625219584
202 4632862720
202.333333333333 4640485376
202.666666666667 4648122368
203 4655745024
203.333333333333 4663367680
203.666666666667 4670994432
204 4678627328
204.333333333333 4686254080
204.666666666667 4693919744
205 4701562880
205.333333333333 4709195776
205.666666666667 4716802048
206 4724412416
206.333333333333 4732047360
206.666666666667 4739647488
207 4747290624
207.333333333333 4754931712
207.666666666667 4762605568
208 4770248704
208.333333333333 4777863168
208.666666666667 4785496064
209 4793135104
209.333333333333 4800759808
209.666666666667 4808388608
210 4816078848
210.333333333333 4823736320
210.666666666667 4831375360
211 4839034880
211.333333333333 4846667776
211.666666666667 4854306816
212 4861943808
212.333333333333 4869603328
212.666666666667 4877248512
213 4884883456
213.333333333333 4892563456
213.666666666667 4900247552
214 4907898880
214.333333333333 4915574784
214.666666666667 4923269120
215 4930971648
215.333333333333 4938665984
215.666666666667 4946341888
216 4954019840
216.333333333333 4961695744
216.666666666667 4969357312
217 4977031168
217.333333333333 4984717312
217.666666666667 4992380928
218 5000046592
218.333333333333 5007734784
218.666666666667 5015422976
219 5023143936
219.333333333333 5030836224
219.666666666667 5038508032
220 5046181888
220.333333333333 5053847552
220.666666666667 5061560320
221 5069232128
221.333333333333 5076910080
221.666666666667 5084592128
222 5092276224
222.333333333333 5099915264
222.666666666667 5107568640
223 5115224064
223.333333333333 5122859008
223.666666666667 5130479616
224 5138118656
224.333333333333 5145786368
224.666666666667 5153427456
225 5161056256
225.333333333333 5168672768
225.666666666667 5176283136
226 5183918080
226.333333333333 5191520256
226.666666666667 5199163392
227 5206806528
227.333333333333 5214461952
227.666666666667 5222113280
228 5229768704
228.333333333333 5237411840
228.666666666667 5245089792
229 5252726784
229.333333333333 5260341248
229.666666666667 5268004864
230 5275650048
230.333333333333 5283260416
230.666666666667 5290915840
231 5298597888
231.333333333333 5306292224
231.666666666667 5313974272
232 5321648128
232.333333333333 5329291264
232.666666666667 5336961024
233 5344608256
233.333333333333 5352239104
233.666666666667 5359892480
234 5367576576
234.333333333333 5375236096
234.666666666667 5382889472
235 5390528512
235.333333333333 5398173696
235.666666666667 5405847552
236 5413525504
236.333333333333 5421176832
236.666666666667 5428822016
237 5436424192
237.333333333333 5444042752
237.666666666667 5451679744
238 5459316736
238.333333333333 5466970112
238.666666666667 5474596864
239 5482225664
239.333333333333 5489862656
239.666666666667 5497503744
240 5505144832
240.333333333333 5512765440
240.666666666667 5520396288
241 5528031232
241.333333333333 5535668224
241.666666666667 5543335936
242 5550987264
242.333333333333 5558616064
242.666666666667 5566230528
243 5573924864
243.333333333333 5581533184
243.666666666667 5589174272
244 5596809216
244.333333333333 5604458496
244.666666666667 5612099584
245 5619720192
245.333333333333 5627340800
245.666666666667 5634971648
246 5642596352
246.333333333333 5650264064
246.666666666667 5657884672
247 5665521664
247.333333333333 5673148416
247.666666666667 5680785408
248 5688453120
248.333333333333 5696075776
248.666666666667 5703710720
249 5711339520
249.333333333333 5718972416
249.666666666667 5726611456
250 5734305792
250.333333333333 5741996032
250.666666666667 5749676032
251 5757353984
251.333333333333 5765015552
251.666666666667 5772701696
252 5780406272
252.333333333333 5788069888
252.666666666667 5795758080
253 5803436032
253.333333333333 5811109888
253.666666666667 5818763264
254 5826428928
254.333333333333 5834078208
254.666666666667 5841715200
255 5849360384
255.333333333333 5856997376
255.666666666667 5864663040
256 5872310272
256.333333333333 5879934976
256.666666666667 5887596544
257 5895254016
257.333333333333 5902931968
257.666666666667 5910575104
258 5918216192
258.333333333333 5925875712
258.666666666667 5933543424
259 5941188608
259.333333333333 5948852224
259.666666666667 5956503552
260 5964154880
260.333333333333 5971849216
260.666666666667 5979506688
261 5987155968
261.333333333333 5994778624
261.666666666667 6002391040
262 6010025984
262.333333333333 6017658880
262.666666666667 6025318400
263 6032945152
263.333333333333 6040608768
263.666666666667 6048280576
264 6055946240
264.333333333333 6063622144
264.666666666667 6071273472
265 6078941184
265.333333333333 6086633472
265.666666666667 6094344192
266 6102030336
266.333333333333 6109708288
266.666666666667 6117388288
267 6125068288
267.333333333333 6132756480
267.666666666667 6140454912
268 6148124672
268.333333333333 6155808768
268.666666666667 6163478528
269 6171148288
269.333333333333 6178799616
269.666666666667 6186461184
270 6194155520
270.333333333333 6201817088
270.666666666667 6209470464
271 6217123840
271.333333333333 6224787456
271.666666666667 6232422400
272 6240057344
272.333333333333 6247698432
272.666666666667 6255357952
273 6263001088
273.333333333333 6270640128
273.666666666667 6278260736
274 6285877248
274.333333333333 6293514240
274.666666666667 6301110272
275 6308753408
275.333333333333 6316388352
275.666666666667 6324039680
276 6331684864
276.333333333333 6339352576
276.666666666667 6347087872
277 6354798592
277.333333333333 6362519552
277.666666666667 6370254848
278 6377975808
278.333333333333 6385678336
278.666666666667 6393399296
279 6401140736
279.333333333333 6408822784
279.666666666667 6416490496
280 6424133632
280.333333333333 6431768576
280.666666666667 6439452672
281 6447126528
281.333333333333 6454804480
281.666666666667 6462455808
282 6470144000
282.333333333333 6477828096
282.666666666667 6485524480
283 6493208576
};
\addlegendentry{\sysKTwo}



==> figures/evaluation/data/normal/criteo-4x/tput.tex <==
\addplot [semithick, color0,mark=square*, mark size=1.5, mark options={solid,fill=white}, mark repeat=60,mark phase=0]
table {%
0 44646.4
0.333333333333333 451584
0.666666666666667 437248
1 427008
1.33333333333333 424140.8
1.66666666666667 420864
2 418816
2.33333333333333 416153.6
2.66666666666667 415129.6
3 414822.4
3.33333333333333 412160
3.66666666666667 410419.2
4 407756.8
4.33333333333333 407449.6
4.66666666666667 408985.6
5 406118.4
5.33333333333333 409088
5.66666666666667 407756.8
6 409292.8
6.33333333333333 408268.8
6.66666666666667 408883.2
7 408166.4
7.33333333333333 408268.8
7.66666666666667 409497.6
8 407654.4
8.33333333333333 405811.2
8.66666666666667 405606.4
9 407347.2
9.33333333333333 408268.8
9.66666666666667 405606.4
10 402534.4
10.3333333333333 401920
10.6666666666667 403456
11 399564.8
11.3333333333333 400281.6
11.6666666666667 400998.4
12 404172.8
12.3333333333333 402022.4
12.6666666666667 401408
13 400998.4
13.3333333333333 400486.4
13.6666666666667 398950.4
14 397926.4
14.3333333333333 397824
14.6666666666667 401305.6
15 399360
15.3333333333333 400691.2
15.6666666666667 401100.8
16 402227.2
16.3333333333333 401100.8
16.6666666666667 399974.4
17 398131.2
17.3333333333333 398745.6
17.6666666666667 400588.8
18 398848
18.3333333333333 398643.2
18.6666666666667 398848
19 398438.4
19.3333333333333 396185.6
19.6666666666667 396288
20 399052.8
20.3333333333333 397926.4
20.6666666666667 398233.6
21 399564.8
21.3333333333333 399974.4
21.6666666666667 398540.8
22 398131.2
22.3333333333333 399667.2
22.6666666666667 397824
23 397926.4
23.3333333333333 398950.4
23.6666666666667 398438.4
24 397721.6
24.3333333333333 397824
24.6666666666667 402432
25 399974.4
25.3333333333333 397516.8
25.6666666666667 398028.8
26 399257.6
26.3333333333333 396800
26.6666666666667 395264
27 395776
27.3333333333333 398028.8
27.6666666666667 397414.4
28 397414.4
28.3333333333333 397926.4
28.6666666666667 397107.2
29 397619.2
29.3333333333333 397004.8
29.6666666666667 400588.8
30 397926.4
30.3333333333333 397107.2
30.6666666666667 397926.4
31 399564.8
31.3333333333333 397721.6
31.6666666666667 398848
32 400793.6
32.3333333333333 400691.2
32.6666666666667 398336
33 398131.2
33.3333333333333 398643.2
33.6666666666667 403353.6
34 397312
34.3333333333333 398028.8
34.6666666666667 398540.8
35 398848
35.3333333333333 395673.6
35.6666666666667 395264
36 397414.4
36.3333333333333 397004.8
36.6666666666667 397721.6
37 398233.6
37.3333333333333 397414.4
37.6666666666667 396185.6
38 398745.6
38.3333333333333 398131.2
38.6666666666667 399155.2
39 398028.8
39.3333333333333 398438.4
39.6666666666667 403456
40 399360
40.3333333333333 399564.8
40.6666666666667 398745.6
41 399667.2
41.3333333333333 399872
41.6666666666667 397824
42 398643.2
42.3333333333333 399667.2
42.6666666666667 397209.6
43 395776
43.3333333333333 396902.4
43.6666666666667 398848
44 398336
44.3333333333333 399564.8
44.6666666666667 399257.6
45 399769.6
45.3333333333333 397926.4
45.6666666666667 398643.2
46 398950.4
46.3333333333333 398643.2
46.6666666666667 403353.6
47 397312
47.3333333333333 398028.8
47.6666666666667 398540.8
48 398848
48.3333333333333 395673.6
48.6666666666667 395264
49 397414.4
49.3333333333333 397004.8
49.6666666666667 397721.6
50 398233.6
50.3333333333333 397414.4
50.6666666666667 396185.6
51 398745.6
51.3333333333333 398131.2
51.6666666666667 399155.2
52 398028.8
52.3333333333333 398438.4
52.6666666666667 401920
53 397209.6
53.3333333333333 395776
53.6666666666667 396902.4
54 398848
54.3333333333333 398336
54.6666666666667 399564.8
55 399257.6
55.3333333333333 399769.6
55.6666666666667 397926.4
56 398643.2
56.3333333333333 398950.4
56.6666666666667 398643.2
57 403353.6
57.3333333333333 397312
57.6666666666667 398028.8
58 398540.8
58.3333333333333 398848
58.6666666666667 395673.6
59 395264
59.3333333333333 396390.4
59.6666666666667 402227.2
60 398438.4
60.3333333333333 396185.6
60.6666666666667 396288
61 399052.8
61.3333333333333 397926.4
61.6666666666667 398233.6
62 399564.8
62.3333333333333 399974.4
62.6666666666667 398540.8
63 398131.2
63.3333333333333 399667.2
63.6666666666667 397824
64 402432
64.3333333333333 399974.4
64.6666666666667 397516.8
65 398028.8
65.3333333333333 399257.6
65.6666666666667 396800
66 395264
66.3333333333333 396390.4
66.6666666666667 402227.2
67 398438.4
67.3333333333333 396185.6
67.6666666666667 396288
68 399052.8
68.3333333333333 397926.4
68.6666666666667 398233.6
69 399564.8
69.3333333333333 399974.4
69.6666666666667 398540.8
70 398131.2
70.3333333333333 399667.2
70.6666666666667 397824
71 402432
71.3333333333333 399974.4
71.6666666666667 397516.8
72 398028.8
72.3333333333333 399257.6
72.6666666666667 397414.4
73 398540.8
73.3333333333333 398848
73.6666666666667 395673.6
74 395776
74.3333333333333 398438.4
74.6666666666667 401920
75 397209.6
75.3333333333333 395776
75.6666666666667 396902.4
76 398848
76.3333333333333 398336
76.6666666666667 399564.8
77 399257.6
77.3333333333333 399769.6
77.6666666666667 397926.4
78 398643.2
78.3333333333333 398950.4
78.6666666666667 398643.2
79 403353.6
79.3333333333333 399257.6
79.6666666666667 399769.6
80 397926.4
80.3333333333333 398643.2
80.6666666666667 398950.4
81 398643.2
81.3333333333333 403353.6
81.6666666666667 397312
82 398028.8
82.3333333333333 398540.8
82.6666666666667 398848
83 395673.6
83.3333333333333 395264
83.6666666666667 396390.4
84 402227.2
84.3333333333333 398438.4
84.6666666666667 396185.6
85 396288
85.3333333333333 399052.8
85.6666666666667 397926.4
86 399155.2
86.3333333333333 397414.4
86.6666666666667 398540.8
87 398848
87.3333333333333 395673.6
87.6666666666667 395776
88 398438.4
88.3333333333333 401920
88.6666666666667 397209.6
89 395776
89.3333333333333 396902.4
89.6666666666667 398848
90 398336
90.3333333333333 399564.8
90.6666666666667 399257.6
91 399769.6
91.3333333333333 397926.4
91.6666666666667 398643.2
92 398950.4
92.3333333333333 398643.2
92.6666666666667 402739.2
93 397926.4
93.3333333333333 398233.6
93.6666666666667 399564.8
94 399974.4
94.3333333333333 398540.8
94.6666666666667 398131.2
95 399667.2
95.3333333333333 397824
95.6666666666667 402432
96 399974.4
96.3333333333333 399974.4
96.6666666666667 398540.8
97 398131.2
97.3333333333333 399667.2
97.6666666666667 397824
98 402432
98.3333333333333 399974.4
98.6666666666667 397516.8
99 398028.8
99.3333333333333 398336
99.6666666666667 397107.2
100 402227.2
100.333333333333 398438.4
100.666666666667 396185.6
101 396288
101.333333333333 399052.8
101.666666666667 397926.4
102 398233.6
102.333333333333 399564.8
102.666666666667 399974.4
103 398540.8
103.333333333333 398131.2
103.666666666667 399667.2
104 397824
104.333333333333 402432
104.666666666667 399974.4
105 397516.8
105.333333333333 398028.8
105.666666666667 399257.6
106 397004.8
106.333333333333 396902.4
106.666666666667 398848
107 398336
107.333333333333 399564.8
107.666666666667 399257.6
108 399769.6
108.333333333333 397926.4
108.666666666667 398643.2
109 398950.4
109.333333333333 398643.2
109.666666666667 403353.6
110 397312
110.333333333333 398028.8
110.666666666667 398540.8
111 398848
111.333333333333 395673.6
111.666666666667 395776
112 398438.4
112.333333333333 401920
112.666666666667 398438.4
113 397926.4
113.333333333333 398643.2
113.666666666667 398950.4
114 398643.2
114.333333333333 403353.6
114.666666666667 399257.6
115 399769.6
115.333333333333 397926.4
115.666666666667 398643.2
116 398950.4
116.333333333333 398643.2
116.666666666667 403353.6
117 397312
117.333333333333 398028.8
117.666666666667 398540.8
118 398848
118.333333333333 395673.6
118.666666666667 395264
119 396390.4
119.333333333333 399360
119.666666666667 398848
120 396288
120.333333333333 399052.8
120.666666666667 397926.4
121 398233.6
121.333333333333 399564.8
121.666666666667 399974.4
122 398540.8
122.333333333333 398131.2
122.666666666667 399667.2
123 397824
123.333333333333 402432
123.666666666667 399974.4
124 397516.8
124.333333333333 398028.8
124.666666666667 399257.6
125 396800
125.333333333333 395264
125.666666666667 396390.4
126 400998.4
126.333333333333 397312
126.666666666667 398028.8
127 398540.8
127.333333333333 398848
127.666666666667 395673.6
128 395776
128.333333333333 398438.4
128.666666666667 401920
129 397209.6
129.333333333333 395776
129.666666666667 396902.4
130 398848
130.333333333333 398336
130.666666666667 399564.8
131 399257.6
131.333333333333 399769.6
131.666666666667 397926.4
132 398643.2
132.333333333333 398950.4
132.666666666667 396800
133 395264
133.333333333333 395776
133.666666666667 398438.4
134 401920
134.333333333333 397209.6
134.666666666667 395776
135 396902.4
135.333333333333 398848
135.666666666667 398336
136 399564.8
136.333333333333 399257.6
136.666666666667 399769.6
137 397926.4
137.333333333333 398643.2
137.666666666667 398950.4
138 398643.2
138.333333333333 403353.6
138.666666666667 397312
139 398028.8
139.333333333333 401920
139.666666666667 399974.4
140 397516.8
140.333333333333 398028.8
140.666666666667 399257.6
141 396800
141.333333333333 395264
141.666666666667 395776
142 398028.8
142.333333333333 397414.4
142.666666666667 397414.4
143 397926.4
143.333333333333 397107.2
143.666666666667 397619.2
144 397004.8
144.333333333333 400588.8
144.666666666667 397926.4
145 397107.2
145.333333333333 397926.4
145.666666666667 399564.8
146 398950.4
146.333333333333 397926.4
146.666666666667 398643.2
147 398950.4
147.333333333333 398643.2
147.666666666667 403353.6
148 399257.6
148.333333333333 399769.6
148.666666666667 397926.4
149 398643.2
149.333333333333 398950.4
149.666666666667 398643.2
150 403353.6
150.333333333333 397312
150.666666666667 398028.8
151 398540.8
151.333333333333 398848
151.666666666667 395673.6
152 395264
152.333333333333 396390.4
152.666666666667 399257.6
153 399564.8
153.333333333333 399257.6
153.666666666667 399769.6
154 397926.4
154.333333333333 398643.2
154.666666666667 398950.4
155 398643.2
155.333333333333 403353.6
155.666666666667 399257.6
156 399769.6
156.333333333333 397926.4
156.666666666667 398643.2
157 398950.4
157.333333333333 398643.2
157.666666666667 403353.6
158 397312
158.333333333333 398028.8
158.666666666667 398540.8
159 398848
159.333333333333 396800
159.666666666667 397414.4
160 397414.4
160.333333333333 397926.4
160.666666666667 397107.2
161 397619.2
161.333333333333 397004.8
161.666666666667 400588.8
162 397926.4
162.333333333333 397107.2
162.666666666667 397926.4
163 399564.8
163.333333333333 397721.6
163.666666666667 398848
164 400793.6
164.333333333333 400691.2
164.666666666667 398336
165 398131.2
165.333333333333 398643.2
165.666666666667 403353.6
166 397721.6
166.333333333333 396185.6
166.666666666667 396288
167 399052.8
167.333333333333 397926.4
167.666666666667 399155.2
168 397414.4
168.333333333333 398540.8
168.666666666667 398848
169 395673.6
169.333333333333 395776
169.666666666667 398438.4
170 401920
170.333333333333 397209.6
170.666666666667 395776
171 396902.4
171.333333333333 398848
171.666666666667 398336
172 399564.8
172.333333333333 399257.6
172.666666666667 399974.4
173 399769.6
173.333333333333 397926.4
173.666666666667 398643.2
174 398950.4
174.333333333333 398643.2
174.666666666667 403353.6
175 399257.6
175.333333333333 399769.6
175.666666666667 397926.4
176 398643.2
176.333333333333 398950.4
176.666666666667 398643.2
177 403353.6
177.333333333333 397312
177.666666666667 398028.8
178 398540.8
178.333333333333 398848
178.666666666667 395673.6
179 395264
179.333333333333 398028.8
179.666666666667 397209.6
180 395776
180.333333333333 396902.4
180.666666666667 398848
181 398336
181.333333333333 399564.8
181.666666666667 399257.6
182 399769.6
182.333333333333 397926.4
182.666666666667 398643.2
183 398950.4
183.333333333333 398643.2
183.666666666667 402739.2
184 397926.4
184.333333333333 398233.6
184.666666666667 399564.8
185 399974.4
185.333333333333 398540.8
185.666666666667 398131.2
186 401817.6
186.333333333333 398438.4
186.666666666667 396185.6
187 396288
187.333333333333 399052.8
187.666666666667 397926.4
188 398233.6
188.333333333333 399564.8
188.666666666667 399974.4
189 398540.8
189.333333333333 398131.2
189.666666666667 399667.2
190 397824
190.333333333333 402432
190.666666666667 398848
191 398336
191.333333333333 399564.8
191.666666666667 399257.6
192 399769.6
192.333333333333 397926.4
192.666666666667 398028.8
193 399974.4
193.333333333333 398540.8
193.666666666667 398131.2
194 399667.2
194.333333333333 397824
194.666666666667 402432
195 399974.4
195.333333333333 397516.8
195.666666666667 398028.8
196 399257.6
196.333333333333 396800
196.666666666667 397004.8
197 397721.6
197.333333333333 398233.6
197.666666666667 397414.4
198 396185.6
198.333333333333 398745.6
198.666666666667 398131.2
199 399155.2
199.333333333333 398950.4
199.666666666667 398950.4
200 398643.2
200.333333333333 403353.6
200.666666666667 399257.6
201 399769.6
201.333333333333 397926.4
201.666666666667 398643.2
202 398950.4
202.333333333333 398643.2
202.666666666667 403353.6
203 397312
203.333333333333 398028.8
203.666666666667 398540.8
204 398848
204.333333333333 395673.6
204.666666666667 395264
205 398028.8
205.333333333333 397209.6
205.666666666667 395776
206 397209.6
206.333333333333 399974.4
206.666666666667 398540.8
207 398131.2
207.333333333333 399667.2
207.666666666667 397824
208 402432
208.333333333333 399974.4
208.666666666667 397516.8
209 398028.8
209.333333333333 399257.6
209.666666666667 396800
210 395264
210.333333333333 395776
210.666666666667 398438.4
211 396185.6
211.333333333333 396288
211.666666666667 399052.8
212 397926.4
212.333333333333 398233.6
212.666666666667 400281.6
213 397926.4
213.333333333333 398643.2
213.666666666667 398950.4
214 398643.2
214.333333333333 403353.6
214.666666666667 399257.6
215 399769.6
215.333333333333 397926.4
215.666666666667 398643.2
216 398950.4
216.333333333333 398643.2
216.666666666667 403353.6
217 397312
217.333333333333 398028.8
217.666666666667 398540.8
218 398848
218.333333333333 395673.6
218.666666666667 395264
219 398028.8
219.333333333333 398643.2
219.666666666667 396800
220 397004.8
220.333333333333 397721.6
220.666666666667 398233.6
221 397414.4
221.333333333333 396185.6
221.666666666667 398745.6
222 398131.2
222.333333333333 399155.2
222.666666666667 398028.8
223 396800
223.333333333333 399667.2
223.666666666667 398336
224 398233.6
224.333333333333 398950.4
224.666666666667 401920
225 399564.8
225.333333333333 397721.6
225.666666666667 397824
226 399052.8
226.333333333333 398848
226.666666666667 395673.6
227 395264
227.333333333333 398028.8
227.666666666667 397209.6
228 395776
228.333333333333 396902.4
228.666666666667 398848
229 398336
229.333333333333 399564.8
229.666666666667 399257.6
230 399769.6
230.333333333333 397926.4
230.666666666667 398643.2
231 398950.4
231.333333333333 398643.2
231.666666666667 402739.2
232 397926.4
232.333333333333 398233.6
232.666666666667 399052.8
233 398131.2
233.333333333333 399667.2
233.666666666667 397824
234 402432
234.333333333333 399974.4
234.666666666667 397516.8
235 398028.8
235.333333333333 399257.6
235.666666666667 396800
236 395264
236.333333333333 396390.4
236.666666666667 402227.2
237 398438.4
237.333333333333 396185.6
237.666666666667 396288
238 399052.8
238.333333333333 397926.4
238.666666666667 398233.6
239 399564.8
239.333333333333 399155.2
239.666666666667 398643.2
240 399667.2
240.333333333333 397209.6
240.666666666667 395776
241 396902.4
241.333333333333 398848
241.666666666667 398336
242 399564.8
242.333333333333 399257.6
242.666666666667 399769.6
243 397926.4
243.333333333333 398643.2
243.666666666667 398540.8
244 398336
244.333333333333 398540.8
244.666666666667 398848
245 397414.4
245.333333333333 398131.2
245.666666666667 398643.2
246 401612.8
246.333333333333 399564.8
246.666666666667 399257.6
247 399769.6
247.333333333333 397926.4
247.666666666667 398643.2
248 398950.4
248.333333333333 398643.2
248.666666666667 403353.6
249 397312
249.333333333333 398028.8
249.666666666667 398540.8
250 398848
250.333333333333 395673.6
250.666666666667 395776
251 398438.4
251.333333333333 399974.4
251.666666666667 397516.8
252 398028.8
252.333333333333 399257.6
252.666666666667 397619.2
253 396185.6
253.333333333333 398745.6
253.666666666667 398131.2
254 399155.2
254.333333333333 398950.4
254.666666666667 398950.4
255 398643.2
255.333333333333 403353.6
255.666666666667 399257.6
256 399769.6
256.333333333333 397926.4
256.666666666667 398643.2
257 398950.4
257.333333333333 398643.2
257.666666666667 403353.6
258 397312
258.333333333333 398028.8
258.666666666667 398540.8
259 398848
259.333333333333 397414.4
259.666666666667 398028.8
260 399257.6
260.333333333333 396800
260.666666666667 395264
261 395776
261.333333333333 398028.8
261.666666666667 397414.4
262 397414.4
262.333333333333 397926.4
262.666666666667 397107.2
263 397619.2
263.333333333333 397004.8
263.666666666667 400588.8
264 397926.4
264.333333333333 397107.2
264.666666666667 402227.2
265 398438.4
265.333333333333 396185.6
265.666666666667 396288
266 397926.4
266.333333333333 398643.2
266.666666666667 399667.2
267 397209.6
267.333333333333 395776
267.666666666667 396902.4
268 398848
268.333333333333 398336
268.666666666667 399564.8
269 399257.6
269.333333333333 399769.6
269.666666666667 397926.4
270 398643.2
270.333333333333 398950.4
270.666666666667 398643.2
271 403353.6
271.333333333333 397312
271.666666666667 398028.8
272 398540.8
272.333333333333 398848
272.666666666667 395673.6
273 395776
273.333333333333 398438.4
273.666666666667 396185.6
274 396288
274.333333333333 399257.6
274.666666666667 399769.6
275 397926.4
275.333333333333 398643.2
275.666666666667 398950.4
276 398643.2
276.333333333333 403353.6
276.666666666667 397312
277 398028.8
277.333333333333 398540.8
277.666666666667 398848
278 395673.6
278.333333333333 395264
278.666666666667 398028.8
279 397209.6
279.333333333333 396390.4
279.666666666667 399667.2
280 397824
280.333333333333 402432
280.666666666667 399974.4
281 399974.4
281.333333333333 398540.8
281.666666666667 398131.2
282 399667.2
282.333333333333 397824
282.666666666667 402432
283 399974.4
283.333333333333 397516.8
283.666666666667 398028.8
284 399257.6
284.333333333333 396800
284.666666666667 395264
285 395776
285.333333333333 398438.4
285.666666666667 396185.6
286 198246.4
};
\addlegendentry{\noFT}
\addplot [semithick, color2,mark=triangle*, mark size=2.0, mark options={solid,fill=white}, mark repeat=60,mark phase=45]
table {%
0 0
0.333333333333333 0
0.666666666666667 0
1 0
1.33333333333333 400486.4
1.66666666666667 402432
2 397312
2.33333333333333 397312
2.66666666666667 395980.8
3 394649.6
3.33333333333333 392499.2
3.66666666666667 391372.8
4 391884.8
4.33333333333333 392192
4.66666666666667 392601.6
5 392601.6
5.33333333333333 391270.4
5.66666666666667 387072
6 387584
6.33333333333333 387584
6.66666666666667 389939.2
7 388096
7.33333333333333 388096
7.66666666666667 389324.8
8 390348.8
8.33333333333333 390348.8
8.66666666666667 388300.8
9 388300.8
9.33333333333333 387993.6
9.66666666666667 385331.2
10 384819.2
10.3333333333333 385843.2
10.6666666666667 389427.2
11 382976
11.3333333333333 385740.8
11.6666666666667 385638.4
12 386355.2
12.3333333333333 384204.8
12.6666666666667 387276.8
13 387788.8
13.3333333333333 386560
13.6666666666667 383385.6
14 382464
14.3333333333333 384307.2
14.6666666666667 382873.6
15 383692.8
15.3333333333333 385740.8
15.6666666666667 386048
16 383180.8
16.3333333333333 381235.2
16.6666666666667 384409.6
17 382156.8
17.3333333333333 389734.4
17.6666666666667 382873.6
18 383180.8
18.3333333333333 380518.4
18.6666666666667 382054.4
19 382668.8
19.3333333333333 384716.8
19.6666666666667 385126.4
20 385331.2
20.3333333333333 386457.6
20.6666666666667 387379.2
21 383488
21.3333333333333 386252.8
21.6666666666667 382771.2
22 383692.8
22.3333333333333 383385.6
22.6666666666667 379801.6
23 381030.4
23.3333333333333 380928
23.6666666666667 383897.6
24 382976
24.3333333333333 386252.8
24.6666666666667 384716.8
25 385536
25.3333333333333 383590.4
25.6666666666667 383180.8
26 383283.2
26.3333333333333 382361.6
26.6666666666667 377651.2
27 380518.4
27.3333333333333 380518.4
27.6666666666667 382668.8
28 384512
28.3333333333333 381952
28.6666666666667 380211.2
29 381235.2
29.3333333333333 381849.6
29.6666666666667 381849.6
30 383692.8
30.3333333333333 383180.8
30.6666666666667 382259.2
31 385433.6
31.3333333333333 383488
31.6666666666667 380518.4
32 381542.4
32.3333333333333 383078.4
32.6666666666667 382668.8
33 386560
33.3333333333333 385945.6
33.6666666666667 385228.8
34 383590.4
34.3333333333333 383692.8
34.6666666666667 383692.8
35 382259.2
35.3333333333333 378880
35.6666666666667 379904
36 380928
36.3333333333333 382361.6
36.6666666666667 383488
37 381235.2
37.3333333333333 380006.4
37.6666666666667 381747.2
38 380723.2
38.3333333333333 381542.4
38.6666666666667 383897.6
39 385638.4
39.3333333333333 385126.4
39.6666666666667 385638.4
40 387993.6
40.3333333333333 383488
40.6666666666667 386252.8
41 382464
41.3333333333333 383488
41.6666666666667 383590.4
42 380006.4
42.3333333333333 381747.2
42.6666666666667 380928
43 384512
43.3333333333333 382976
43.6666666666667 385331.2
44 385638.4
44.3333333333333 385024
44.6666666666667 383795.2
45 383795.2
45.3333333333333 383488
45.6666666666667 381132.8
46 382464
46.3333333333333 383078.4
46.6666666666667 385024
47 385126.4
47.3333333333333 385638.4
47.6666666666667 385740.8
48 387686.4
48.3333333333333 383590.4
48.6666666666667 386662.4
49 382259.2
49.3333333333333 383897.6
49.6666666666667 383180.8
50 380211.2
50.3333333333333 382361.6
50.6666666666667 381030.4
51 383897.6
51.3333333333333 382361.6
51.6666666666667 385331.2
52 383897.6
52.3333333333333 382259.2
52.6666666666667 385536
53 384819.2
53.3333333333333 386969.6
53.6666666666667 383795.2
54 382976
54.3333333333333 382464
54.6666666666667 382464
55 380620.8
55.3333333333333 377958.4
55.6666666666667 379289.6
56 382771.2
56.3333333333333 382259.2
56.6666666666667 383692.8
57 379801.6
57.3333333333333 381644.8
57.6666666666667 380006.4
58 383385.6
58.3333333333333 381952
58.6666666666667 383590.4
59 379289.6
59.3333333333333 382771.2
59.6666666666667 380006.4
60 382361.6
60.3333333333333 383180.8
60.6666666666667 383385.6
61 381644.8
61.3333333333333 383488
61.6666666666667 385740.8
62 381132.8
62.3333333333333 380108.8
62.6666666666667 384102.4
63 381542.4
63.3333333333333 385536
63.6666666666667 384614.4
64 386457.6
64.3333333333333 383590.4
64.6666666666667 383590.4
65 383488
65.3333333333333 387584
65.6666666666667 383897.6
66 387584
66.3333333333333 382771.2
66.6666666666667 383488
67 383283.2
67.3333333333333 380211.2
67.6666666666667 381542.4
68 380416
68.3333333333333 383590.4
68.6666666666667 382566.4
69 386764.8
69.3333333333333 385126.4
69.6666666666667 384716.8
70 383692.8
70.3333333333333 384204.8
70.6666666666667 383590.4
71 381030.4
71.3333333333333 382668.8
71.6666666666667 381337.6
72 385331.2
72.3333333333333 385228.8
72.6666666666667 386969.6
73 385331.2
73.3333333333333 383692.8
73.6666666666667 384102.4
74 382259.2
74.3333333333333 383897.6
74.6666666666667 381542.4
75 381644.8
75.3333333333333 382156.8
75.6666666666667 383795.2
76 381849.6
76.3333333333333 385433.6
76.6666666666667 384204.8
77 386457.6
77.3333333333333 383488
77.6666666666667 383283.2
78 382566.4
78.3333333333333 381542.4
78.6666666666667 382771.2
79 382566.4
79.3333333333333 380825.6
79.6666666666667 381849.6
80 381747.2
80.3333333333333 384204.8
80.6666666666667 385024
81 385843.2
81.3333333333333 386150.4
81.6666666666667 387276.8
82 383897.6
82.3333333333333 386048
82.6666666666667 383078.4
83 383795.2
83.3333333333333 382771.2
83.6666666666667 381337.6
84 381849.6
84.3333333333333 381235.2
84.6666666666667 384307.2
85 381849.6
85.3333333333333 382873.6
85.6666666666667 385228.8
86 385433.6
86.3333333333333 385126.4
86.6666666666667 383692.8
87 383692.8
87.3333333333333 383180.8
87.6666666666667 381440
88 382156.8
88.3333333333333 381849.6
88.6666666666667 385024
89 386048
89.3333333333333 386969.6
89.6666666666667 385536
90 383897.6
90.3333333333333 383897.6
90.6666666666667 383283.2
91 384102.4
91.3333333333333 380108.8
91.6666666666667 381542.4
92 378265.6
92.3333333333333 380006.4
92.6666666666667 382566.4
93 382464
93.3333333333333 383488
93.6666666666667 378982.4
94 381337.6
94.3333333333333 380518.4
94.6666666666667 382464
95 382156.8
95.3333333333333 385126.4
95.6666666666667 382054.4
96 383795.2
96.3333333333333 385536
96.6666666666667 382464
97 380313.6
97.3333333333333 383897.6
97.6666666666667 381132.8
98 385843.2
98.3333333333333 384716.8
98.6666666666667 382771.2
99 382566.4
99.3333333333333 384204.8
99.6666666666667 381952
100 382873.6
100.333333333333 385536
100.666666666667 381644.8
101 379494.4
101.333333333333 384102.4
101.666666666667 380825.6
102 385945.6
102.333333333333 384307.2
102.666666666667 385536
103 383590.4
103.333333333333 382771.2
103.666666666667 382566.4
104 382771.2
104.333333333333 380825.6
104.666666666667 378982.4
105 380723.2
105.333333333333 383897.6
105.666666666667 382566.4
106 385740.8
106.333333333333 383488
106.666666666667 381644.8
107 385536
107.333333333333 385024
107.666666666667 386969.6
108 384000
108.333333333333 383385.6
108.666666666667 382771.2
109 381952
109.333333333333 381337.6
109.666666666667 378572.8
110 380108.8
110.333333333333 383078.4
110.666666666667 381849.6
111 383692.8
111.333333333333 379494.4
111.666666666667 382259.2
112 384307.2
112.333333333333 381235.2
112.666666666667 384921.6
113 384000
113.333333333333 384409.6
113.666666666667 383078.4
114 386457.6
114.333333333333 385024
114.666666666667 385228.8
115 384102.4
115.333333333333 383488
115.666666666667 382668.8
116 381542.4
116.333333333333 378163.2
116.666666666667 380108.8
117 379494.4
117.333333333333 382259.2
117.666666666667 382464
118 381440
118.333333333333 380108.8
118.666666666667 382771.2
119 385331.2
119.333333333333 385126.4
119.666666666667 387174.4
120 383795.2
120.333333333333 383283.2
120.666666666667 383078.4
121 382259.2
121.333333333333 383078.4
121.666666666667 382259.2
122 380416
122.333333333333 381952
122.666666666667 382361.6
123 384614.4
123.333333333333 384921.6
123.666666666667 386048
124 386560
124.333333333333 387174.4
124.666666666667 383385.6
125 386662.4
125.333333333333 383590.4
125.666666666667 380620.8
126 382464
126.333333333333 382054.4
126.666666666667 386867.2
127 385638.4
127.333333333333 386969.6
127.666666666667 385433.6
128 383897.6
128.333333333333 384512
128.666666666667 382668.8
129 384102.4
129.333333333333 380620.8
129.666666666667 380108.8
130 378060.8
130.333333333333 379699.2
130.666666666667 383488
131 382054.4
131.333333333333 383180.8
131.666666666667 380620.8
132 385740.8
132.333333333333 384512
132.666666666667 384512
133 383180.8
133.333333333333 384102.4
133.666666666667 381132.8
134 380313.6
134.333333333333 380825.6
134.666666666667 384102.4
135 381644.8
135.333333333333 385433.6
135.666666666667 384512
136 386560
136.333333333333 384307.2
136.666666666667 382771.2
137 383283.2
137.333333333333 382259.2
137.666666666667 382976
138 382668.8
138.333333333333 381030.4
138.666666666667 380620.8
139 382976
139.333333333333 382668.8
139.666666666667 381644.8
140 382771.2
140.333333333333 383590.4
140.666666666667 386457.6
141 383385.6
141.333333333333 383795.2
141.666666666667 383897.6
142 380313.6
142.333333333333 381849.6
142.666666666667 381440
143 384204.8
143.333333333333 382771.2
143.666666666667 386355.2
144 385536
144.333333333333 385228.8
144.666666666667 382873.6
145 383488
145.333333333333 382259.2
145.666666666667 383078.4
146 386457.6
146.333333333333 384921.6
146.666666666667 384819.2
147 384000
147.333333333333 383078.4
147.666666666667 383180.8
148 382259.2
148.333333333333 382771.2
148.666666666667 382873.6
149 381849.6
149.333333333333 381030.4
149.666666666667 383795.2
150 384512
150.333333333333 386457.6
150.666666666667 385740.8
151 386764.8
151.333333333333 385228.8
151.666666666667 382464
152 384921.6
152.333333333333 380211.2
152.666666666667 379801.6
153 380620.8
153.333333333333 383692.8
153.666666666667 382054.4
154 384921.6
154.333333333333 384204.8
154.666666666667 384204.8
155 382668.8
155.333333333333 385536
155.666666666667 385638.4
156 384409.6
156.333333333333 383795.2
156.666666666667 383692.8
157 383180.8
157.333333333333 382054.4
157.666666666667 377753.6
158 379904
158.333333333333 380825.6
158.666666666667 382976
159 383078.4
159.333333333333 382873.6
159.666666666667 382873.6
160 382976
160.333333333333 380108.8
160.666666666667 380006.4
161 382771.2
161.333333333333 383692.8
161.666666666667 381132.8
162 382361.6
162.333333333333 383897.6
162.666666666667 386662.4
163 382873.6
163.333333333333 383488
163.666666666667 383180.8
164 379392
164.333333333333 381542.4
164.666666666667 381132.8
165 383385.6
165.333333333333 385638.4
165.666666666667 385536
166 386560
166.333333333333 385228.8
166.666666666667 384307.2
167 384000
167.333333333333 380211.2
167.666666666667 380518.4
168 381952
168.333333333333 384409.6
168.666666666667 381747.2
169 385433.6
169.333333333333 383795.2
169.666666666667 384409.6
170 382156.8
170.333333333333 385740.8
170.666666666667 385126.4
171 385126.4
171.333333333333 383488
171.666666666667 382668.8
172 380620.8
172.333333333333 380620.8
172.666666666667 381337.6
173 383692.8
173.333333333333 382361.6
173.666666666667 385024
174 385126.4
174.333333333333 386662.4
174.666666666667 383795.2
175 382566.4
175.333333333333 383283.2
175.666666666667 383078.4
176 381030.4
176.333333333333 380928
176.666666666667 383283.2
177 385536
177.333333333333 386457.6
177.666666666667 386355.2
178 386457.6
178.333333333333 385740.8
178.666666666667 378982.4
179 383180.8
179.333333333333 382361.6
179.666666666667 382464
180 380211.2
180.333333333333 385945.6
180.666666666667 383692.8
181 384512
181.333333333333 383078.4
181.666666666667 384204.8
182 380416
182.333333333333 380108.8
182.666666666667 381644.8
183 383385.6
183.333333333333 383795.2
183.666666666667 385024
184 385536
184.333333333333 387072
184.666666666667 383590.4
185 384614.4
185.333333333333 383897.6
185.666666666667 385536
186 383692.8
186.333333333333 383488
186.666666666667 383385.6
187 382464
187.333333333333 380825.6
187.666666666667 377651.2
188 379904
188.333333333333 383078.4
188.666666666667 381952
189 383283.2
189.333333333333 378675.2
189.666666666667 381235.2
190 380006.4
190.333333333333 383692.8
190.666666666667 382464
191 383897.6
191.333333333333 379596.8
191.666666666667 381747.2
192 387891.2
192.333333333333 385126.4
192.666666666667 385536
193 385843.2
193.333333333333 389120
193.666666666667 382771.2
194 385331.2
194.333333333333 386048
194.666666666667 386969.6
195 383385.6
195.333333333333 387072
195.666666666667 387276.8
196 386764.8
196.333333333333 383488
196.666666666667 381542.4
197 384512
197.333333333333 382259.2
197.666666666667 383692.8
198 385740.8
198.333333333333 385945.6
198.666666666667 385740.8
199 383897.6
199.333333333333 383590.4
199.666666666667 383078.4
200 381747.2
200.333333333333 377651.2
200.666666666667 380723.2
201 380825.6
201.333333333333 382771.2
201.666666666667 382464
202 381542.4
202.333333333333 380108.8
202.666666666667 382361.6
203 381747.2
203.333333333333 381235.2
203.666666666667 383283.2
204 381952
204.333333333333 380723.2
204.666666666667 385024
205 386560
205.333333333333 386560
205.666666666667 384204.8
206 382771.2
206.333333333333 383692.8
206.666666666667 382464
207 380825.6
207.333333333333 378368
207.666666666667 380108.8
208 382976
208.333333333333 381337.6
208.666666666667 383283.2
209 378368
209.333333333333 381747.2
209.666666666667 384614.4
210 381644.8
210.333333333333 385536
210.666666666667 384409.6
211 384819.2
211.333333333333 382873.6
211.666666666667 386150.4
212 382771.2
212.333333333333 383180.8
212.666666666667 383078.4
213 380006.4
213.333333333333 378265.6
213.666666666667 380108.8
214 379904
214.333333333333 382771.2
214.666666666667 383180.8
215 381952
215.333333333333 381952
215.666666666667 384000
216 386662.4
216.333333333333 382873.6
216.666666666667 383590.4
217 383795.2
217.333333333333 379596.8
217.666666666667 381644.8
218 381030.4
218.333333333333 383795.2
218.666666666667 382668.8
219 383385.6
219.333333333333 378982.4
219.666666666667 382156.8
220 380211.2
220.333333333333 382668.8
220.666666666667 382976
221 384102.4
221.333333333333 379187.2
221.666666666667 381440
222 387584
222.333333333333 385740.8
222.666666666667 385024
223 384307.2
223.333333333333 383180.8
223.666666666667 382361.6
224 381644.8
224.333333333333 378880
224.666666666667 380518.4
225 380825.6
225.333333333333 381132.8
225.666666666667 382668.8
226 382259.2
226.333333333333 386252.8
226.666666666667 386662.4
227 386764.8
227.333333333333 386048
227.666666666667 384307.2
228 385228.8
228.333333333333 383897.6
228.666666666667 383897.6
229 380518.4
229.333333333333 380620.8
229.666666666667 378368
230 380518.4
230.333333333333 383590.4
230.666666666667 381747.2
231 384512
231.333333333333 380006.4
231.666666666667 382668.8
232 383488
232.333333333333 384512
232.666666666667 383078.4
233 383078.4
233.333333333333 381030.4
233.666666666667 380518.4
234 380518.4
234.333333333333 383897.6
234.666666666667 383897.6
235 385843.2
235.333333333333 386150.4
235.666666666667 388096
236 383283.2
236.333333333333 384512
236.666666666667 383180.8
237 379904
237.333333333333 381132.8
237.666666666667 380518.4
238 383692.8
238.333333333333 382771.2
238.666666666667 380108.8
239 383385.6
239.333333333333 383897.6
239.666666666667 381849.6
240 380518.4
240.333333333333 382464
240.666666666667 385126.4
241 384716.8
241.333333333333 387072
241.666666666667 384409.6
242 383385.6
242.333333333333 382771.2
242.666666666667 382464
243 382464
243.333333333333 383795.2
243.666666666667 380928
244 382976
244.333333333333 381952
244.666666666667 384512
245 385024
245.333333333333 384614.4
245.666666666667 382771.2
246 379596.8
246.333333333333 381849.6
246.666666666667 381542.4
247 384512
247.333333333333 382668.8
247.666666666667 380416
248 383692.8
248.333333333333 383488
248.666666666667 380518.4
249 380211.2
249.333333333333 381440
249.666666666667 385536
250 385433.6
250.333333333333 386355.2
250.666666666667 383795.2
251 383385.6
251.333333333333 383692.8
251.666666666667 382361.6
252 380723.2
252.333333333333 380928
252.666666666667 381849.6
253 383795.2
253.333333333333 381747.2
253.666666666667 385638.4
254 384409.6
254.333333333333 386355.2
254.666666666667 384307.2
255 383590.4
255.333333333333 383283.2
255.666666666667 381747.2
256 386150.4
256.333333333333 384716.8
256.666666666667 386867.2
257 383897.6
257.333333333333 383180.8
257.666666666667 383283.2
258 381849.6
258.333333333333 382668.8
258.666666666667 382259.2
259 381132.8
259.333333333333 384000
259.666666666667 382976
260 385740.8
260.333333333333 385433.6
260.666666666667 384409.6
261 383692.8
261.333333333333 383897.6
261.666666666667 382566.4
262 380211.2
262.333333333333 381235.2
262.666666666667 382156.8
263 384512
263.333333333333 385228.8
263.666666666667 385843.2
264 386150.4
264.333333333333 387788.8
264.666666666667 382771.2
265 386662.4
265.333333333333 382361.6
265.666666666667 380416
266 384204.8
266.333333333333 385945.6
266.666666666667 385638.4
267 386969.6
267.333333333333 385433.6
267.666666666667 383180.8
268 384819.2
268.333333333333 384921.6
268.666666666667 385228.8
269 384000
269.333333333333 382873.6
269.666666666667 382873.6
270 381849.6
270.333333333333 378572.8
270.666666666667 379801.6
271 380928
271.333333333333 383283.2
271.666666666667 383078.4
272 383590.4
272.333333333333 385843.2
272.666666666667 385126.4
273 383590.4
273.333333333333 384921.6
273.666666666667 382771.2
274 384307.2
274.333333333333 380723.2
274.666666666667 380416
275 381644.8
275.333333333333 383590.4
275.666666666667 381542.4
276 385433.6
276.333333333333 384819.2
276.666666666667 385843.2
277 384614.4
277.333333333333 382259.2
277.666666666667 383590.4
278 383590.4
278.333333333333 381440
278.666666666667 379699.2
279 382464
279.333333333333 382668.8
279.666666666667 386457.6
280 385433.6
280.333333333333 384819.2
280.666666666667 383590.4
281 383692.8
281.333333333333 383488
281.666666666667 382361.6
282 382976
282.333333333333 382566.4
282.666666666667 381440
283 381030.4
283.333333333333 382976
283.666666666667 385024
284 386048
284.333333333333 384000
284.666666666667 380211.2
285 381132.8
};
\addlegendentry{\sysKFour}
\addplot [semithick, color1, mark=*, mark size=1.5, mark options={solid,fill=white}, mark repeat=60,mark phase=30]
table {%
0 160358.4
0.333333333333333 331776
0.666666666666667 400998.4
1 401510.4
1.33333333333333 400588.8
1.66666666666667 399462.4
2 398028.8
2.33333333333333 398233.6
2.66666666666667 398745.6
3 398848
3.33333333333333 398336
3.66666666666667 400076.8
4 398540.8
4.33333333333333 397721.6
4.66666666666667 399155.2
5 397824
5.33333333333333 399155.2
5.66666666666667 395673.6
6 399155.2
6.33333333333333 397516.8
6.66666666666667 398745.6
7 399462.4
7.33333333333333 398233.6
7.66666666666667 396902.4
8 399667.2
8.33333333333333 397926.4
8.66666666666667 398028.8
9 397516.8
9.33333333333333 398848
9.66666666666667 397209.6
10 396902.4
10.3333333333333 397619.2
10.6666666666667 398233.6
11 398848
11.3333333333333 398028.8
11.6666666666667 397516.8
12 397926.4
12.3333333333333 396595.2
12.6666666666667 397414.4
13 398028.8
13.3333333333333 398233.6
13.6666666666667 399155.2
14 397824
14.3333333333333 397107.2
14.6666666666667 397516.8
15 395264
15.3333333333333 397209.6
15.6666666666667 396492.8
16 397926.4
16.3333333333333 396185.6
16.6666666666667 397004.8
17 399052.8
17.3333333333333 397414.4
17.6666666666667 397721.6
18 397926.4
18.3333333333333 397107.2
18.6666666666667 398233.6
19 397721.6
19.3333333333333 397824
19.6666666666667 396492.8
20 396390.4
20.3333333333333 397721.6
20.6666666666667 397721.6
21 397926.4
21.3333333333333 397516.8
21.6666666666667 398643.2
22 397926.4
22.3333333333333 398131.2
22.6666666666667 397209.6
23 397004.8
23.3333333333333 398336
23.6666666666667 396595.2
24 397312
24.3333333333333 397926.4
24.6666666666667 397619.2
25 398336
25.3333333333333 396492.8
25.6666666666667 397824
26 398438.4
26.3333333333333 397926.4
26.6666666666667 397619.2
27 396492.8
27.3333333333333 398131.2
27.6666666666667 397926.4
28 397721.6
28.3333333333333 397824
28.6666666666667 398643.2
29 397414.4
29.3333333333333 398028.8
29.6666666666667 397414.4
30 397926.4
30.3333333333333 199168
30.6666666666667 0
31 0
31.3333333333333 0
31.6666666666667 0
32 0
32.3333333333333 0
32.6666666666667 0
33 0
33.3333333333333 0
33.6666666666667 0
34 0
34.3333333333333 0
34.6666666666667 0
35 0
35.3333333333333 0
35.6666666666667 0
36 0
36.3333333333333 0
36.6666666666667 0
37 0
37.3333333333333 0
37.6666666666667 0
38 0
38.3333333333333 0
38.6666666666667 0
39 0
39.3333333333333 0
39.6666666666667 0
40 199372.8
40.3333333333333 397619.2
40.6666666666667 397209.6
41 397209.6
41.3333333333333 397414.4
41.6666666666667 397926.4
42 397312
42.3333333333333 398745.6
42.6666666666667 396800
43 397107.2
43.3333333333333 397414.4
43.6666666666667 399155.2
44 399257.6
44.3333333333333 398848
44.6666666666667 396288
45 396185.6
45.3333333333333 396902.4
45.6666666666667 398540.8
46 397721.6
46.3333333333333 397721.6
46.6666666666667 398131.2
47 397824
47.3333333333333 397824
47.6666666666667 397414.4
48 398233.6
48.3333333333333 398233.6
48.6666666666667 396697.6
49 398438.4
49.3333333333333 397721.6
49.6666666666667 397516.8
50 397312
50.3333333333333 398540.8
50.6666666666667 398643.2
51 397619.2
51.3333333333333 397619.2
51.6666666666667 398336
52 398131.2
52.3333333333333 397004.8
52.6666666666667 396492.8
53 398438.4
53.3333333333333 397312
53.6666666666667 396083.2
54 397312
54.3333333333333 398233.6
54.6666666666667 397107.2
55 397721.6
55.3333333333333 397414.4
55.6666666666667 397107.2
56 397926.4
56.3333333333333 398643.2
56.6666666666667 397824
57 397312
57.3333333333333 398233.6
57.6666666666667 397926.4
58 397209.6
58.3333333333333 399462.4
58.6666666666667 396697.6
59 397312
59.3333333333333 396288
59.6666666666667 397414.4
60 397312
60.3333333333333 397619.2
60.6666666666667 396800
61 396492.8
61.3333333333333 397619.2
61.6666666666667 398028.8
62 397824
62.3333333333333 397619.2
62.6666666666667 396800
63 395673.6
63.3333333333333 397926.4
63.6666666666667 396902.4
64 397414.4
64.3333333333333 398028.8
64.6666666666667 396595.2
65 398028.8
65.3333333333333 397312
65.6666666666667 399155.2
66 398131.2
66.3333333333333 398848
66.6666666666667 397824
67 399257.6
67.3333333333333 398438.4
67.6666666666667 397824
68 397926.4
68.3333333333333 398131.2
68.6666666666667 397414.4
69 395468.8
69.3333333333333 399052.8
69.6666666666667 397004.8
70 397516.8
70.3333333333333 399462.4
70.6666666666667 0
71 0
71.3333333333333 0
71.6666666666667 0
72 0
72.3333333333333 0
72.6666666666667 0
73 0
73.3333333333333 0
73.6666666666667 0
74 0
74.3333333333333 0
74.6666666666667 0
75 0
75.3333333333333 0
75.6666666666667 0
76 0
76.3333333333333 0
76.6666666666667 0
77 0
77.3333333333333 0
77.6666666666667 0
78 0
78.3333333333333 0
78.6666666666667 0
79 0
79.3333333333333 0
79.6666666666667 0
80 0
80.3333333333333 198656
80.6666666666667 398131.2
81 396595.2
81.3333333333333 397721.6
81.6666666666667 397209.6
82 396697.6
82.3333333333333 397824
82.6666666666667 397824
83 396902.4
83.3333333333333 398950.4
83.6666666666667 396492.8
84 397004.8
84.3333333333333 397516.8
84.6666666666667 397312
85 397926.4
85.3333333333333 396083.2
85.6666666666667 397414.4
86 398540.8
86.3333333333333 396697.6
86.6666666666667 397107.2
87 397824
87.3333333333333 399257.6
87.6666666666667 398028.8
88 398745.6
88.3333333333333 398233.6
88.6666666666667 397926.4
89 396800
89.3333333333333 396800
89.6666666666667 397312
90 397516.8
90.3333333333333 396595.2
90.6666666666667 397107.2
91 397107.2
91.3333333333333 396492.8
91.6666666666667 397107.2
92 396390.4
92.3333333333333 397721.6
92.6666666666667 397107.2
93 397312
93.3333333333333 397312
93.6666666666667 396697.6
94 397926.4
94.3333333333333 397516.8
94.6666666666667 398028.8
95 398438.4
95.3333333333333 396902.4
95.6666666666667 399769.6
96 399564.8
96.3333333333333 399155.2
96.6666666666667 398336
97 397209.6
97.3333333333333 397619.2
97.6666666666667 396902.4
98 398643.2
98.3333333333333 398233.6
98.6666666666667 397516.8
99 397721.6
99.3333333333333 397414.4
99.6666666666667 398131.2
100 398643.2
100.333333333333 398233.6
100.666666666667 398233.6
101 397414.4
101.333333333333 398233.6
101.666666666667 397107.2
102 397516.8
102.333333333333 397619.2
102.666666666667 397926.4
103 397721.6
103.333333333333 397824
103.666666666667 398028.8
104 396800
104.333333333333 396697.6
104.666666666667 397107.2
105 395673.6
105.333333333333 398438.4
105.666666666667 396697.6
106 397926.4
106.333333333333 398540.8
106.666666666667 396697.6
107 397926.4
107.333333333333 397107.2
107.666666666667 399257.6
108 398131.2
108.333333333333 398438.4
108.666666666667 398233.6
109 398745.6
109.333333333333 398848
109.666666666667 397619.2
110 397824
110.333333333333 397926.4
110.666666666667 397824
111 0
111.333333333333 0
111.666666666667 0
112 0
112.333333333333 0
112.666666666667 0
113 0
113.333333333333 0
113.666666666667 0
114 0
114.333333333333 0
114.666666666667 0
115 0
115.333333333333 0
115.666666666667 0
116 0
116.333333333333 0
116.666666666667 0
117 0
117.333333333333 0
117.666666666667 0
118 0
118.333333333333 0
118.666666666667 0
119 0
119.333333333333 0
119.666666666667 0
120 0
120.333333333333 0
120.666666666667 0
121 0
121.333333333333 0
121.666666666667 197939.2
122 397926.4
122.333333333333 397516.8
122.666666666667 397209.6
123 397516.8
123.333333333333 396902.4
123.666666666667 397209.6
124 396595.2
124.333333333333 397926.4
124.666666666667 399155.2
125 397516.8
125.333333333333 397516.8
125.666666666667 396800
126 398028.8
126.333333333333 396902.4
126.666666666667 398643.2
127 397619.2
127.333333333333 397824
127.666666666667 396390.4
128 397721.6
128.333333333333 398336
128.666666666667 398745.6
129 398438.4
129.333333333333 395980.8
129.666666666667 397516.8
130 396697.6
130.333333333333 398028.8
130.666666666667 397209.6
131 398745.6
131.333333333333 398540.8
131.666666666667 397516.8
132 397209.6
132.333333333333 398131.2
132.666666666667 397824
133 397516.8
133.333333333333 397209.6
133.666666666667 398438.4
134 398131.2
134.333333333333 398028.8
134.666666666667 398336
135 396697.6
135.333333333333 398028.8
135.666666666667 396595.2
136 397824
136.333333333333 397312
136.666666666667 398540.8
137 397619.2
137.333333333333 397312
137.666666666667 397721.6
138 398028.8
138.333333333333 398745.6
138.666666666667 398028.8
139 397209.6
139.333333333333 396902.4
139.666666666667 398643.2
140 396595.2
140.333333333333 398131.2
140.666666666667 396697.6
141 397004.8
141.333333333333 398336
141.666666666667 396800
142 398848
142.333333333333 398438.4
142.666666666667 399564.8
143 397619.2
143.333333333333 397004.8
143.666666666667 397516.8
144 396902.4
144.333333333333 398336
144.666666666667 396697.6
145 397516.8
145.333333333333 397926.4
145.666666666667 397414.4
146 397721.6
146.333333333333 398540.8
146.666666666667 397516.8
147 397414.4
147.333333333333 396697.6
147.666666666667 397209.6
148 399155.2
148.333333333333 397312
148.666666666667 397721.6
149 398336
149.333333333333 397926.4
149.666666666667 397004.8
150 398438.4
150.333333333333 397721.6
150.666666666667 397414.4
151 398233.6
151.333333333333 397107.2
151.666666666667 397312
152 397414.4
152.333333333333 198144
152.666666666667 0
153 0
153.333333333333 0
153.666666666667 0
154 0
154.333333333333 0
154.666666666667 0
155 0
155.333333333333 0
155.666666666667 0
156 0
156.333333333333 0
156.666666666667 0
157 0
157.333333333333 0
157.666666666667 0
158 0
158.333333333333 0
158.666666666667 0
159 0
159.333333333333 0
159.666666666667 0
160 0
160.333333333333 0
160.666666666667 0
161 0
161.333333333333 0
161.666666666667 397619.2
162 397312
162.333333333333 397721.6
162.666666666667 397209.6
163 397824
163.333333333333 397107.2
163.666666666667 395980.8
164 398233.6
164.333333333333 396800
164.666666666667 397414.4
165 397619.2
165.333333333333 396595.2
165.666666666667 396902.4
166 397619.2
166.333333333333 398233.6
166.666666666667 397824
167 398643.2
167.333333333333 397721.6
167.666666666667 399052.8
168 398745.6
168.333333333333 397209.6
168.666666666667 398028.8
169 396595.2
169.333333333333 397414.4
169.666666666667 398028.8
170 397312
170.333333333333 396390.4
170.666666666667 397824
171 397107.2
171.333333333333 397414.4
171.666666666667 398848
172 397516.8
172.333333333333 397824
172.666666666667 397004.8
173 398233.6
173.333333333333 397619.2
173.666666666667 398028.8
174 395776
174.333333333333 398540.8
174.666666666667 397619.2
175 397209.6
175.333333333333 396083.2
175.666666666667 397926.4
176 397926.4
176.333333333333 397312
176.666666666667 398540.8
177 396902.4
177.333333333333 397004.8
177.666666666667 396902.4
178 399257.6
178.333333333333 397516.8
178.666666666667 398233.6
179 398028.8
179.333333333333 398848
179.666666666667 398438.4
180 398438.4
180.333333333333 397926.4
180.666666666667 398848
181 397414.4
181.333333333333 396390.4
181.666666666667 398028.8
182 397824
182.333333333333 396902.4
182.666666666667 398131.2
183 397721.6
183.333333333333 397312
183.666666666667 398131.2
184 396595.2
184.333333333333 397721.6
184.666666666667 398131.2
185 398233.6
185.333333333333 397312
185.666666666667 397926.4
186 398131.2
186.333333333333 397619.2
186.666666666667 397209.6
187 399257.6
187.333333333333 397721.6
187.666666666667 396288
188 398438.4
188.333333333333 398028.8
188.666666666667 397414.4
189 398336
189.333333333333 398028.8
189.666666666667 397414.4
190 398028.8
190.333333333333 397004.8
190.666666666667 396595.2
191 398028.8
191.333333333333 398028.8
191.666666666667 397107.2
192 198656
192.333333333333 0
192.666666666667 0
193 0
193.333333333333 0
193.666666666667 0
194 0
194.333333333333 0
194.666666666667 0
195 0
195.333333333333 0
195.666666666667 0
196 0
196.333333333333 0
196.666666666667 0
197 0
197.333333333333 0
197.666666666667 0
198 0
198.333333333333 0
198.666666666667 0
199 0
199.333333333333 0
199.666666666667 0
200 0
200.333333333333 0
200.666666666667 0
201 0
201.333333333333 0
201.666666666667 0
202 0
202.333333333333 199577.6
202.666666666667 398540.8
203 397721.6
203.333333333333 396697.6
203.666666666667 399360
204 397824
204.333333333333 397312
204.666666666667 398540.8
205 397516.8
205.333333333333 396492.8
205.666666666667 398131.2
206 397209.6
206.333333333333 397107.2
206.666666666667 397312
207 398131.2
207.333333333333 397721.6
207.666666666667 398131.2
208 399974.4
208.333333333333 397926.4
208.666666666667 397926.4
209 398131.2
209.333333333333 398643.2
209.666666666667 397721.6
210 395980.8
210.333333333333 398028.8
210.666666666667 397824
211 396697.6
211.333333333333 397619.2
211.666666666667 397824
212 397312
212.333333333333 397414.4
212.666666666667 396902.4
213 398540.8
213.333333333333 397209.6
213.666666666667 397926.4
214 397312
214.333333333333 399360
214.666666666667 398848
215 397926.4
215.333333333333 399155.2
215.666666666667 398028.8
216 400179.2
216.333333333333 397619.2
216.666666666667 396800
217 397721.6
217.333333333333 397107.2
217.666666666667 397619.2
218 397312
218.333333333333 396800
218.666666666667 398028.8
219 397619.2
219.333333333333 398028.8
219.666666666667 397619.2
220 397824
220.333333333333 397824
220.666666666667 397516.8
221 398028.8
221.333333333333 396390.4
221.666666666667 397414.4
222 397516.8
222.333333333333 397619.2
222.666666666667 397824
223 398950.4
223.333333333333 399462.4
223.666666666667 397414.4
224 399462.4
224.333333333333 398745.6
224.666666666667 398848
225 397619.2
225.333333333333 397107.2
225.666666666667 397824
226 397414.4
226.333333333333 398438.4
226.666666666667 397721.6
227 397004.8
227.333333333333 395980.8
227.666666666667 396800
228 397209.6
228.333333333333 398028.8
228.666666666667 396697.6
229 397414.4
229.333333333333 397107.2
229.666666666667 397004.8
230 397209.6
230.333333333333 397824
230.666666666667 397004.8
231 397209.6
231.333333333333 397619.2
231.666666666667 396492.8
232 396902.4
232.333333333333 397004.8
232.666666666667 397619.2
233 0
233.333333333333 0
233.666666666667 0
234 0
234.333333333333 0
234.666666666667 0
235 0
235.333333333333 0
235.666666666667 0
236 0
236.333333333333 0
236.666666666667 0
237 0
237.333333333333 0
237.666666666667 0
238 0
238.333333333333 0
238.666666666667 0
239 0
239.333333333333 0
239.666666666667 0
240 0
240.333333333333 0
240.666666666667 0
241 0
241.333333333333 0
241.666666666667 0
242 0
242.333333333333 0
242.666666666667 0
243 0
243.333333333333 199782.4
243.666666666667 398336
244 399052.8
244.333333333333 398745.6
244.666666666667 397209.6
245 399360
245.333333333333 398233.6
245.666666666667 397619.2
246 396902.4
246.333333333333 397107.2
246.666666666667 397107.2
247 397516.8
247.333333333333 397004.8
247.666666666667 399257.6
248 398131.2
248.333333333333 398438.4
248.666666666667 397209.6
249 396902.4
249.333333333333 397004.8
249.666666666667 397107.2
250 396697.6
250.333333333333 398950.4
250.666666666667 397209.6
251 396800
251.333333333333 399155.2
251.666666666667 398438.4
252 399462.4
252.333333333333 398336
252.666666666667 396697.6
253 398028.8
253.333333333333 397107.2
253.666666666667 396492.8
254 398438.4
254.333333333333 395980.8
254.666666666667 397107.2
255 398745.6
255.333333333333 397516.8
255.666666666667 396390.4
256 399052.8
256.333333333333 397209.6
256.666666666667 396902.4
257 399052.8
257.333333333333 397516.8
257.666666666667 397926.4
258 397107.2
258.333333333333 397414.4
258.666666666667 396902.4
259 396902.4
259.333333333333 399564.8
259.666666666667 397721.6
260 398848
260.333333333333 398028.8
260.666666666667 397107.2
261 398233.6
261.333333333333 397414.4
261.666666666667 397926.4
262 396697.6
262.333333333333 397004.8
262.666666666667 397721.6
263 397414.4
263.333333333333 397824
263.666666666667 396595.2
264 398131.2
264.333333333333 397926.4
264.666666666667 395878.4
265 397721.6
265.333333333333 397107.2
265.666666666667 396492.8
266 397312
266.333333333333 397414.4
266.666666666667 397209.6
267 396800
267.333333333333 398336
267.666666666667 399155.2
268 397516.8
268.333333333333 398028.8
268.666666666667 396595.2
269 397004.8
269.333333333333 399769.6
269.666666666667 397209.6
270 397414.4
270.333333333333 396288
270.666666666667 397721.6
271 398131.2
271.333333333333 397721.6
271.666666666667 397312
272 398950.4
272.333333333333 397209.6
272.666666666667 399155.2
273 398233.6
273.333333333333 398950.4
273.666666666667 398028.8
274 0
274.333333333333 0
274.666666666667 0
275 0
275.333333333333 0
275.666666666667 0
276 0
276.333333333333 0
276.666666666667 0
277 0
277.333333333333 0
277.666666666667 0
278 0
278.333333333333 0
278.666666666667 0
279 0
279.333333333333 0
279.666666666667 0
280 0
280.333333333333 0
280.666666666667 0
281 0
281.333333333333 0
281.666666666667 0
282 0
282.333333333333 0
282.666666666667 0
283 0
283.333333333333 0
283.666666666667 0
284 398233.6
284.333333333333 397721.6
284.666666666667 398950.4
285 397619.2
285.333333333333 396595.2
285.666666666667 397414.4
286 397926.4
286.333333333333 396288
286.666666666667 398233.6
287 397721.6
287.333333333333 398131.2
287.666666666667 397414.4
288 398540.8
288.333333333333 398131.2
288.666666666667 396595.2
289 398131.2
289.333333333333 397721.6
289.666666666667 397107.2
290 397619.2
290.333333333333 397107.2
290.666666666667 397721.6
291 397824
291.333333333333 398028.8
291.666666666667 399052.8
292 397926.4
292.333333333333 398233.6
292.666666666667 397824
293 397824
293.333333333333 397209.6
293.666666666667 396390.4
294 398233.6
294.333333333333 395776
294.666666666667 397312
295 397516.8
295.333333333333 397004.8
295.666666666667 397721.6
296 397312
296.333333333333 397004.8
296.666666666667 397926.4
297 398131.2
297.333333333333 399155.2
297.666666666667 399155.2
298 396595.2
298.333333333333 399360
298.666666666667 399360
299 399257.6
299.333333333333 397824
299.666666666667 397619.2
300 398745.6
300.333333333333 396288
300.666666666667 397312
301 397721.6
301.333333333333 397209.6
301.666666666667 397312
302 395776
302.333333333333 398233.6
302.666666666667 397004.8
303 397721.6
303.333333333333 397926.4
303.666666666667 397926.4
304 397926.4
304.333333333333 398336
304.666666666667 397721.6
305 396288
305.333333333333 398950.4
305.666666666667 398028.8
306 395571.2
306.333333333333 396697.6
306.666666666667 397312
307 397107.2
307.333333333333 397824
307.666666666667 396492.8
308 396800
308.333333333333 398336
308.666666666667 398028.8
309 397414.4
309.333333333333 398643.2
309.666666666667 398540.8
310 396288
310.333333333333 397824
310.666666666667 397414.4
311 396390.4
311.333333333333 398233.6
311.666666666667 396595.2
312 398233.6
312.333333333333 397414.4
312.666666666667 397824
313 396288
313.333333333333 396390.4
313.666666666667 398643.2
314 396697.6
314.333333333333 398233.6
314.666666666667 0
315 0
315.333333333333 0
315.666666666667 0
316 0
316.333333333333 0
316.666666666667 0
317 0
317.333333333333 0
317.666666666667 0
318 0
318.333333333333 0
318.666666666667 0
319 0
319.333333333333 0
319.666666666667 0
320 0
320.333333333333 0
320.666666666667 0
321 0
321.333333333333 0
321.666666666667 0
322 0
322.333333333333 0
322.666666666667 0
323 0
323.333333333333 0
323.666666666667 0
};
\addlegendentry{\ckptThirty}
\addplot [semithick, color3, mark=diamond*, mark size=2.0, mark options={solid,fill=white}, mark repeat=60,mark phase=15]
table {%
0 0
0.333333333333333 35532.8
0.666666666666667 416665.6
1 406118.4
1.33333333333333 401612.8
1.66666666666667 398028.8
2 397312
2.33333333333333 394444.8
2.66666666666667 391372.8
3 390758.4
3.33333333333333 393011.2
3.66666666666667 391577.6
4 393113.6
4.33333333333333 389017.6
4.66666666666667 388915.2
5 388505.6
5.33333333333333 386560
5.66666666666667 388812.8
6 387584
6.33333333333333 389324.8
6.66666666666667 387584
7 388198.4
7.33333333333333 385740.8
7.66666666666667 386048
8 387174.4
8.33333333333333 386355.2
8.66666666666667 386662.4
9 384614.4
9.33333333333333 386867.2
9.66666666666667 385843.2
10 383283.2
10.3333333333333 383283.2
10.6666666666667 382156.8
11 382771.2
11.3333333333333 384204.8
11.6666666666667 384102.4
12 382566.4
12.3333333333333 384000
12.6666666666667 384409.6
13 383897.6
13.3333333333333 386048
13.6666666666667 384307.2
14 383283.2
14.3333333333333 384000
14.6666666666667 383385.6
15 385536
15.3333333333333 383692.8
15.6666666666667 383795.2
16 385126.4
16.3333333333333 383385.6
16.6666666666667 384614.4
17 382361.6
17.3333333333333 384204.8
17.6666666666667 382668.8
18 382054.4
18.3333333333333 381952
18.6666666666667 384204.8
19 382156.8
19.3333333333333 382668.8
19.6666666666667 382668.8
20 382566.4
20.3333333333333 384307.2
20.6666666666667 383897.6
21 382361.6
21.3333333333333 382566.4
21.6666666666667 382873.6
22 382464
22.3333333333333 381747.2
22.6666666666667 381644.8
23 382873.6
23.3333333333333 381747.2
23.6666666666667 380313.6
24 382464
24.3333333333333 381337.6
24.6666666666667 380620.8
25 382156.8
25.3333333333333 381849.6
25.6666666666667 382566.4
26 381132.8
26.3333333333333 381440
26.6666666666667 381644.8
27 381644.8
27.3333333333333 383385.6
27.6666666666667 381849.6
28 381849.6
28.3333333333333 381132.8
28.6666666666667 381030.4
29 381747.2
29.3333333333333 380211.2
29.6666666666667 381337.6
30 381747.2
30.3333333333333 382873.6
30.6666666666667 382156.8
31 383078.4
31.3333333333333 382156.8
31.6666666666667 383180.8
32 382361.6
32.3333333333333 381337.6
32.6666666666667 383590.4
33 382566.4
33.3333333333333 383078.4
33.6666666666667 383488
34 382976
34.3333333333333 383180.8
34.6666666666667 380006.4
35 382771.2
35.3333333333333 382873.6
35.6666666666667 382566.4
36 383692.8
36.3333333333333 382668.8
36.6666666666667 383897.6
37 383795.2
37.3333333333333 382976
37.6666666666667 381952
38 383897.6
38.3333333333333 383795.2
38.6666666666667 384409.6
39 381952
39.3333333333333 383590.4
39.6666666666667 384819.2
40 385331.2
40.3333333333333 384614.4
40.6666666666667 384000
41 383795.2
41.3333333333333 383488
41.6666666666667 384409.6
42 384716.8
42.3333333333333 383897.6
42.6666666666667 384204.8
43 384102.4
43.3333333333333 383385.6
43.6666666666667 382361.6
44 382873.6
44.3333333333333 382976
44.6666666666667 381542.4
45 382259.2
45.3333333333333 381235.2
45.6666666666667 383283.2
46 382156.8
46.3333333333333 381132.8
46.6666666666667 382259.2
47 380416
47.3333333333333 381235.2
47.6666666666667 382156.8
48 382464
48.3333333333333 382566.4
48.6666666666667 381132.8
49 381030.4
49.3333333333333 381747.2
49.6666666666667 382566.4
50 381952
50.3333333333333 384102.4
50.6666666666667 383795.2
51 382566.4
51.3333333333333 383385.6
51.6666666666667 382771.2
52 381644.8
52.3333333333333 382156.8
52.6666666666667 381644.8
53 383283.2
53.3333333333333 382054.4
53.6666666666667 381440
54 382668.8
54.3333333333333 380518.4
54.6666666666667 381337.6
55 382156.8
55.3333333333333 382873.6
55.6666666666667 382259.2
56 381235.2
56.3333333333333 381747.2
56.6666666666667 382566.4
57 381952
57.3333333333333 382156.8
57.6666666666667 380825.6
58 381747.2
58.3333333333333 381337.6
58.6666666666667 381337.6
59 382668.8
59.3333333333333 382259.2
59.6666666666667 381440
60 380825.6
60.3333333333333 380723.2
60.6666666666667 381644.8
61 380518.4
61.3333333333333 381542.4
61.6666666666667 381747.2
62 383180.8
62.3333333333333 381952
62.6666666666667 382771.2
63 382156.8
63.3333333333333 383385.6
63.6666666666667 383897.6
64 384409.6
64.3333333333333 383897.6
64.6666666666667 384000
65 382464
65.3333333333333 383795.2
65.6666666666667 382976
66 381747.2
66.3333333333333 382361.6
66.6666666666667 384102.4
67 382771.2
67.3333333333333 383078.4
67.6666666666667 382259.2
68 381849.6
68.3333333333333 383488
68.6666666666667 384409.6
69 382668.8
69.3333333333333 383488
69.6666666666667 382668.8
70 382771.2
70.3333333333333 381132.8
70.6666666666667 381132.8
71 380723.2
71.3333333333333 381849.6
71.6666666666667 380518.4
72 381337.6
72.3333333333333 382259.2
72.6666666666667 383078.4
73 381849.6
73.3333333333333 383283.2
73.6666666666667 382361.6
74 383692.8
74.3333333333333 384204.8
74.6666666666667 384409.6
75 383897.6
75.3333333333333 384409.6
75.6666666666667 381952
76 383283.2
76.3333333333333 382873.6
76.6666666666667 383180.8
77 381849.6
77.3333333333333 381132.8
77.6666666666667 383180.8
78 381952
78.3333333333333 383180.8
78.6666666666667 383180.8
79 383078.4
79.3333333333333 383488
79.6666666666667 380620.8
80 382873.6
80.3333333333333 382771.2
80.6666666666667 382464
81 383692.8
81.3333333333333 383078.4
81.6666666666667 383692.8
82 383795.2
82.3333333333333 382771.2
82.6666666666667 382259.2
83 384307.2
83.3333333333333 381644.8
83.6666666666667 380928
84 382361.6
84.3333333333333 381030.4
84.6666666666667 380928
85 381542.4
85.3333333333333 382361.6
85.6666666666667 382259.2
86 381337.6
86.3333333333333 381030.4
86.6666666666667 381030.4
87 382054.4
87.3333333333333 383488
87.6666666666667 382464
88 382054.4
88.3333333333333 380620.8
88.6666666666667 380108.8
89 382156.8
89.3333333333333 380211.2
89.6666666666667 382054.4
90 380620.8
90.3333333333333 382259.2
90.6666666666667 381030.4
91 381337.6
91.3333333333333 381952
91.6666666666667 381542.4
92 382361.6
92.3333333333333 381030.4
92.6666666666667 381747.2
93 382361.6
93.3333333333333 382566.4
93.6666666666667 381849.6
94 381542.4
94.3333333333333 381747.2
94.6666666666667 381644.8
95 381337.6
95.3333333333333 383385.6
95.6666666666667 382054.4
96 381644.8
96.3333333333333 381030.4
96.6666666666667 384614.4
97 385024
97.3333333333333 383488
97.6666666666667 383692.8
98 384307.2
98.3333333333333 383078.4
98.6666666666667 382873.6
99 382873.6
99.3333333333333 382873.6
99.6666666666667 381952
100 382054.4
100.333333333333 381952
100.666666666667 382873.6
101 382054.4
101.333333333333 381132.8
101.666666666667 382259.2
102 380723.2
102.333333333333 381235.2
102.666666666667 382054.4
103 382668.8
103.333333333333 382156.8
103.666666666667 381644.8
104 380928
104.333333333333 381440
104.666666666667 381849.6
105 382976
105.333333333333 381132.8
105.666666666667 382156.8
106 381337.6
106.333333333333 381235.2
106.666666666667 383180.8
107 381132.8
107.333333333333 382054.4
107.666666666667 381235.2
108 381337.6
108.333333333333 382771.2
108.666666666667 383795.2
109 380723.2
109.333333333333 381337.6
109.666666666667 382771.2
110 382566.4
110.333333333333 382668.8
110.666666666667 382566.4
111 381952
111.333333333333 382156.8
111.666666666667 381747.2
112 383590.4
112.333333333333 381747.2
112.666666666667 381235.2
113 382771.2
113.333333333333 380518.4
113.666666666667 381337.6
114 382361.6
114.333333333333 382054.4
114.666666666667 382054.4
115 380928
115.333333333333 381440
115.666666666667 381849.6
116 382361.6
116.333333333333 382566.4
116.666666666667 381337.6
117 381440
117.333333333333 381030.4
117.666666666667 381849.6
118 383590.4
118.333333333333 382464
118.666666666667 381542.4
119 381440
119.333333333333 383078.4
119.666666666667 382464
120 383180.8
120.333333333333 381542.4
120.666666666667 381747.2
121 382361.6
121.333333333333 382771.2
121.666666666667 382259.2
122 380825.6
122.333333333333 382054.4
122.666666666667 381132.8
123 381235.2
123.333333333333 383488
123.666666666667 384000
124 383692.8
124.333333333333 383897.6
124.666666666667 383283.2
125 383078.4
125.333333333333 384000
125.666666666667 382259.2
126 382054.4
126.333333333333 383283.2
126.666666666667 384102.4
127 381440
127.333333333333 383283.2
127.666666666667 383180.8
128 382668.8
128.333333333333 384819.2
128.666666666667 382771.2
129 382976
129.333333333333 383283.2
129.666666666667 381440
130 382054.4
130.333333333333 381542.4
130.666666666667 381030.4
131 381542.4
131.333333333333 381849.6
131.666666666667 382566.4
132 381030.4
132.333333333333 382361.6
132.666666666667 381849.6
133 380928
133.333333333333 382566.4
133.666666666667 383590.4
134 380620.8
134.333333333333 381952
134.666666666667 380620.8
135 381132.8
135.333333333333 380108.8
135.666666666667 380723.2
136 382873.6
136.333333333333 382668.8
136.666666666667 383590.4
137 380928
137.333333333333 382156.8
137.666666666667 381030.4
138 381440
138.333333333333 382566.4
138.666666666667 382464
139 384716.8
139.333333333333 382566.4
139.666666666667 382156.8
140 383488
140.333333333333 382259.2
140.666666666667 381849.6
141 382771.2
141.333333333333 382771.2
141.666666666667 381849.6
142 381337.6
142.333333333333 382259.2
142.666666666667 381542.4
143 381849.6
143.333333333333 381542.4
143.666666666667 381542.4
144 381747.2
144.333333333333 382976
144.666666666667 381542.4
145 382156.8
145.333333333333 381132.8
145.666666666667 381337.6
146 382259.2
146.333333333333 382771.2
146.666666666667 384614.4
147 382156.8
147.333333333333 382976
147.666666666667 383488
148 381747.2
148.333333333333 382054.4
148.666666666667 382361.6
149 382361.6
149.333333333333 381952
149.666666666667 381132.8
150 383078.4
150.333333333333 383795.2
150.666666666667 382668.8
151 383385.6
151.333333333333 384716.8
151.666666666667 385331.2
152 384307.2
152.333333333333 384409.6
152.666666666667 383590.4
153 383692.8
153.333333333333 384819.2
153.666666666667 384921.6
154 383385.6
154.333333333333 384307.2
154.666666666667 384000
155 383590.4
155.333333333333 382259.2
155.666666666667 383180.8
156 382668.8
156.333333333333 381542.4
156.666666666667 381132.8
157 382054.4
157.333333333333 384000
157.666666666667 381132.8
158 381542.4
158.333333333333 380620.8
158.666666666667 381440
159 380723.2
159.333333333333 381235.2
159.666666666667 382873.6
160 382566.4
160.333333333333 382259.2
160.666666666667 382566.4
161 382361.6
161.333333333333 382566.4
161.666666666667 383385.6
162 384000
162.333333333333 383385.6
162.666666666667 383897.6
163 383385.6
163.333333333333 383897.6
163.666666666667 383488
164 382464
164.333333333333 382976
164.666666666667 383385.6
165 382668.8
165.333333333333 381747.2
165.666666666667 381235.2
166 380313.6
166.333333333333 382054.4
166.666666666667 380108.8
167 381644.8
167.333333333333 382566.4
167.666666666667 382976
168 382464
168.333333333333 383283.2
168.666666666667 382054.4
169 382976
169.333333333333 383692.8
169.666666666667 384307.2
170 381440
170.333333333333 382873.6
170.666666666667 381030.4
171 381952
171.333333333333 381440
171.666666666667 381235.2
172 381952
172.333333333333 383897.6
172.666666666667 381030.4
173 381849.6
173.333333333333 380825.6
173.666666666667 380928
174 380518.4
174.333333333333 380620.8
174.666666666667 382464
175 382873.6
175.333333333333 382771.2
175.666666666667 381235.2
176 381849.6
176.333333333333 380825.6
176.666666666667 381644.8
177 381440
177.333333333333 381132.8
177.666666666667 382054.4
178 383897.6
178.333333333333 381030.4
178.666666666667 381132.8
179 382259.2
179.333333333333 382976
179.666666666667 383180.8
180 382976
180.333333333333 381644.8
180.666666666667 382156.8
181 381542.4
181.333333333333 383283.2
181.666666666667 381952
182 381132.8
182.333333333333 382361.6
182.666666666667 380928
183 381849.6
183.333333333333 382361.6
183.666666666667 379494.4
184 381747.2
184.333333333333 381542.4
184.666666666667 383180.8
185 382464
185.333333333333 382873.6
185.666666666667 382668.8
186 383692.8
186.333333333333 382361.6
186.666666666667 381235.2
187 382976
187.333333333333 381747.2
187.666666666667 383385.6
188 383283.2
188.333333333333 383180.8
188.666666666667 383385.6
189 381030.4
189.333333333333 382259.2
189.666666666667 382873.6
190 382054.4
190.333333333333 381747.2
190.666666666667 383078.4
191 381747.2
191.333333333333 381132.8
191.666666666667 382054.4
192 380518.4
192.333333333333 382054.4
192.666666666667 383488
193 384204.8
193.333333333333 383692.8
193.666666666667 384409.6
194 382361.6
194.333333333333 383488
194.666666666667 382668.8
195 381542.4
195.333333333333 382668.8
195.666666666667 385024
196 382566.4
196.333333333333 383078.4
196.666666666667 382361.6
197 382054.4
197.333333333333 381747.2
197.666666666667 383283.2
198 381747.2
198.333333333333 380928
198.666666666667 382464
199 381030.4
199.333333333333 381030.4
199.666666666667 382156.8
200 382259.2
200.333333333333 382054.4
200.666666666667 380825.6
201 381235.2
201.333333333333 381747.2
201.666666666667 381952
202 382156.8
202.333333333333 381132.8
202.666666666667 381849.6
203 381132.8
203.333333333333 381132.8
203.666666666667 381337.6
204 381644.8
204.333333333333 381337.6
204.666666666667 383283.2
205 382156.8
205.333333333333 381644.8
205.666666666667 380313.6
206 380518.4
206.333333333333 381747.2
206.666666666667 380006.4
207 382156.8
207.333333333333 382054.4
207.666666666667 383692.8
208 382156.8
208.333333333333 380723.2
208.666666666667 381644.8
209 381952
209.333333333333 381235.2
209.666666666667 381440
210 384512
210.333333333333 382873.6
210.666666666667 381952
211 382976
211.333333333333 381644.8
211.666666666667 381952
212 381849.6
212.333333333333 382976
212.666666666667 382259.2
213 381747.2
213.333333333333 384000
213.666666666667 384204.8
214 382566.4
214.333333333333 383795.2
214.666666666667 384716.8
215 385126.4
215.333333333333 384716.8
215.666666666667 383795.2
216 383897.6
216.333333333333 383795.2
216.666666666667 383078.4
217 383692.8
217.333333333333 384307.2
217.666666666667 383180.8
218 383283.2
218.333333333333 384409.6
218.666666666667 384409.6
219 386048
219.333333333333 384614.4
219.666666666667 383590.4
220 383692.8
220.333333333333 383283.2
220.666666666667 385638.4
221 383590.4
221.333333333333 383897.6
221.666666666667 384102.4
222 384204.8
222.333333333333 381952
222.666666666667 382668.8
223 382771.2
223.333333333333 381747.2
223.666666666667 381030.4
224 381952
224.333333333333 383385.6
224.666666666667 382054.4
225 381440
225.333333333333 380825.6
225.666666666667 380518.4
226 381747.2
226.333333333333 380108.8
226.666666666667 382156.8
227 382156.8
227.333333333333 382771.2
227.666666666667 382566.4
228 382771.2
228.333333333333 382156.8
228.666666666667 383897.6
229 381849.6
229.333333333333 380723.2
229.666666666667 383180.8
230 382259.2
230.333333333333 380518.4
230.666666666667 382771.2
231 384102.4
231.333333333333 384716.8
231.666666666667 384102.4
232 383692.8
232.333333333333 382156.8
232.666666666667 383488
233 382361.6
233.333333333333 381542.4
233.666666666667 382668.8
234 384204.8
234.333333333333 382976
234.666666666667 382668.8
235 381952
235.333333333333 382259.2
235.666666666667 383692.8
236 383897.6
236.333333333333 382566.4
236.666666666667 382259.2
237 380108.8
237.333333333333 380928
237.666666666667 381849.6
238 381849.6
238.333333333333 382668.8
238.666666666667 381337.6
239 381440
239.333333333333 381849.6
239.666666666667 382054.4
240 382054.4
240.333333333333 381030.4
240.666666666667 381542.4
241 381747.2
241.333333333333 381849.6
241.666666666667 383385.6
242 382566.4
242.333333333333 381440
242.666666666667 380723.2
243 384716.8
243.333333333333 380416
243.666666666667 382054.4
244 381747.2
244.333333333333 382464
244.666666666667 382054.4
245 381030.4
245.333333333333 381030.4
245.666666666667 381542.4
246 381235.2
246.333333333333 383385.6
246.666666666667 381030.4
247 381849.6
247.333333333333 381337.6
247.666666666667 381849.6
248 383385.6
248.333333333333 381132.8
248.666666666667 381747.2
249 381440
249.333333333333 381644.8
249.666666666667 381952
250 384716.8
250.333333333333 384512
250.666666666667 384000
251 383897.6
251.333333333333 383078.4
251.666666666667 384307.2
252 385228.8
252.333333333333 383180.8
252.666666666667 384409.6
253 383897.6
253.333333333333 383692.8
253.666666666667 382668.8
254 383283.2
254.333333333333 382464
254.666666666667 381849.6
255 382259.2
255.333333333333 381849.6
255.666666666667 383283.2
256 382361.6
256.333333333333 381235.2
256.666666666667 383078.4
257 382873.6
257.333333333333 383897.6
257.666666666667 382156.8
258 382054.4
258.333333333333 382976
258.666666666667 383385.6
259 382259.2
259.333333333333 383180.8
259.666666666667 382566.4
260 382566.4
260.333333333333 384716.8
260.666666666667 382873.6
261 382464
261.333333333333 381132.8
261.666666666667 380620.8
262 381747.2
262.333333333333 381644.8
262.666666666667 382976
263 381337.6
263.333333333333 383180.8
263.666666666667 383590.4
264 383283.2
264.333333333333 383795.2
264.666666666667 382566.4
265 383385.6
265.333333333333 384614.4
265.666666666667 385536
266 384307.2
266.333333333333 383897.6
266.666666666667 384000
267 384000
267.333333333333 384409.6
267.666666666667 384921.6
268 383488
268.333333333333 384204.8
268.666666666667 383488
269 383488
269.333333333333 382566.4
269.666666666667 383078.4
270 384716.8
270.333333333333 383078.4
270.666666666667 382668.8
271 382668.8
271.333333333333 383180.8
271.666666666667 381747.2
272 381747.2
272.333333333333 382054.4
272.666666666667 382976
273 382156.8
273.333333333333 381952
273.666666666667 381030.4
274 380825.6
274.333333333333 381849.6
274.666666666667 379801.6
275 382156.8
275.333333333333 381747.2
275.666666666667 382566.4
276 382259.2
276.333333333333 383385.6
276.666666666667 386764.8
277 385536
277.333333333333 386048
277.666666666667 386764.8
278 386048
278.333333333333 385126.4
278.666666666667 386048
279 387072
279.333333333333 384102.4
279.666666666667 383385.6
280 382156.8
280.333333333333 381747.2
280.666666666667 384204.8
281 383692.8
281.333333333333 383897.6
281.666666666667 382566.4
282 384409.6
282.333333333333 384204.8
282.666666666667 384819.2
283 384204.8
};
\addlegendentry{\sysKTwo}

==> figures/evaluation/data/recovery/criteo-4x/progress.tex <==
\addplot [semithick, color0,mark=*, mark size=1.5, mark options={solid,fill=white}, mark repeat=15,mark phase=3]
table {%
0 8086271.84333628
0.333333333333333 16170413.4780732
0.666666666666667 24237513.4440148
1 32319524.8701523
1.33333333333333 40431359.2166814
1.66666666666667 48524021.6858159
2 56631595.6151462
2.33333333333333 64739169.5444765
2.66666666666667 72793488.2588217
3 80920234.0655467
3.33333333333333 88980943.4056901
3.66666666666667 97045913.1630324
4 105125794.38057
4.33333333333333 113190764.137913
4.66666666666667 121287687.024246
5 129363307.824585
5.33333333333333 137443189.042123
5.66666666666667 145542242.137056
6 153647685.857787
6.33333333333333 161736087.909723
6.66666666666667 169860703.507848
7 177957626.394181
7.33333333333333 186046028.446117
7.66666666666667 194106737.786261
8 202195139.838196
8.33333333333333 210283541.890132
8.66666666666667 218378334.567866
9 226479517.871398
9.33333333333333 234559399.088936
9.66666666666667 242643540.723673
10 242643540.723673
10.3333333333333 242643540.723673
10.6666666666667 242643540.723673
11 242643540.723673
11.3333333333333 242643540.723673
11.6666666666667 242643540.723673
12 242643540.723673
12.3333333333333 242643540.723673
12.6666666666667 242643540.723673
13 242643540.723673
13.3333333333333 242643540.723673
13.6666666666667 242643540.723673
14 242643540.723673
14.3333333333333 242643540.723673
14.6666666666667 242643540.723673
15 242643540.723673
15.3333333333333 242643540.723673
15.6666666666667 242643540.723673
16 250757505.278801
16.3333333333333 258813954.201746
16.6666666666667 266881054.167688
17 274986497.888418
17.3333333333333 283085550.983351
17.6666666666667 291195255.121281
18 299273006.13022
18.3333333333333 307346496.721959
18.6666666666667 315417857.1051
19 323512649.782834
19.3333333333333 331637265.380959
19.6666666666667 339740578.893091
20 347848152.822421
20.3333333333333 355883299.659372
20.6666666666667 363986613.171503
21 372070754.80624
21.3333333333333 380150636.023778
21.6666666666667 388219866.198319
22 396355132.839442
22.3333333333333 404452055.725775
22.6666666666667 412521285.900316
23 420573474.406062
23.3333333333333 428666136.875196
23.6666666666667 436735367.049738
24 444819508.684474
24.3333333333333 452924952.405205
24.6666666666667 461030396.125936
25 469116667.969272
25.3333333333333 477249804.401796
25.6666666666667 485353117.913927
26 493441519.965863
26.3333333333333 501576786.606985
26.6666666666667 509633235.52993
27 517721637.581866
27.3333333333333 525818560.468199
27.6666666666667 533877139.599743
28 541980453.111874
28.3333333333333 550066724.955211
28.6666666666667 558157257.215746
29 566230747.807486
29.3333333333333 574304238.399226
29.6666666666667 582362817.53077
30 590466131.042901
30.3333333333333 598548142.469038
30.6666666666667 606625893.477977
31 614692993.443919
31.3333333333333 622775004.870056
31.6666666666667 630886839.216585
32 638998673.563115
32.3333333333333 647136070.412836
32.6666666666667 655245774.550766
33 663321395.351105
33.3333333333333 671377844.27405
33.6666666666667 679472636.951784
34 687518434.831732
34.3333333333333 695594055.632071
34.6666666666667 703682457.684006
35 711755948.275746
35.3333333333333 719880563.873872
35.6666666666667 727943403.422615
36 736042456.517547
36.3333333333333 744143639.82108
36.6666666666667 752212869.995621
37 760311923.090553
37.3333333333333 768404585.559688
37.6666666666667 776490857.403024
38 784564347.994764
38.3333333333333 792635708.377904
38.6666666666667 800715589.595442
39 808772038.518387
39.3333333333333 816860440.570323
39.6666666666667 824897717.615873
40 832990380.085007
40.3333333333333 841121386.308931
40.6666666666667 849177835.231876
41 857255586.240814
41.3333333333333 865367420.587343
41.6666666666667 873506947.645665
42 881593219.489001
42.3333333333333 889677361.123738
42.6666666666667 897774284.010071
43 905834993.350215
43.3333333333333 913925525.61075
43.6666666666667 922013927.662686
44 930136413.052212
44.3333333333333 938254638.024539
44.6666666666667 946313217.156083
45 954386707.747823
45.3333333333333 962470849.38256
45.6666666666667 970512386.845309
46 978568835.768253
46.3333333333333 986635935.734195
46.6666666666667 994741379.454926
47 1002857474.21865
47.3333333333333 1010922443.976
47.6666666666667 1018998064.77634
48 1027084336.61967
48.3333333333333 1035185519.9232
48.6666666666667 1043276052.18374
49 1051336761.52388
49.3333333333333 1059423033.36722
49.6666666666667 1067526346.87935
50 1075587056.21949
50.3333333333333 1083692499.94022
50.6666666666667 1091778771.78356
51 1099841611.3323
51.3333333333333 1107910841.50684
51.6666666666667 1116009894.60178
52 1124098296.65371
52.3333333333333 1132152615.36806
52.6666666666667 1140272970.54898
53 1148335810.09773
53.3333333333333 1156424212.14966
53.6666666666667 1164519004.8274
54 1172609537.08793
54.3333333333333 1180680897.47107
54.6666666666667 1188769299.52301
55 1196842790.11475
55.3333333333333 1204965275.50427
55.6666666666667 1213053677.55621
56 1221139949.39955
56.3333333333333 1229196398.32249
56.6666666666667 1237276279.54003
57 1245383853.46936
57.3333333333333 1253446693.0181
57.6666666666667 1261524444.02704
58 1269595804.41018
58.3333333333333 1277720420.00831
58.6666666666667 1285766217.88825
59 1293841838.68859
59.3333333333333 1301951542.82652
59.6666666666667 1310022903.20966
60 1318113435.4702
60.3333333333333 1326233790.65113
60.6666666666667 1334262546.86228
61 1342338167.66262
61.3333333333333 1350437220.75755
61.6666666666667 1358549055.10408
62 1366645977.99041
62.3333333333333 1374727989.41655
62.6666666666667 1382837693.55448
63 1390949527.90101
63.3333333333333 1399035799.74434
63.6666666666667 1407098639.29309
64 1415182780.92782
64.3333333333333 1423275443.39696
64.6666666666667 1431370236.07469
65 1439490591.25562
65.3333333333333 1447561951.63876
65.6666666666667 1455652483.8993
66 1463749406.78563
66.3333333333333 1471822897.37737
66.6666666666667 1479866565.04872
67 1487937925.43186
67.3333333333333 1496019936.85799
67.6666666666667 1504097687.86693
68 1512201001.37906
68.3333333333333 1520283012.8052
68.6666666666667 1528347982.56254
69 1536406561.69409
69.3333333333333 1544499224.16322
69.6666666666667 1552570584.54636
70 1560612122.00911
70.3333333333333 1568692003.22665
70.6666666666667 1576774014.65279
71 1584853895.87033
71.3333333333333 1592931646.87926
71.6666666666667 1601020048.9312
72 1609140404.11213
72.3333333333333 1617207504.07807
72.6666666666667 1625298036.3386
73 1633358745.67875
73.3333333333333 1641466319.60808
73.6666666666667 1649533419.57402
74 1657632472.66895
74.3333333333333 1665716614.30369
74.6666666666667 1673839099.69321
75 1681921111.11935
75.3333333333333 1689996731.91969
75.6666666666667 1698095785.01462
76 1706167145.39776
76.3333333333333 1714251287.0325
76.6666666666667 1722324777.62424
77 1730396138.00738
77.3333333333333 1738495191.10231
77.6666666666667 1746577202.52845
78 1754646432.70299
78.3333333333333 1762734834.75493
78.6666666666667 1770870101.39605
79 1778967024.28238
79.3333333333333 1787023473.20533
79.6666666666667 1795082052.33687
80 1803170454.38881
80.3333333333333 1811267377.27514
80.6666666666667 1819330216.82388
81 1827439920.96181
81.3333333333333 1835511281.34496
81.6666666666667 1843586902.14529
82 1851662522.94563
82.3333333333333 1859750924.99757
82.6666666666667 1867867019.7613
83 1875978854.10783
83.3333333333333 1884077907.20276
83.6666666666667 1892164179.0461
84 1900227018.59484
84.3333333333333 1908289858.14358
84.6666666666667 1916356958.10952
85 1924432578.90986
85.3333333333333 1932529501.7962
85.6666666666667 1940639205.93412
86 1948731868.40326
86.3333333333333 1956796838.1606
86.6666666666667 1964908672.50713
87 1972969381.84727
87.3333333333333 1981068434.94221
87.6666666666667 1989186659.91453
88 1997272931.75787
88.3333333333333 2005369854.6442
88.6666666666667 2013460386.90474
89 2021540268.12228
89.3333333333333 2029620149.33981
89.6666666666667 2037663817.01116
90 2045745828.4373
90.3333333333333 2053849141.94943
90.6666666666667 2061918372.12397
91 2070015295.01031
91.3333333333333 2078093046.01924
91.6666666666667 2086170797.02818
92 2094257068.87152
92.3333333333333 2102296476.12567
92.6666666666667 2110427482.34959
93 2118494582.31553
93.3333333333333 2126593635.41047
93.6666666666667 2134677777.0452
94 2142740616.59395
94.3333333333333 2150818367.60289
94.6666666666667 2158891858.19462
95 2166997301.91536
95.3333333333333 2175079313.34149
95.6666666666667 2183182626.85362
96 2191277419.53136
96.3333333333333 2199355170.5403
96.6666666666667 2207420140.29764
97 2215508542.34958
97.3333333333333 2223573512.10692
97.6666666666667 2231695997.49644
98 2239767357.87958
98.3333333333333 2247864280.76592
98.6666666666667 2255924990.10606
99 2264024043.20099
};
\addplot [semithick, color1,mark=square*, mark size=1.5, mark options={solid,fill=white}, mark repeat=15,mark phase=9]
table {%
0 8086271.84333628
0.333333333333333 16170413.4780732
0.666666666666667 24237513.4440148
1 32319524.8701523
1.33333333333333 40431359.2166814
1.66666666666667 48524021.6858159
2 56631595.6151462
2.33333333333333 64739169.5444765
2.66666666666667 72793488.2588217
3 80920234.0655467
3.33333333333333 88980943.4056901
3.66666666666667 97045913.1630324
4 105125794.38057
4.33333333333333 113190764.137913
4.66666666666667 121287687.024246
5 129363307.824585
5.33333333333333 137443189.042123
5.66666666666667 145542242.137056
6 153647685.857787
6.33333333333333 161736087.909723
6.66666666666667 169860703.507848
7 177957626.394181
7.33333333333333 186046028.446117
7.66666666666667 194106737.786261
8 202195139.838196
8.33333333333333 210283541.890132
8.66666666666667 218378334.567866
9 226479517.871398
9.33333333333333 234559399.088936
9.66666666666667 242643540.723673
10 242643540.723673
10.3333333333333 242643540.723673
10.6666666666667 242643540.723673
11 242643540.723673
11.3333333333333 242643540.723673
11.6666666666667 242643540.723673
12 242643540.723673
12.3333333333333 242643540.723673
12.6666666666667 242643540.723673
13 242643540.723673
13.3333333333333 242643540.723673
13.6666666666667 242643540.723673
14 242643540.723673
14.3333333333333 242643540.723673
14.6666666666667 242643540.723673
15 242643540.723673
15.3333333333333 242643540.723673
15.6666666666667 242643540.723673
16 242643540.723673
16.3333333333333 242643540.723673
16.6666666666667 242643540.723673
17 242643540.723673
17.3333333333333 242643540.723673
17.6666666666667 242643540.723673
18 242643540.723673
18.3333333333333 242643540.723673
18.6666666666667 242643540.723673
19 242643540.723673
19.3333333333333 242643540.723673
19.6666666666667 242643540.723673
20 242643540.723673
20.3333333333333 242643540.723673
20.6666666666667 242643540.723673
21 242643540.723673
21.3333333333333 242643540.723673
21.6666666666667 242643540.723673
22 242643540.723673
22.3333333333333 242643540.723673
22.6666666666667 242643540.723673
23 242643540.723673
23.3333333333333 242643540.723673
23.6666666666667 242643540.723673
24 242643540.723673
24.3333333333333 242643540.723673
24.6666666666667 242643540.723673
25 242643540.723673
25.3333333333333 242643540.723673
25.6666666666667 242643540.723673
26 242643540.723673
26.3333333333333 242643540.723673
26.6666666666667 242643540.723673
27 242643540.723673
27.3333333333333 242643540.723673
27.6666666666667 242643540.723673
28 242643540.723673
28.3333333333333 242643540.723673
28.6666666666667 242643540.723673
29 242643540.723673
29.3333333333333 242643540.723673
29.6666666666667 242643540.723673
30 242643540.723673
30.3333333333333 242643540.723673
30.6666666666667 242643540.723673
31 250736203.192807
31.3333333333333 258824605.244743
31.6666666666667 266902356.253682
32 274948154.133629
32.3333333333333 283062118.688758
32.6666666666667 291152650.949293
33 299270875.92162
33.3333333333333 307369929.016553
33.6666666666667 315460461.277088
34 323538212.286027
34.3333333333333 331603182.043369
34.6666666666667 339706495.5555
35 347852413.23962
35.3333333333333 355908862.162564
35.6666666666667 363967441.294109
36 372047322.511647
36.3333333333333 380137854.772182
36.6666666666667 388241168.284313
37 396380695.342634
37.3333333333333 404469097.39457
37.6666666666667 412587322.366898
38 420699156.713427
38.3333333333333 428759866.05357
38.6666666666667 436856788.939903
39 444957972.243436
39.3333333333333 453029332.626576
39.6666666666667 461117734.678512
40 469206136.730447
40.3333333333333 477273236.696389
40.6666666666667 485355248.122526
41 493447910.591661
41.3333333333333 501559744.93819
41.6666666666667 509633235.52993
42 517713116.747468
42.3333333333333 525807909.425202
42.6666666666667 533868618.765345
43 541971932.277477
43.3333333333333 550090157.249804
43.6666666666667 558180689.510339
44 566273351.979474
44.3333333333333 574372405.074406
44.6666666666667 582499150.881131
45 590574771.681471
45.3333333333333 598686606.028
45.6666666666667 606768617.454137
46 614888972.635064
46.3333333333333 622985895.521397
46.6666666666667 631052995.487339
47 639143527.747874
47.3333333333333 647219148.548213
47.6666666666667 655318201.643146
48 663395952.652084
48.3333333333333 671495005.747017
48.6666666666667 679570626.547356
49 687693111.936882
49.3333333333333 695807076.492011
49.6666666666667 703880567.083751
50 711939146.215295
50.3333333333333 720053110.770424
50.6666666666667 728120210.736365
51 736219263.831298
51.3333333333333 744318316.926231
51.6666666666667 752425890.855561
52 760556897.079485
52.3333333333333 768662340.800216
52.6666666666667 776710268.888763
53 784792280.3149
53.3333333333333 792880682.366836
53.6666666666667 800949912.541377
54 809053226.053508
54.3333333333333 817148018.731242
54.6666666666667 825238550.991777
55 833318432.209315
55.3333333333333 841400443.635453
55.6666666666667 849456892.558397
56 857543164.401734
56.3333333333333 865629436.24507
56.6666666666667 873677364.333617
57 881738073.67376
57.3333333333333 889815824.682699
57.6666666666667 897899966.317436
58 905947894.405983
58.3333333333333 914027775.623521
58.6666666666667 922103396.42386
59 930181147.432799
59.3333333333333 938265289.067536
59.6666666666667 946315347.364682
60 954410140.042416
60.3333333333333 962530495.223343
60.6666666666667 970593334.772086
61 978713689.953012
61.3333333333333 986812743.047945
61.6666666666667 994871322.179489
62 1002970375.27442
62.3333333333333 1011094990.87255
62.6666666666667 1019172741.88149
63 1027246232.47323
63.3333333333333 1035334634.52516
63.6666666666667 1043457119.91469
64 1051545521.96662
64.3333333333333 1059621142.76696
64.6666666666667 1067724456.27909
65 1075761733.32464
65.3333333333333 1083877828.08837
65.6666666666667 1091983271.8091
66 1100022679.06325
66.3333333333333 1108123862.36678
66.6666666666667 1116199483.16712
67 1124304926.88785
67.3333333333333 1132389068.52259
67.6666666666667 1140505163.28632
68 1148563742.41786
68.3333333333333 1156643623.6354
68.6666666666667 1164700072.55835
69 1172777823.56728
69.3333333333333 1180906699.58261
69.6666666666667 1188971669.33995
70 1197036639.09729
70.3333333333333 1205118650.52343
70.6666666666667 1213234745.28716
71 1221327407.75629
71.3333333333333 1229411549.39103
71.6666666666667 1237514862.90316
72 1245603264.9551
72.3333333333333 1253689536.79843
72.6666666666667 1261782199.26757
73 1269849299.23351
73.3333333333333 1277944091.91124
73.6666666666667 1286026103.33738
74 1294129416.84951
74.3333333333333 1302211428.27565
74.6666666666667 1310284918.86739
75 1318388232.37952
75.3333333333333 1326465983.38846
75.6666666666667 1334552255.2318
76 1342655568.74393
76.3333333333333 1350754621.83886
76.6666666666667 1358828112.4306
77 1366914384.27394
77.3333333333333 1375028348.82907
77.6666666666667 1383140183.17559
78 1391207283.14154
78.3333333333333 1399295685.19347
78.6666666666667 1407407519.54
79 1415538525.76392
79.3333333333333 1423607755.93847
79.6666666666667 1431691897.5732
80 1439748346.49615
80.3333333333333 1447830357.92228
80.6666666666667 1455914499.55702
81 1463968818.27137
81.3333333333333 1472033788.02871
81.6666666666667 1480126450.49784
82 1488229764.00997
82.3333333333333 1496303254.60171
82.6666666666667 1504415088.94824
83 1512499230.58298
83.3333333333333 1520559939.92312
83.6666666666667 1528648341.97506
84 1536726092.984
84.3333333333333 1544812364.82733
84.6666666666667 1552892246.04487
85 1560980648.09681
85.3333333333333 1569034966.81115
85.6666666666667 1577123368.86309
86 1585190468.82903
86.3333333333333 1593295912.54976
86.6666666666667 1601382184.3931
87 1609423721.85585
87.3333333333333 1617527035.36798
87.6666666666667 1625602656.16832
88 1633663365.50846
88.3333333333333 1641749637.3518
88.6666666666667 1649852950.86393
89 1657949873.75026
89.3333333333333 1666036145.5936
89.6666666666667 1674160761.19172
90 1682268335.12105
90.3333333333333 1690358867.38159
90.6666666666667 1698470701.72812
91 1706571885.03165
91.3333333333333 1714677328.75238
91.6666666666667 1722774251.63871
92 1730852002.64765
92.3333333333333 1738948925.53399
92.6666666666667 1747060759.88052
93 1755147031.72385
93.3333333333333 1763243954.61019
93.6666666666667 1771340877.49652
94 1779435670.17425
94.3333333333333 1787502770.14019
94.6666666666667 1795565609.68894
95 1803662532.57527
95.3333333333333 1811718981.49821
95.6666666666667 1819822295.01035
96 1827938389.77407
96.3333333333333 1836018270.99161
96.6666666666667 1844108803.25215
97 1852165252.17509
97.3333333333333 1860281346.93882
97.6666666666667 1868346316.69616
98 1876449630.20829
98.3333333333333 1884520990.59143
98.6666666666667 1892594481.18317
99 1900653060.31472
99.3333333333333 1908726550.90646
99.6666666666667 1916823473.79279
100 1924950219.59952
100.333333333333 1933019449.77406
100.666666666667 1941080159.1142
101 1949166430.95754
101.333333333333 1957263353.84387
101.666666666667 1965381578.8162
102 1973472111.07673
102.333333333333 1981560513.12867
102.666666666667 1989680868.30959
103 1997784181.82173
103.333333333333 2005898146.37685
103.666666666667 2013973767.17719
104 2022070690.06353
104.333333333333 2030152701.48966
104.666666666667 2038226192.0814
105 2046291161.83875
105.333333333333 2054409386.81107
105.666666666667 2062495658.65441
106 2070575539.87195
106.333333333333 2078625598.16909
106.666666666667 2086716130.42963
107 2094798141.85577
107.333333333333 2102897194.9507
107.666666666667 2110985597.00264
108 2119099561.55776
108.333333333333 2127192224.0269
108.666666666667 2135267844.82724
109 2143390330.21676
109.333333333333 2151465951.0171
109.666666666667 2159592696.82383
110 2167687489.50156
110.333333333333 2175765240.5105
110.666666666667 2183830210.26784
111 2191952695.65737
111.333333333333 2200026186.24911
111.666666666667 2208084765.38065
112 2216139084.095
112.333333333333 2224208314.26954
112.666666666667 2232300976.73867
113 2240419201.711
113.333333333333 2248505473.55434
113.666666666667 2256549141.22569
114 2264643933.90342
};
\addplot [semithick, color2,mark=x, mark size=1.8, mark options={solid,fill=white}, mark repeat=15,mark phase=13]
table {%
0 8086271.84333628
0.333333333333333 16170413.4780732
0.666666666666667 24237513.4440148
1 32319524.8701523
1.33333333333333 40431359.2166814
1.66666666666667 48524021.6858159
2 56631595.6151462
2.33333333333333 64739169.5444765
2.66666666666667 72793488.2588217
3 80920234.0655467
3.33333333333333 88980943.4056901
3.66666666666667 97045913.1630324
4 105125794.38057
4.33333333333333 113190764.137913
4.66666666666667 121287687.024246
5 129363307.824585
5.33333333333333 137443189.042123
5.66666666666667 145542242.137056
6 153647685.857787
6.33333333333333 161736087.909723
6.66666666666667 169860703.507848
7 177957626.394181
7.33333333333333 186046028.446117
7.66666666666667 194106737.786261
8 202195139.838196
8.33333333333333 210283541.890132
8.66666666666667 218378334.567866
9 226479517.871398
9.33333333333333 234559399.088936
9.66666666666667 242643540.723673
10 242643540.723673
10.3333333333333 242643540.723673
10.6666666666667 242643540.723673
11 242643540.723673
11.3333333333333 242643540.723673
11.6666666666667 242643540.723673
12 242643540.723673
12.3333333333333 242643540.723673
12.6666666666667 242643540.723673
13 242643540.723673
13.3333333333333 242643540.723673
13.6666666666667 242643540.723673
14 242643540.723673
14.3333333333333 242643540.723673
14.6666666666667 242643540.723673
15 242643540.723673
15.3333333333333 242643540.723673
15.6666666666667 242643540.723673
16 242643540.723673
16.3333333333333 242643540.723673
16.6666666666667 242643540.723673
17 242643540.723673
17.3333333333333 242643540.723673
17.6666666666667 242643540.723673
18 242643540.723673
18.3333333333333 242643540.723673
18.6666666666667 242643540.723673
19 242643540.723673
19.3333333333333 242643540.723673
19.6666666666667 242643540.723673
20 242643540.723673
20.3333333333333 242643540.723673
20.6666666666667 242643540.723673
21 242643540.723673
21.3333333333333 242643540.723673
21.6666666666667 242643540.723673
22 242643540.723673
22.3333333333333 242643540.723673
22.6666666666667 242643540.723673
23 242643540.723673
23.3333333333333 242643540.723673
23.6666666666667 242643540.723673
24 242643540.723673
24.3333333333333 242643540.723673
24.6666666666667 242643540.723673
25 242643540.723673
25.3333333333333 242643540.723673
25.6666666666667 242643540.723673
26 242643540.723673
26.3333333333333 242643540.723673
26.6666666666667 242643540.723673
27 242643540.723673
27.3333333333333 242643540.723673
27.6666666666667 242643540.723673
28 242643540.723673
28.3333333333333 242643540.723673
28.6666666666667 242643540.723673
29 242643540.723673
29.3333333333333 242643540.723673
29.6666666666667 242643540.723673
30 242643540.723673
30.3333333333333 242643540.723673
30.6666666666667 242643540.723673
31 242643540.723673
31.3333333333333 242643540.723673
31.6666666666667 242643540.723673
32 242643540.723673
32.3333333333333 242643540.723673
32.6666666666667 242643540.723673
33 242643540.723673
33.3333333333333 242643540.723673
33.6666666666667 242643540.723673
34 242643540.723673
34.3333333333333 242643540.723673
34.6666666666667 242643540.723673
35 242643540.723673
35.3333333333333 242643540.723673
35.6666666666667 242643540.723673
36 242643540.723673
36.3333333333333 242643540.723673
36.6666666666667 242643540.723673
37 242643540.723673
37.3333333333333 242643540.723673
37.6666666666667 242643540.723673
38 242643540.723673
38.3333333333333 242643540.723673
38.6666666666667 242643540.723673
39 242643540.723673
39.3333333333333 242643540.723673
39.6666666666667 242643540.723673
40 242643540.723673
40.3333333333333 242643540.723673
40.6666666666667 242643540.723673
41 242643540.723673
41.3333333333333 242643540.723673
41.6666666666667 242643540.723673
42 242643540.723673
42.3333333333333 242643540.723673
42.6666666666667 242643540.723673
43 242643540.723673
43.3333333333333 242643540.723673
43.6666666666667 242643540.723673
44 242643540.723673
44.3333333333333 242643540.723673
44.6666666666667 242643540.723673
45 242643540.723673
45.3333333333333 242643540.723673
45.6666666666667 242643540.723673
46 250738333.401407
46.3333333333333 258845907.330737
46.6666666666667 266887444.793486
47 274982237.47122
47.3333333333333 283038686.394164
47.6666666666667 291146260.323495
48 299262355.087222
48.3333333333333 307346496.721959
48.6666666666667 315439159.191094
49 323497738.322638
49.3333333333333 331618093.503565
49.6666666666667 339691584.095304
50 347716079.889258
50.3333333333333 355795961.106796
50.6666666666667 363926967.33072
51 372006848.548258
51.3333333333333 380046255.802407
51.6666666666667 388130397.437144
52 396214539.071881
52.3333333333333 404288029.663621
52.6666666666667 412374301.506957
53 420471224.393291
53.3333333333333 428566017.071024
53.6666666666667 436665070.165957
54 444730039.923299
54.3333333333333 452826962.809633
54.6666666666667 460900453.401372
55 469012287.747902
55.3333333333333 477107080.425635
55.6666666666667 485206133.520568
56 493294535.572504
56.3333333333333 501402109.501834
56.6666666666667 509526725.09996
57 517583174.022904
57.3333333333333 525675836.492039
57.6666666666667 533772759.378372
58 541869682.264705
58.3333333333333 549928261.396249
58.6666666666667 558033705.11698
59 566105065.500121
59.3333333333333 574233941.515445
59.6666666666667 582309562.315784
60 590383052.907524
60.3333333333333 598482106.002457
60.6666666666667 606561987.219995
61 614667430.940726
61.3333333333333 622768614.244258
61.6666666666667 630871927.756389
62 638953939.182527
62.3333333333333 647029559.982866
62.6666666666667 655122222.452
63 663227666.172731
63.3333333333333 671322458.850465
63.6666666666667 679410860.902401
64 687501393.162936
64.3333333333333 695562102.50308
64.6666666666667 703680327.475407
65 711770859.735942
65.3333333333333 719818787.824489
65.6666666666667 727917840.919422
66 736025414.848752
66.3333333333333 744081863.771697
66.6666666666667 752168135.615033
67 760252277.24977
67.3333333333333 768344939.718904
67.6666666666667 776407779.267647
68 784466358.399191
68.3333333333333 792565411.494124
68.6666666666667 800655943.754659
69 808754996.849592
69.3333333333333 816843398.901527
69.6666666666667 824944582.205059
70 833003161.336603
70.3333333333333 841127776.934729
70.6666666666667 849205527.943668
71 857268367.492411
71.3333333333333 865397243.507735
71.6666666666667 873432390.344685
72 881505880.936425
72.3333333333333 889613454.865756
72.6666666666667 897706117.33489
73 905783868.343829
73.3333333333333 913889312.06456
73.6666666666667 921981974.533694
74 930040553.665238
74.3333333333333 938122565.091376
74.6666666666667 946200316.100314
75 954263155.649057
75.3333333333333 962364338.952589
75.6666666666667 970476173.299118
76 978558184.725256
76.3333333333333 986584810.727809
76.6666666666667 994711556.534534
77 1002780786.70907
77.3333333333333 1010843626.25782
77.6666666666667 1018889424.13777
78 1026999128.27569
78.3333333333333 1035093920.95343
78.6666666666667 1043190843.83976
79 1051298417.76909
79.3333333333333 1059363387.52643
79.6666666666667 1067449659.36977
80 1075525280.17011
80.3333333333333 1083598770.76185
80.6666666666667 1091697823.85678
81 1099820309.24631
81.3333333333333 1107951315.47023
81.6666666666667 1116026936.27057
82 1124104687.27951
82.3333333333333 1132201610.16584
82.6666666666667 1140260189.29739
83 1148344330.93212
83.3333333333333 1156426342.35826
83.6666666666667 1164499832.95
84 1172556281.87295
84.3333333333333 1180663855.80228
84.6666666666667 1188728825.55962
85 1196842790.11475
85.3333333333333 1204922671.33229
85.6666666666667 1212985510.88103
86 1221082433.76736
86.3333333333333 1229198528.53109
86.6666666666667 1237278409.74863
87 1245368942.00916
87.3333333333333 1253455213.8525
87.6666666666667 1261543615.90443
88 1269668231.50256
88.3333333333333 1277765154.38889
88.6666666666667 1285849296.02363
89 1293920656.40677
89.3333333333333 1301994146.99851
89.6666666666667 1310095330.30204
90 1318202904.23137
90.3333333333333 1326325389.6209
90.6666666666667 1334383968.75244
91 1342451068.71839
91.3333333333333 1350541600.97892
91.6666666666667 1358610831.15346
92 1366724795.70859
92.3333333333333 1374808937.34333
92.6666666666667 1382886688.35227
93 1390985741.4472
93.3333333333333 1399084794.54213
93.6666666666667 1407164675.75967
94 1415261598.646
94.3333333333333 1423322307.98615
94.6666666666667 1431370236.07469
95 1439452247.50083
95.3333333333333 1447532128.71837
95.6666666666667 1455597098.47571
96 1463681240.11045
96.3333333333333 1471741949.45059
96.6666666666667 1479843132.75412
97 1487903842.09427
97.3333333333333 1495990113.9376
97.6666666666667 1504080646.19814
98 1512162657.62427
98.3333333333333 1520255320.09341
98.6666666666667 1528350112.77114
99 1536440645.03168
99.3333333333333 1544516265.83202
99.6666666666667 1552602537.67535
100 1560669637.6413
100.333333333333 1568732477.19004
100.666666666667 1576795316.73878
101 1584890109.41652
101.333333333333 1592978511.46845
101.666666666667 1601062653.10319
102 1609174487.44972
102.333333333333 1617211764.49527
102.666666666667 1625323598.8418
103 1633407740.47653
103.333333333333 1641515314.40586
103.666666666667 1649588804.9976
104 1657724071.63873
104.333333333333 1665818864.31646
104.666666666667 1673932828.87159
105 1681972236.12574
105.333333333333 1690067028.80347
105.666666666667 1698140519.39521
106 1706222530.82135
106.333333333333 1714304542.24749
106.666666666667 1722390814.09082
107 1730485606.76856
107.333333333333 1738563357.77749
107.666666666667 1746660280.66383
108 1754761463.96736
108.333333333333 1762856256.64509
108.666666666667 1770944658.69703
109 1779026670.12317
109.333333333333 1787093770.08911
109.666666666667 1795192823.18404
110 1803249272.10699
110.333333333333 1811350455.41052
110.666666666667 1819432466.83666
111 1827518738.67999
111.333333333333 1835647614.69532
111.666666666667 1843753058.41605
112 1851845720.88518
112.333333333333 1859919211.47692
112.666666666667 1868039566.65785
113 1876142880.16998
113.333333333333 1884237672.84771
113.666666666667 1892317554.06525
114 1900403825.90859
114.333333333333 1908496488.37772
114.666666666667 1916597671.68126
115 1924709506.02778
115.333333333333 1932774475.78513
115.666666666667 1940873528.88006
116 1948942759.0546
116.333333333333 1957001338.18614
116.666666666667 1965096130.86388
117 1973195183.95881
117.333333333333 1981262283.92475
117.666666666667 1989335774.51649
118 1997415655.73403
118.333333333333 2005525359.87196
118.666666666667 2013575418.16911
119 2021661690.01244
119.333333333333 2029745831.64718
119.666666666667 2037838494.11631
120 2045929026.37685
120.333333333333 2053989735.71699
120.666666666667 2062099439.85492
121 2070177190.86386
121.333333333333 2078254941.8728
121.666666666667 2086349734.55053
122 2094440266.81107
122.333333333333 2102526538.6544
122.666666666667 2110614940.70634
123 2118703342.75828
123.333333333333 2126840739.608
123.666666666667 2134914230.19974
124 2143032455.17207
124.333333333333 2151088904.09501
124.666666666667 2159164524.89535
125 2167248666.53009
125.333333333333 2175298724.82723
125.666666666667 2183402038.33936
126 2191492570.5999
126.333333333333 2199595884.11203
126.666666666667 2207709848.66716
127 2215766297.5901
127.333333333333 2223890913.18823
127.666666666667 2231966533.98857
128 2240044284.99751
128.333333333333 2248111384.96345
128.666666666667 2256225349.51858
129 2264326532.82211
};
\addplot [semithick, color3,mark=triangle*, mark size=2.0, mark options={solid,fill=white}, mark repeat=15,mark phase=7]
table {%
0 0
0.333333333333333 3459072
0.666666666666667 11245568
1 19003392
1.33333333333333 26742784
1.66666666666667 34519040
2 42256384
2.33333333333333 50014208
2.66666666666667 57755648
3 65519616
3.33333333333333 73287680
3.66666666666667 81049600
4 88797184
4.33333333333333 96550912
4.66666666666667 104294400
5 112048128
5.33333333333333 119816192
5.66666666666667 127614976
6 135405568
6.33333333333333 143171584
6.66666666666667 150953984
7 158730240
7.33333333333333 166486016
7.66666666666667 174245888
8 181993472
8.33333333333333 189777920
8.66666666666667 197527552
9 205277184
9.33333333333333 213069824
9.66666666666667 220846080
10 220846080
10.3333333333333 225171456
10.6666666666667 232335360
11 239544320
11.3333333333333 246712320
11.6666666666667 253810688
12 260876288
12.3333333333333 267876352
12.6666666666667 274843648
13 281823232
13.3333333333333 288837632
13.6666666666667 295837696
14 302753792
14.3333333333333 309659648
14.6666666666667 316579840
15 323438592
15.3333333333333 330356736
15.6666666666667 337250304
16 344115200
16.3333333333333 350963712
16.6666666666667 357808128
17 364650496
17.3333333333333 371499008
17.6666666666667 378314752
18 385130496
18.3333333333333 391927808
18.6666666666667 398729216
19 405542912
19.3333333333333 412379136
19.6666666666667 419194880
20 425963520
20.3333333333333 432775168
20.6666666666667 440076288
21 447836160
21.3333333333333 455628800
21.6666666666667 463390720
22 471123968
22.3333333333333 478875648
22.6666666666667 486633472
23 494376960
23.3333333333333 502124544
23.6666666666667 509933568
24 517709824
24.3333333333333 525467648
24.6666666666667 533245952
25 540997632
25.3333333333333 548755456
25.6666666666667 556511232
26 564289536
26.3333333333333 572053504
26.6666666666667 579807232
27 587606016
27.3333333333333 595408896
27.6666666666667 603179008
28 610973696
28.3333333333333 618786816
28.6666666666667 626608128
29 634421248
29.3333333333333 642215936
29.6666666666667 650012672
30 657807360
30.3333333333333 665587712
30.6666666666667 673380352
31 681185280
31.3333333333333 688967680
31.6666666666667 696752128
32 704559104
32.3333333333333 712366080
32.6666666666667 720205824
33 728016896
33.3333333333333 735807488
33.6666666666667 743600128
34 751384576
34.3333333333333 759216128
34.6666666666667 767006720
35 774803456
35.3333333333333 782604288
35.6666666666667 790407168
36 798164992
36.3333333333333 805937152
36.6666666666667 813711360
37 821465088
37.3333333333333 829204480
37.6666666666667 836962304
38 844748800
38.3333333333333 852508672
38.6666666666667 860256256
39 867991552
39.3333333333333 875720704
39.6666666666667 883474432
40 891195392
40.3333333333333 898957312
40.6666666666667 906719232
41 914493440
41.3333333333333 922263552
41.6666666666667 930037760
42 937799680
42.3333333333333 945596416
42.6666666666667 953352192
43 961085440
43.3333333333333 968867840
43.6666666666667 976631808
44 984360960
44.3333333333333 992135168
44.6666666666667 999936000
45 1007749120
45.3333333333333 1015549952
45.6666666666667 1023342592
46 1031104512
46.3333333333333 1038893056
46.6666666666667 1046659072
47 1054408704
47.3333333333333 1062180864
47.6666666666667 1069983744
48 1077762048
48.3333333333333 1085534208
48.6666666666667 1093292032
49 1101056000
49.3333333333333 1108828160
49.6666666666667 1116588032
50 1124370432
50.3333333333333 1132138496
50.6666666666667 1139937280
51 1147695104
51.3333333333333 1155461120
51.6666666666667 1163278336
52 1171058688
52.3333333333333 1178828800
52.6666666666667 1186562048
53 1194356736
53.3333333333333 1202120704
53.6666666666667 1209911296
54 1217695744
54.3333333333333 1225422848
54.6666666666667 1233195008
55 1240975360
55.3333333333333 1248753664
55.6666666666667 1256517632
56 1264283648
56.3333333333333 1272055808
56.6666666666667 1279805440
57 1287563264
57.3333333333333 1295347712
57.6666666666667 1303115776
58 1310869504
58.3333333333333 1318660096
58.6666666666667 1326428160
59 1334212608
59.3333333333333 1341992960
59.6666666666667 1349767168
60 1357535232
60.3333333333333 1365297152
60.6666666666667 1373071360
61 1380868096
61.3333333333333 1388679168
61.6666666666667 1396455424
62 1404241920
62.3333333333333 1412022272
62.6666666666667 1419790336
63 1427566592
63.3333333333333 1435344896
63.6666666666667 1443096576
64 1450860544
64.3333333333333 1458644992
64.6666666666667 1466400768
65 1474168832
65.3333333333333 1481926656
65.6666666666667 1489707008
66 1497487360
66.3333333333333 1505280000
66.6666666666667 1513048064
67 1520812032
67.3333333333333 1528584192
67.6666666666667 1536366592
68 1544138752
68.3333333333333 1551900672
68.6666666666667 1559646208
69 1567401984
69.3333333333333 1575174144
69.6666666666667 1582950400
70 1590726656
70.3333333333333 1598521344
70.6666666666667 1606313984
71 1614090240
71.3333333333333 1621872640
71.6666666666667 1629652992
72 1637421056
72.3333333333333 1645185024
72.6666666666667 1652955136
73 1660743680
73.3333333333333 1668526080
73.6666666666667 1676318720
74 1684076544
74.3333333333333 1691889664
74.6666666666667 1699657728
75 1707411456
75.3333333333333 1715163136
75.6666666666667 1722955776
76 1730738176
76.3333333333333 1738506240
76.6666666666667 1746259968
77 1754042368
77.3333333333333 1761814528
77.6666666666667 1769621504
78 1777405952
78.3333333333333 1785182208
78.6666666666667 1792985088
79 1800751104
79.3333333333333 1808531456
79.6666666666667 1816297472
80 1824063488
80.3333333333333 1831870464
80.6666666666667 1839628288
81 1847406592
81.3333333333333 1855156224
81.6666666666667 1862928384
82 1870704640
82.3333333333333 1878468608
82.6666666666667 1886236672
83 1894023168
83.3333333333333 1901793280
83.6666666666667 1909532672
84 1917304832
84.3333333333333 1925085184
84.6666666666667 1932869632
85 1940625408
85.3333333333333 1948401664
85.6666666666667 1956206592
86 1963995136
86.3333333333333 1971765248
86.6666666666667 1979514880
87 1987260416
87.3333333333333 1995034624
87.6666666666667 2002776064
88 2010544128
88.3333333333333 2018316288
88.6666666666667 2026072064
89 2033840128
89.3333333333333 2041624576
89.6666666666667 2049390592
90 2057181184
90.3333333333333 2064996352
90.6666666666667 2072770560
91 2080542720
91.3333333333333 2088323072
91.6666666666667 2096068608
92 2103805952
92.3333333333333 2111574016
92.6666666666667 2119335936
93 2127095808
93.3333333333333 2134867968
93.6666666666667 2142631936
94 2150410240
94.3333333333333 2158192640
94.6666666666667 2166003712
95 2173790208
95.3333333333333 2181562368
95.6666666666667 2189352960
96 2197131264
96.3333333333333 2204930048
96.6666666666667 2212716544
97 2220505088
97.3333333333333 2228287488
97.6666666666667 2236073984
98 2243872768
98.3333333333333 2251665408
98.6666666666667 2259427328
99 2267199488
99.3333333333333 2274961408
99.6666666666667 2282727424
100 2290532352
100.333333333333 2298347520
100.666666666667 2306111488
101 2313842688
101.333333333333 2321633280
101.666666666667 2329419776
102 2337202176
102.333333333333 2344955904
102.666666666667 2352730112
103 2360535040
103.333333333333 2368327680
103.666666666667 2376110080
104 2383892480
104.333333333333 2391652352
104.666666666667 2399434752
105 2407227392
105.333333333333 2415003648
105.666666666667 2422818816
106 2430590976
106.333333333333 2438402048
106.666666666667 2446170112
107 2453958656
107.333333333333 2461691904
107.666666666667 2469449728
108 2477217792
108.333333333333 2484987904
108.666666666667 2492801024
109 2500521984
109.333333333333 2508285952
109.666666666667 2516088832
110 2523885568
110.333333333333 2531680256
110.666666666667 2539468800
111 2547210240
111.333333333333 2554974208
111.666666666667 2562760704
112 2570520576
112.333333333333 2578305024
112.666666666667 2586114048
113 2593867776
113.333333333333 2601652224
113.666666666667 2609424384
114 2617192448
114.333333333333 2624968704
114.666666666667 2632744960
115 2640533504
115.333333333333 2648301568
115.666666666667 2656067584
116 2656454656
};
\addplot [semithick, color4,mark=diamond*, mark size=2.0, mark options={solid,fill=white}, mark repeat=15,mark phase=30]
table {%
0 7731200
0.333333333333333 15509504
0.666666666666667 23281664
1 31131648
1.33333333333333 38903808
1.66666666666667 46690304
2 54474752
2.33333333333333 62197760
2.66666666666667 69953536
3 77780992
3.33333333333333 85608448
3.66666666666667 93448192
4 101322752
4.33333333333333 109115392
4.66666666666667 116965376
5 124737536
5.33333333333333 132515840
5.66666666666667 140298240
6 148049920
6.33333333333333 155774976
6.66666666666667 163530752
7 171290624
7.33333333333333 179040256
7.66666666666667 186855424
8 194670592
8.33333333333333 202450944
8.66666666666667 210251776
9 217982976
9.33333333333333 225716224
9.66666666666667 233502720
10 233502720
10.3333333333333 239151104
10.6666666666667 246534144
11 253724672
11.3333333333333 260878336
11.6666666666667 267964416
12 274941952
12.3333333333333 281888768
12.6666666666667 288847872
13 295909376
13.3333333333333 302929920
13.6666666666667 309852160
14 316731392
14.3333333333333 323575808
14.6666666666667 330444800
15 337326080
15.3333333333333 344164352
15.6666666666667 350980096
16 357900288
16.3333333333333 364777472
16.6666666666667 371617792
17 378458112
17.3333333333333 385314816
17.6666666666667 392087552
18 398839808
18.3333333333333 405673984
18.6666666666667 412428288
19 419166208
19.3333333333333 426012672
19.6666666666667 432859136
20 439691264
20.3333333333333 446545920
20.6666666666667 453408768
21 460124160
21.3333333333333 466831360
21.6666666666667 473534464
22 480329728
22.3333333333333 487114752
22.6666666666667 494071808
23 500934656
23.3333333333333 507799552
23.6666666666667 514719744
24 521637888
24.3333333333333 528486400
24.6666666666667 535324672
25 542169088
25.3333333333333 548954112
25.6666666666667 555732992
26 562503680
26.3333333333333 569300992
26.6666666666667 576065536
27 582832128
27.3333333333333 589598720
27.6666666666667 596330496
28 603138048
28.3333333333333 609918976
28.6666666666667 616734720
29 624039936
29.3333333333333 631820288
29.6666666666667 639565824
30 647403520
30.3333333333333 655241216
30.6666666666667 663101440
31 670873600
31.3333333333333 678647808
31.6666666666667 686401536
32 694149120
32.3333333333333 701935616
32.6666666666667 709763072
33 717604864
33.3333333333333 725446656
33.6666666666667 733304832
34 741115904
34.3333333333333 748926976
34.6666666666667 756692992
35 764471296
35.3333333333333 772243456
35.6666666666667 780093440
36 787865600
36.3333333333333 795652096
36.6666666666667 803436544
37 811159552
37.3333333333333 818909184
37.6666666666667 826701824
38 834494464
38.3333333333333 842233856
38.6666666666667 850016256
39 857776128
39.3333333333333 865554432
39.6666666666667 873316352
40 881076224
40.3333333333333 888850432
40.6666666666667 896645120
41 904413184
41.3333333333333 912185344
41.6666666666667 919967744
42 927725568
42.3333333333333 935514112
42.6666666666667 943300608
43 951109632
43.3333333333333 958898176
43.6666666666667 966682624
44 974456832
44.3333333333333 982245376
44.6666666666667 990007296
45 997789696
45.3333333333333 1005563904
45.6666666666667 1013331968
46 1021108224
46.3333333333333 1028886528
46.6666666666667 1036683264
47 1044469760
47.3333333333333 1052262400
47.6666666666667 1060050944
48 1067841536
48.3333333333333 1075582976
48.6666666666667 1083361280
49 1091143680
49.3333333333333 1098938368
49.6666666666667 1106704384
50 1114513408
50.3333333333333 1122322432
50.6666666666667 1130100736
51 1137899520
51.3333333333333 1145669632
51.6666666666667 1153419264
52 1161185280
52.3333333333333 1168965632
52.6666666666667 1176733696
53 1184530432
53.3333333333333 1192327168
53.6666666666667 1200138240
54 1207898112
54.3333333333333 1215674368
54.6666666666667 1223458816
55 1231249408
55.3333333333333 1239027712
55.6666666666667 1246814208
56 1254602752
56.3333333333333 1262381056
56.6666666666667 1270153216
57 1277941760
57.3333333333333 1285683200
57.6666666666667 1293443072
58 1301227520
58.3333333333333 1309014016
58.6666666666667 1316777984
59 1324546048
59.3333333333333 1332322304
59.6666666666667 1340119040
60 1347885056
60.3333333333333 1355669504
60.6666666666667 1363439616
61 1371215872
61.3333333333333 1379024896
61.6666666666667 1386840064
62 1394612224
62.3333333333333 1402368000
62.6666666666667 1410146304
63 1417932800
63.3333333333333 1425702912
63.6666666666667 1433473024
64 1441222656
64.3333333333333 1449035776
64.6666666666667 1456783360
65 1464567808
65.3333333333333 1472339968
65.6666666666667 1480112128
66 1487896576
66.3333333333333 1495670784
66.6666666666667 1503426560
67 1511204864
67.3333333333333 1518977024
67.6666666666667 1526753280
68 1534504960
68.3333333333333 1542293504
68.6666666666667 1550059520
69 1557854208
69.3333333333333 1565632512
69.6666666666667 1573392384
70 1581125632
70.3333333333333 1588895744
70.6666666666667 1596651520
71 1604425728
71.3333333333333 1612179456
71.6666666666667 1619974144
72 1627738112
72.3333333333333 1635530752
72.6666666666667 1643317248
73 1651054592
73.3333333333333 1658789888
73.6666666666667 1666555904
74 1674309632
74.3333333333333 1682069504
74.6666666666667 1689862144
75 1697644544
75.3333333333333 1705439232
75.6666666666667 1713207296
76 1720981504
76.3333333333333 1728749568
76.6666666666667 1736519680
77 1744289792
77.3333333333333 1752064000
77.6666666666667 1759858688
78 1767636992
78.3333333333333 1775407104
78.6666666666667 1783142400
79 1790943232
79.3333333333333 1798715392
79.6666666666667 1806473216
80 1814269952
80.3333333333333 1822068736
80.6666666666667 1829853184
81 1837637632
81.3333333333333 1845428224
81.6666666666667 1853171712
82 1860909056
82.3333333333333 1868675072
82.6666666666667 1876453376
83 1884223488
83.3333333333333 1892018176
83.6666666666667 1899786240
84 1907597312
84.3333333333333 1915369472
84.6666666666667 1923123200
85 1930862592
85.3333333333333 1938644992
85.6666666666667 1946415104
86 1954191360
86.3333333333333 1961965568
86.6666666666667 1969739776
87 1977507840
87.3333333333333 1985269760
87.6666666666667 1993048064
88 2000816128
88.3333333333333 2008565760
88.6666666666667 2016335872
89 2024105984
89.3333333333333 2031894528
89.6666666666667 2039648256
90 2047397888
90.3333333333333 2055168000
90.6666666666667 2062934016
91 2070718464
91.3333333333333 2078470144
91.6666666666667 2086256640
92 2094026752
92.3333333333333 2101796864
92.6666666666667 2109569024
93 2117335040
93.3333333333333 2125096960
93.6666666666667 2132908032
94 2140678144
94.3333333333333 2148442112
94.6666666666667 2156210176
95 2163970048
95.3333333333333 2171736064
95.6666666666667 2179518464
96 2187298816
96.3333333333333 2195060736
96.6666666666667 2202843136
97 2210596864
97.3333333333333 2218352640
97.6666666666667 2226126848
98 2233886720
98.3333333333333 2241650688
98.6666666666667 2249447424
99 2257238016
99.3333333333333 2265016320
99.6666666666667 2272811008
100 2280622080
100.333333333333 2288377856
100.666666666667 2296164352
101 2303963136
101.333333333333 2311745536
101.666666666667 2319536128
102 2327308288
102.333333333333 2335094784
102.666666666667 2342875136
103 2350657536
103.333333333333 2358392832
103.666666666667 2366144512
};


==> figures/evaluation/data/recovery/criteo-4x/tput.tex <==
\addplot [semithick, color0,mark=*, mark size=1.5, mark options={solid,fill=white}, mark repeat=15,mark phase=3]
table {%
0 404313.592166814
0.333333333333333 404207.081736844
0.666666666666667 403354.998297082
1 404100.571306874
1.33333333333333 405591.717326456
1.66666666666667 404633.123456724
2 405378.696466516
2.33333333333333 405378.696466516
2.66666666666667 402715.935717261
3 406337.290336247
3.33333333333333 403035.467007172
3.66666666666667 403248.487867112
4 403994.060876903
4.33333333333333 403248.487867112
4.66666666666667 404846.144316665
5 403781.040016963
5.33333333333333 403994.060876903
5.66666666666667 404952.654746635
6 405272.186036546
6.33333333333333 404420.102596784
6.66666666666667 406230.779906277
7 404846.144316665
7.33333333333333 404420.102596784
7.66666666666667 403035.467007172
8 404420.102596784
8.33333333333333 404420.102596784
8.66666666666667 404739.633886695
9 405059.165176605
9.33333333333333 403994.060876903
9.66666666666667 404207.081736844
10 0
10.3333333333333 0
10.6666666666667 0
11 0
11.3333333333333 0
11.6666666666667 0
12 0
12.3333333333333 0
12.6666666666667 0
13 0
13.3333333333333 0
13.6666666666667 0
14 0
14.3333333333333 0
14.6666666666667 0
15 0
15.3333333333333 0
15.6666666666667 0
16 405698.227756426
16.3333333333333 402822.446147231
16.6666666666667 403354.998297082
17 405272.186036546
17.3333333333333 404952.654746635
17.6666666666667 405485.206896486
18 403887.550446933
18.3333333333333 403674.529586993
18.6666666666667 403568.019157023
19 404739.633886695
19.3333333333333 406230.779906277
19.6666666666667 405165.675606575
20 405378.696466516
20.3333333333333 401757.34184753
20.6666666666667 405165.675606575
21 404207.081736844
21.3333333333333 403994.060876903
21.6666666666667 403461.508727052
22 406763.332056128
22.3333333333333 404846.144316665
22.6666666666667 403461.508727052
23 402609.425287291
23.3333333333333 404633.123456724
23.6666666666667 403461.508727052
24 404207.081736844
24.3333333333333 405272.186036546
24.6666666666667 405272.186036546
25 404313.592166814
25.3333333333333 406656.821626158
25.6666666666667 405165.675606575
26 404420.102596784
26.3333333333333 406763.332056128
26.6666666666667 402822.446147231
27 404420.102596784
27.3333333333333 404846.144316665
27.6666666666667 402928.956577202
28 405165.675606575
28.3333333333333 404313.592166814
28.6666666666667 404526.613026754
29 403674.529586993
29.3333333333333 403674.529586993
29.6666666666667 402928.956577202
30 405165.675606575
30.3333333333333 404100.571306874
30.6666666666667 403887.550446933
31 403354.998297082
31.3333333333333 404100.571306874
31.6666666666667 405591.717326456
32 405591.717326456
32.3333333333333 406869.842486098
32.6666666666667 405485.206896486
33 403781.040016963
33.3333333333333 402822.446147231
33.6666666666667 404739.633886695
34 402289.89399738
34.3333333333333 403781.040016963
34.6666666666667 404420.102596784
35 403674.529586993
35.3333333333333 406230.779906277
35.6666666666667 403141.977437142
36 404952.654746635
36.3333333333333 405059.165176605
36.6666666666667 403461.508727052
37 404952.654746635
37.3333333333333 404633.123456724
37.6666666666667 404313.592166814
38 403674.529586993
38.3333333333333 403568.019157023
38.6666666666667 403994.060876903
39 402822.446147231
39.3333333333333 404420.102596784
39.6666666666667 401863.8522775
40 404633.123456724
40.3333333333333 406550.311196188
40.6666666666667 402822.446147231
41 403887.550446933
41.3333333333333 405591.717326456
41.6666666666667 406976.352916069
42 404313.592166814
42.3333333333333 404207.081736844
42.6666666666667 404846.144316665
43 403035.467007172
43.3333333333333 404526.613026754
43.6666666666667 404420.102596784
44 406124.269476307
44.3333333333333 405911.248616367
44.6666666666667 402928.956577202
45 403674.529586993
45.3333333333333 404207.081736844
45.6666666666667 402076.87313744
46 402822.446147231
46.3333333333333 403354.998297082
46.6666666666667 405272.186036546
47 405804.738186396
47.3333333333333 403248.487867112
47.6666666666667 403781.040016963
48 404313.592166814
48.3333333333333 405059.165176605
48.6666666666667 404526.613026754
49 403035.467007172
49.3333333333333 404313.592166814
49.6666666666667 405165.675606575
50 403035.467007172
50.3333333333333 405272.186036546
50.6666666666667 404313.592166814
51 403141.977437142
51.3333333333333 403461.508727052
51.6666666666667 404952.654746635
52 404420.102596784
52.3333333333333 402715.935717261
52.6666666666667 406017.759046337
53 403141.977437142
53.3333333333333 404420.102596784
53.6666666666667 404739.633886695
54 404526.613026754
54.3333333333333 403568.019157023
54.6666666666667 404420.102596784
55 403674.529586993
55.3333333333333 406124.269476307
55.6666666666667 404420.102596784
56 404313.592166814
56.3333333333333 402822.446147231
56.6666666666667 403994.060876903
57 405378.696466516
57.3333333333333 403141.977437142
57.6666666666667 403887.550446933
58 403568.019157023
58.3333333333333 406230.779906277
58.6666666666667 402289.89399738
59 403781.040016963
59.3333333333333 405485.206896486
59.6666666666667 403568.019157023
60 404526.613026754
60.3333333333333 406017.759046337
60.6666666666667 401437.810557619
61 403781.040016963
61.3333333333333 404952.654746635
61.6666666666667 405591.717326456
62 404846.144316665
62.3333333333333 404100.571306874
62.6666666666667 405485.206896486
63 405591.717326456
63.3333333333333 404313.592166814
63.6666666666667 403141.977437142
64 404207.081736844
64.3333333333333 404633.123456724
64.6666666666667 404739.633886695
65 406017.759046337
65.3333333333333 403568.019157023
65.6666666666667 404526.613026754
66 404846.144316665
66.3333333333333 403674.529586993
66.6666666666667 402183.38356741
67 403568.019157023
67.3333333333333 404100.571306874
67.6666666666667 403887.550446933
68 405165.675606575
68.3333333333333 404100.571306874
68.6666666666667 403248.487867112
69 402928.956577202
69.3333333333333 404633.123456724
69.6666666666667 403568.019157023
70 402076.87313744
70.3333333333333 403994.060876903
70.6666666666667 404100.571306874
71 403994.060876903
71.3333333333333 403887.550446933
71.6666666666667 404420.102596784
72 406017.759046337
72.3333333333333 403354.998297082
72.6666666666667 404526.613026754
73 403035.467007172
73.3333333333333 405378.696466516
73.6666666666667 403354.998297082
74 404952.654746635
74.3333333333333 404207.081736844
74.6666666666667 406124.269476307
75 404100.571306874
75.3333333333333 403781.040016963
75.6666666666667 404952.654746635
76 403568.019157023
76.3333333333333 404207.081736844
76.6666666666667 403674.529586993
77 403568.019157023
77.3333333333333 404952.654746635
77.6666666666667 404100.571306874
78 403461.508727052
78.3333333333333 404420.102596784
78.6666666666667 406763.332056128
79 404846.144316665
79.3333333333333 402822.446147231
79.6666666666667 402928.956577202
80 404420.102596784
80.3333333333333 404846.144316665
80.6666666666667 403141.977437142
81 405485.206896486
81.3333333333333 403568.019157023
81.6666666666667 403781.040016963
82 403781.040016963
82.3333333333333 404420.102596784
82.6666666666667 405804.738186396
83 405591.717326456
83.3333333333333 404952.654746635
83.6666666666667 404313.592166814
84 403141.977437142
84.3333333333333 403141.977437142
84.6666666666667 403354.998297082
85 403781.040016963
85.3333333333333 404846.144316665
85.6666666666667 405485.206896486
86 404633.123456724
86.3333333333333 403248.487867112
86.6666666666667 405591.717326456
87 403035.467007172
87.3333333333333 404952.654746635
87.6666666666667 405911.248616367
88 404313.592166814
88.3333333333333 404846.144316665
88.6666666666667 404526.613026754
89 403994.060876903
89.3333333333333 403994.060876903
89.6666666666667 402183.38356741
90 404100.571306874
90.3333333333333 405165.675606575
90.6666666666667 403461.508727052
91 404846.144316665
91.3333333333333 403887.550446933
91.6666666666667 403887.550446933
92 404313.592166814
92.3333333333333 401970.36270747
92.6666666666667 406550.311196188
93 403354.998297082
93.3333333333333 404952.654746635
93.6666666666667 404207.081736844
94 403141.977437142
94.3333333333333 403887.550446933
94.6666666666667 403674.529586993
95 405272.186036546
95.3333333333333 404100.571306874
95.6666666666667 405165.675606575
96 404739.633886695
96.3333333333333 403887.550446933
96.6666666666667 403248.487867112
97 404420.102596784
97.3333333333333 403248.487867112
97.6666666666667 406124.269476307
98 403568.019157023
98.3333333333333 404846.144316665
98.6666666666667 403035.467007172
99 404952.654746635
};
\addlegendentry{\ckptThirty best}
\addplot [semithick, color1,mark=square*, mark size=1.5, mark options={solid,fill=white}, mark repeat=15,mark phase=9]
table {%
0 404313.592166814
0.333333333333333 404207.081736844
0.666666666666667 403354.998297082
1 404100.571306874
1.33333333333333 405591.717326456
1.66666666666667 404633.123456724
2 405378.696466516
2.33333333333333 405378.696466516
2.66666666666667 402715.935717261
3 406337.290336247
3.33333333333333 403035.467007172
3.66666666666667 403248.487867112
4 403994.060876903
4.33333333333333 403248.487867112
4.66666666666667 404846.144316665
5 403781.040016963
5.33333333333333 403994.060876903
5.66666666666667 404952.654746635
6 405272.186036546
6.33333333333333 404420.102596784
6.66666666666667 406230.779906277
7 404846.144316665
7.33333333333333 404420.102596784
7.66666666666667 403035.467007172
8 404420.102596784
8.33333333333333 404420.102596784
8.66666666666667 404739.633886695
9 405059.165176605
9.33333333333333 403994.060876903
9.66666666666667 404207.081736844
10 0
10.3333333333333 0
10.6666666666667 0
11 0
11.3333333333333 0
11.6666666666667 0
12 0
12.3333333333333 0
12.6666666666667 0
13 0
13.3333333333333 0
13.6666666666667 0
14 0
14.3333333333333 0
14.6666666666667 0
15 0
15.3333333333333 0
15.6666666666667 0
16 0
16.3333333333333 0
16.6666666666667 0
17 0
17.3333333333333 0
17.6666666666667 0
18 0
18.3333333333333 0
18.6666666666667 0
19 0
19.3333333333333 0
19.6666666666667 0
20 0
20.3333333333333 0
20.6666666666667 0
21 0
21.3333333333333 0
21.6666666666667 0
22 0
22.3333333333333 0
22.6666666666667 0
23 0
23.3333333333333 0
23.6666666666667 0
24 0
24.3333333333333 0
24.6666666666667 0
25 0
25.3333333333333 0
25.6666666666667 0
26 0
26.3333333333333 0
26.6666666666667 0
27 0
27.3333333333333 0
27.6666666666667 0
28 0
28.3333333333333 0
28.6666666666667 0
29 0
29.3333333333333 0
29.6666666666667 0
30 0
30.3333333333333 0
30.6666666666667 0
31 404633.123456724
31.3333333333333 404420.102596784
31.6666666666667 403887.550446933
32 402289.89399738
32.3333333333333 405698.227756426
32.6666666666667 404526.613026754
33 405911.248616367
33.3333333333333 404952.654746635
33.6666666666667 404526.613026754
34 403887.550446933
34.3333333333333 403248.487867112
34.6666666666667 405165.675606575
35 407295.884205979
35.3333333333333 402822.446147231
35.6666666666667 402928.956577202
36 403994.060876903
36.3333333333333 404526.613026754
36.6666666666667 405165.675606575
37 406976.352916069
37.3333333333333 404420.102596784
37.6666666666667 405911.248616367
38 405591.717326456
38.3333333333333 403035.467007172
38.6666666666667 404846.144316665
39 405059.165176605
39.3333333333333 403568.019157023
39.6666666666667 404420.102596784
40 404420.102596784
40.3333333333333 403354.998297082
40.6666666666667 404100.571306874
41 404633.123456724
41.3333333333333 405591.717326456
41.6666666666667 403674.529586993
42 403994.060876903
42.3333333333333 404739.633886695
42.6666666666667 403035.467007172
43 405165.675606575
43.3333333333333 405911.248616367
43.6666666666667 404526.613026754
44 404633.123456724
44.3333333333333 404952.654746635
44.6666666666667 406337.290336247
45 403781.040016963
45.3333333333333 405591.717326456
45.6666666666667 404100.571306874
46 406017.759046337
46.3333333333333 404846.144316665
46.6666666666667 403354.998297082
47 404526.613026754
47.3333333333333 403781.040016963
47.6666666666667 404952.654746635
48 403887.550446933
48.3333333333333 404952.654746635
48.6666666666667 403781.040016963
49 406124.269476307
49.3333333333333 405698.227756426
49.6666666666667 403674.529586993
50 402928.956577202
50.3333333333333 405698.227756426
50.6666666666667 403354.998297082
51 404952.654746635
51.3333333333333 404952.654746635
51.6666666666667 405378.696466516
52 406550.311196188
52.3333333333333 405272.186036546
52.6666666666667 402396.404427351
53 404100.571306874
53.3333333333333 404420.102596784
53.6666666666667 403461.508727052
54 405165.675606575
54.3333333333333 404739.633886695
54.6666666666667 404526.613026754
55 403994.060876903
55.3333333333333 404100.571306874
55.6666666666667 402822.446147231
56 404313.592166814
56.3333333333333 404313.592166814
56.6666666666667 402396.404427351
57 403035.467007172
57.3333333333333 403887.550446933
57.6666666666667 404207.081736844
58 402396.404427351
58.3333333333333 403994.060876903
58.6666666666667 403781.040016963
59 403887.550446933
59.3333333333333 404207.081736844
59.6666666666667 402502.914857321
60 404739.633886695
60.3333333333333 406017.759046337
60.6666666666667 403141.977437142
61 406017.759046337
61.3333333333333 404952.654746635
61.6666666666667 402928.956577202
62 404952.654746635
62.3333333333333 406230.779906277
62.6666666666667 403887.550446933
63 403674.529586993
63.3333333333333 404420.102596784
63.6666666666667 406124.269476307
64 404420.102596784
64.3333333333333 403781.040016963
64.6666666666667 405165.675606575
65 401863.8522775
65.3333333333333 405804.738186396
65.6666666666667 405272.186036546
66 401970.36270747
66.3333333333333 405059.165176605
66.6666666666667 403781.040016963
67 405272.186036546
67.3333333333333 404207.081736844
67.6666666666667 405804.738186396
68 402928.956577202
68.3333333333333 403994.060876903
68.6666666666667 402822.446147231
69 403887.550446933
69.3333333333333 406443.800766218
69.6666666666667 403248.487867112
70 403248.487867112
70.3333333333333 404100.571306874
70.6666666666667 405804.738186396
71 404633.123456724
71.3333333333333 404207.081736844
71.6666666666667 405165.675606575
72 404420.102596784
72.3333333333333 404313.592166814
72.6666666666667 404633.123456724
73 403354.998297082
73.3333333333333 404739.633886695
73.6666666666667 404100.571306874
74 405165.675606575
74.3333333333333 404100.571306874
74.6666666666667 403674.529586993
75 405165.675606575
75.3333333333333 403887.550446933
75.6666666666667 404313.592166814
76 405165.675606575
76.3333333333333 404952.654746635
76.6666666666667 403674.529586993
77 404313.592166814
77.3333333333333 405698.227756426
77.6666666666667 405591.717326456
78 403354.998297082
78.3333333333333 404420.102596784
78.6666666666667 405591.717326456
79 406550.311196188
79.3333333333333 403461.508727052
79.6666666666667 404207.081736844
80 402822.446147231
80.3333333333333 404100.571306874
80.6666666666667 404207.081736844
81 402715.935717261
81.3333333333333 403248.487867112
81.6666666666667 404633.123456724
82 405165.675606575
82.3333333333333 403674.529586993
82.6666666666667 405591.717326456
83 404207.081736844
83.3333333333333 403035.467007172
83.6666666666667 404420.102596784
84 403887.550446933
84.3333333333333 404313.592166814
84.6666666666667 403994.060876903
85 404420.102596784
85.3333333333333 402715.935717261
85.6666666666667 404420.102596784
86 403354.998297082
86.3333333333333 405272.186036546
86.6666666666667 404313.592166814
87 402076.87313744
87.3333333333333 405165.675606575
87.6666666666667 403781.040016963
88 403035.467007172
88.3333333333333 404313.592166814
88.6666666666667 405165.675606575
89 404846.144316665
89.3333333333333 404313.592166814
89.6666666666667 406230.779906277
90 405378.696466516
90.3333333333333 404526.613026754
90.6666666666667 405591.717326456
91 405059.165176605
91.3333333333333 405272.186036546
91.6666666666667 404846.144316665
92 403887.550446933
92.3333333333333 404846.144316665
92.6666666666667 405591.717326456
93 404313.592166814
93.3333333333333 404846.144316665
93.6666666666667 404846.144316665
94 404739.633886695
94.3333333333333 403354.998297082
94.6666666666667 403141.977437142
95 404846.144316665
95.3333333333333 402822.446147231
95.6666666666667 405165.675606575
96 405804.738186396
96.3333333333333 403994.060876903
96.6666666666667 404526.613026754
97 402822.446147231
97.3333333333333 405804.738186396
97.6666666666667 403248.487867112
98 405165.675606575
98.3333333333333 403568.019157023
98.6666666666667 403674.529586993
99 402928.956577202
99.3333333333333 403674.529586993
99.6666666666667 404846.144316665
100 406337.290336247
100.333333333333 403461.508727052
100.666666666667 403035.467007172
101 404313.592166814
101.333333333333 404846.144316665
101.666666666667 405911.248616367
102 404526.613026754
102.333333333333 404420.102596784
102.666666666667 406017.759046337
103 405165.675606575
103.333333333333 405698.227756426
103.666666666667 403781.040016963
104 404846.144316665
104.333333333333 404100.571306874
104.666666666667 403674.529586993
105 403248.487867112
105.333333333333 405911.248616367
105.666666666667 404313.592166814
106 403994.060876903
106.333333333333 402502.914857321
106.666666666667 404526.613026754
107 404100.571306874
107.333333333333 404952.654746635
107.666666666667 404420.102596784
108 405698.227756426
108.333333333333 404633.123456724
108.666666666667 403781.040016963
109 406124.269476307
109.333333333333 403781.040016963
109.666666666667 406337.290336247
110 404739.633886695
110.333333333333 403887.550446933
110.666666666667 403248.487867112
111 406124.269476307
111.333333333333 403674.529586993
111.666666666667 402928.956577202
112 402715.935717261
112.333333333333 403461.508727052
112.666666666667 404633.123456724
113 405911.248616367
113.333333333333 404313.592166814
113.666666666667 402183.38356741
114 404739.633886695
};
\addlegendentry{\ckptThirty average}
\addplot [semithick, color2,mark=x, mark size=1.8, mark options={solid,fill=white}, mark repeat=15,mark phase=13]
table {%
0 404313.592166814
0.333333333333333 404207.081736844
0.666666666666667 403354.998297082
1 404100.571306874
1.33333333333333 405591.717326456
1.66666666666667 404633.123456724
2 405378.696466516
2.33333333333333 405378.696466516
2.66666666666667 402715.935717261
3 406337.290336247
3.33333333333333 403035.467007172
3.66666666666667 403248.487867112
4 403994.060876903
4.33333333333333 403248.487867112
4.66666666666667 404846.144316665
5 403781.040016963
5.33333333333333 403994.060876903
5.66666666666667 404952.654746635
6 405272.186036546
6.33333333333333 404420.102596784
6.66666666666667 406230.779906277
7 404846.144316665
7.33333333333333 404420.102596784
7.66666666666667 403035.467007172
8 404420.102596784
8.33333333333333 404420.102596784
8.66666666666667 404739.633886695
9 405059.165176605
9.33333333333333 403994.060876903
9.66666666666667 404207.081736844
10 0
10.3333333333333 0
10.6666666666667 0
11 0
11.3333333333333 0
11.6666666666667 0
12 0
12.3333333333333 0
12.6666666666667 0
13 0
13.3333333333333 0
13.6666666666667 0
14 0
14.3333333333333 0
14.6666666666667 0
15 0
15.3333333333333 0
15.6666666666667 0
16 0
16.3333333333333 0
16.6666666666667 0
17 0
17.3333333333333 0
17.6666666666667 0
18 0
18.3333333333333 0
18.6666666666667 0
19 0
19.3333333333333 0
19.6666666666667 0
20 0
20.3333333333333 0
20.6666666666667 0
21 0
21.3333333333333 0
21.6666666666667 0
22 0
22.3333333333333 0
22.6666666666667 0
23 0
23.3333333333333 0
23.6666666666667 0
24 0
24.3333333333333 0
24.6666666666667 0
25 0
25.3333333333333 0
25.6666666666667 0
26 0
26.3333333333333 0
26.6666666666667 0
27 0
27.3333333333333 0
27.6666666666667 0
28 0
28.3333333333333 0
28.6666666666667 0
29 0
29.3333333333333 0
29.6666666666667 0
30 0
30.3333333333333 0
30.6666666666667 0
31 0
31.3333333333333 0
31.6666666666667 0
32 0
32.3333333333333 0
32.6666666666667 0
33 0
33.3333333333333 0
33.6666666666667 0
34 0
34.3333333333333 0
34.6666666666667 0
35 0
35.3333333333333 0
35.6666666666667 0
36 0
36.3333333333333 0
36.6666666666667 0
37 0
37.3333333333333 0
37.6666666666667 0
38 0
38.3333333333333 0
38.6666666666667 0
39 0
39.3333333333333 0
39.6666666666667 0
40 0
40.3333333333333 0
40.6666666666667 0
41 0
41.3333333333333 0
41.6666666666667 0
42 0
42.3333333333333 0
42.6666666666667 0
43 0
43.3333333333333 0
43.6666666666667 0
44 0
44.3333333333333 0
44.6666666666667 0
45 0
45.3333333333333 0
45.6666666666667 0
46 404739.633886695
46.3333333333333 405378.696466516
46.6666666666667 402076.87313744
47 404739.633886695
47.3333333333333 402822.446147231
47.6666666666667 405378.696466516
48 405804.738186396
48.3333333333333 404207.081736844
48.6666666666667 404633.123456724
49 402928.956577202
49.3333333333333 406017.759046337
49.6666666666667 403674.529586993
50 401224.789697679
50.3333333333333 403994.060876903
50.6666666666667 406550.311196188
51 403994.060876903
51.3333333333333 401970.36270747
51.6666666666667 404207.081736844
52 404207.081736844
52.3333333333333 403674.529586993
52.6666666666667 404313.592166814
53 404846.144316665
53.3333333333333 404739.633886695
53.6666666666667 404952.654746635
54 403248.487867112
54.3333333333333 404846.144316665
54.6666666666667 403674.529586993
55 405591.717326456
55.3333333333333 404739.633886695
55.6666666666667 404952.654746635
56 404420.102596784
56.3333333333333 405378.696466516
56.6666666666667 406230.779906277
57 402822.446147231
57.3333333333333 404633.123456724
57.6666666666667 404846.144316665
58 404846.144316665
58.3333333333333 402928.956577202
58.6666666666667 405272.186036546
59 403568.019157023
59.3333333333333 406443.800766218
59.6666666666667 403781.040016963
60 403674.529586993
60.3333333333333 404952.654746635
60.6666666666667 403994.060876903
61 405272.186036546
61.3333333333333 405059.165176605
61.6666666666667 405165.675606575
62 404100.571306874
62.3333333333333 403781.040016963
62.6666666666667 404633.123456724
63 405272.186036546
63.3333333333333 404739.633886695
63.6666666666667 404420.102596784
64 404526.613026754
64.3333333333333 403035.467007172
64.6666666666667 405911.248616367
65 404526.613026754
65.3333333333333 402396.404427351
65.6666666666667 404952.654746635
66 405378.696466516
66.3333333333333 402822.446147231
66.6666666666667 404313.592166814
67 404207.081736844
67.3333333333333 404633.123456724
67.6666666666667 403141.977437142
68 402928.956577202
68.3333333333333 404952.654746635
68.6666666666667 404526.613026754
69 404952.654746635
69.3333333333333 404420.102596784
69.6666666666667 405059.165176605
70 402928.956577202
70.3333333333333 406230.779906277
70.6666666666667 403887.550446933
71 403141.977437142
71.3333333333333 406443.800766218
71.6666666666667 401757.34184753
72 403674.529586993
72.3333333333333 405378.696466516
72.6666666666667 404633.123456724
73 403887.550446933
73.3333333333333 405272.186036546
73.6666666666667 404633.123456724
74 402928.956577202
74.3333333333333 404100.571306874
74.6666666666667 403887.550446933
75 403141.977437142
75.3333333333333 405059.165176605
75.6666666666667 405591.717326456
76 404100.571306874
76.3333333333333 401331.300127649
76.6666666666667 406337.290336247
77 403461.508727052
77.3333333333333 403141.977437142
77.6666666666667 402289.89399738
78 405485.206896486
78.3333333333333 404739.633886695
78.6666666666667 404846.144316665
79 405378.696466516
79.3333333333333 403248.487867112
79.6666666666667 404313.592166814
80 403781.040016963
80.3333333333333 403674.529586993
80.6666666666667 404952.654746635
81 406124.269476307
81.3333333333333 406550.311196188
81.6666666666667 403781.040016963
82 403887.550446933
82.3333333333333 404846.144316665
82.6666666666667 402928.956577202
83 404207.081736844
83.3333333333333 404100.571306874
83.6666666666667 403674.529586993
84 402822.446147231
84.3333333333333 405378.696466516
84.6666666666667 403248.487867112
85 405698.227756426
85.3333333333333 403994.060876903
85.6666666666667 403141.977437142
86 404846.144316665
86.3333333333333 405804.738186396
86.6666666666667 403994.060876903
87 404526.613026754
87.3333333333333 404313.592166814
87.6666666666667 404420.102596784
88 406230.779906277
88.3333333333333 404846.144316665
88.6666666666667 404207.081736844
89 403568.019157023
89.3333333333333 403674.529586993
89.6666666666667 405059.165176605
90 405378.696466516
90.3333333333333 406124.269476307
90.6666666666667 402928.956577202
91 403354.998297082
91.3333333333333 404526.613026754
91.6666666666667 403461.508727052
92 405698.227756426
92.3333333333333 404207.081736844
92.6666666666667 403887.550446933
93 404952.654746635
93.3333333333333 404952.654746635
93.6666666666667 403994.060876903
94 404846.144316665
94.3333333333333 403035.467007172
94.6666666666667 402396.404427351
95 404100.571306874
95.3333333333333 403994.060876903
95.6666666666667 403248.487867112
96 404207.081736844
96.3333333333333 403035.467007172
96.6666666666667 405059.165176605
97 403035.467007172
97.3333333333333 404313.592166814
97.6666666666667 404526.613026754
98 404100.571306874
98.3333333333333 404633.123456724
98.6666666666667 404739.633886695
99 404526.613026754
99.3333333333333 403781.040016963
99.6666666666667 404313.592166814
100 403354.998297082
100.333333333333 403141.977437142
100.666666666667 403141.977437142
101 404739.633886695
101.333333333333 404420.102596784
101.666666666667 404207.081736844
102 405591.717326456
102.333333333333 401863.8522775
102.666666666667 405591.717326456
103 404207.081736844
103.333333333333 405378.696466516
103.666666666667 403674.529586993
104 406763.332056128
104.333333333333 404739.633886695
104.666666666667 405698.227756426
105 401970.36270747
105.333333333333 404739.633886695
105.666666666667 403674.529586993
106 404100.571306874
106.333333333333 404100.571306874
106.666666666667 404313.592166814
107 404739.633886695
107.333333333333 403887.550446933
107.666666666667 404846.144316665
108 405059.165176605
108.333333333333 404739.633886695
108.666666666667 404420.102596784
109 404100.571306874
109.333333333333 403354.998297082
109.666666666667 404952.654746635
110 402822.446147231
110.333333333333 405059.165176605
110.666666666667 404100.571306874
111 404313.592166814
111.333333333333 406443.800766218
111.666666666667 405272.186036546
112 404633.123456724
112.333333333333 403674.529586993
112.666666666667 406017.759046337
113 405165.675606575
113.333333333333 404739.633886695
113.666666666667 403994.060876903
114 404313.592166814
114.333333333333 404633.123456724
114.666666666667 405059.165176605
115 405591.717326456
115.333333333333 403248.487867112
115.666666666667 404952.654746635
116 403461.508727052
116.333333333333 402928.956577202
116.666666666667 404739.633886695
117 404952.654746635
117.333333333333 403354.998297082
117.666666666667 403674.529586993
118 403994.060876903
118.333333333333 405485.206896486
118.666666666667 402502.914857321
119 404313.592166814
119.333333333333 404207.081736844
119.666666666667 404633.123456724
120 404526.613026754
120.333333333333 403035.467007172
120.666666666667 405485.206896486
121 403887.550446933
121.333333333333 403887.550446933
121.666666666667 404739.633886695
122 404526.613026754
122.333333333333 404313.592166814
122.666666666667 404420.102596784
123 404420.102596784
123.333333333333 406869.842486098
123.666666666667 403674.529586993
124 405911.248616367
124.333333333333 402822.446147231
124.666666666667 403781.040016963
125 404207.081736844
125.333333333333 402502.914857321
125.666666666667 405165.675606575
126 404526.613026754
126.333333333333 405165.675606575
126.666666666667 405698.227756426
127 402822.446147231
127.333333333333 406230.779906277
127.666666666667 403781.040016963
128 403887.550446933
128.333333333333 403354.998297082
128.666666666667 405698.227756426
129 405059.165176605
};
\addlegendentry{\ckptThirty worst}
\addplot [semithick, color3,mark=triangle*, mark size=2.0, mark options={solid,fill=white}, mark repeat=30,mark phase=8]
table {%
0 0
0.333333333333333 172953.6
0.666666666666667 389324.8
1 387891.2
1.33333333333333 386969.6
1.66666666666667 388812.8
2 386867.2
2.33333333333333 387891.2
2.66666666666667 387072
3 388198.4
3.33333333333333 388403.2
3.66666666666667 388096
4 387379.2
4.33333333333333 387686.4
4.66666666666667 387174.4
5 387686.4
5.33333333333333 388403.2
5.66666666666667 389939.2
6 389529.6
6.33333333333333 388300.8
6.66666666666667 389120
7 388812.8
7.33333333333333 387788.8
7.66666666666667 387993.6
8 387379.2
8.33333333333333 389222.4
8.66666666666667 387481.6
9 387481.6
9.33333333333333 389632
9.66666666666667 388812.8
10 0
10.3333333333333 216268.8
10.6666666666667 358195.2
11 360448
11.3333333333333 358400
11.6666666666667 354918.4
12 353280
12.3333333333333 350003.2
12.6666666666667 348364.8
13 348979.2
13.3333333333333 350720
13.6666666666667 350003.2
14 345804.8
14.3333333333333 345292.8
14.6666666666667 346009.6
15 342937.6
15.3333333333333 345907.2
15.6666666666667 344678.4
16 343244.8
16.3333333333333 342425.6
16.6666666666667 342220.8
17 342118.4
17.3333333333333 342425.6
17.6666666666667 340787.2
18 340787.2
18.3333333333333 339865.6
18.6666666666667 340070.4
19 340684.8
19.3333333333333 341811.2
19.6666666666667 340787.2
20 338432
20.3333333333333 340582.4
20.6666666666667 365056
21 387993.6
21.3333333333333 389632
21.6666666666667 388096
22 386662.4
22.3333333333333 387584
22.6666666666667 387891.2
23 387174.4
23.3333333333333 387379.2
23.6666666666667 390451.2
24 388812.8
24.3333333333333 387891.2
24.6666666666667 388915.2
25 387584
25.3333333333333 387891.2
25.6666666666667 387788.8
26 388915.2
26.3333333333333 388198.4
26.6666666666667 387686.4
27 389939.2
27.3333333333333 390144
27.6666666666667 388505.6
28 389734.4
28.3333333333333 390656
28.6666666666667 391065.6
29 390656
29.3333333333333 389734.4
29.6666666666667 389836.8
30 389734.4
30.3333333333333 389017.6
30.6666666666667 389632
31 390246.4
31.3333333333333 389120
31.6666666666667 389222.4
32 390348.8
32.3333333333333 390348.8
32.6666666666667 391987.2
33 390553.6
33.3333333333333 389529.6
33.6666666666667 389632
34 389222.4
34.3333333333333 391577.6
34.6666666666667 389529.6
35 389836.8
35.3333333333333 390041.6
35.6666666666667 390144
36 387891.2
36.3333333333333 388608
36.6666666666667 388710.4
37 387686.4
37.3333333333333 386969.6
37.6666666666667 387891.2
38 389324.8
38.3333333333333 387993.6
38.6666666666667 387379.2
39 386764.8
39.3333333333333 386457.6
39.6666666666667 387686.4
40 386048
40.3333333333333 388096
40.6666666666667 388096
41 388710.4
41.3333333333333 388505.6
41.6666666666667 388710.4
42 388096
42.3333333333333 389836.8
42.6666666666667 387788.8
43 386662.4
43.3333333333333 389120
43.6666666666667 388198.4
44 386457.6
44.3333333333333 388710.4
44.6666666666667 390041.6
45 390656
45.3333333333333 390041.6
45.6666666666667 389632
46 388096
46.3333333333333 389427.2
46.6666666666667 388300.8
47 387481.6
47.3333333333333 388608
47.6666666666667 390144
48 388915.2
48.3333333333333 388608
48.6666666666667 387891.2
49 388198.4
49.3333333333333 388608
49.6666666666667 387993.6
50 389120
50.3333333333333 388403.2
50.6666666666667 389939.2
51 387891.2
51.3333333333333 388300.8
51.6666666666667 390860.8
52 389017.6
52.3333333333333 388505.6
52.6666666666667 386662.4
53 389734.4
53.3333333333333 388198.4
53.6666666666667 389529.6
54 389222.4
54.3333333333333 386355.2
54.6666666666667 388608
55 389017.6
55.3333333333333 388915.2
55.6666666666667 388198.4
56 388300.8
56.3333333333333 388608
56.6666666666667 387481.6
57 387891.2
57.3333333333333 389222.4
57.6666666666667 388403.2
58 387686.4
58.3333333333333 389529.6
58.6666666666667 388403.2
59 389222.4
59.3333333333333 389017.6
59.6666666666667 388710.4
60 388403.2
60.3333333333333 388096
60.6666666666667 388710.4
61 389836.8
61.3333333333333 390553.6
61.6666666666667 388812.8
62 389324.8
62.3333333333333 389017.6
62.6666666666667 388403.2
63 388812.8
63.3333333333333 388915.2
63.6666666666667 387584
64 388198.4
64.3333333333333 389222.4
64.6666666666667 387788.8
65 388403.2
65.3333333333333 387891.2
65.6666666666667 389017.6
66 389017.6
66.3333333333333 389632
66.6666666666667 388403.2
67 388198.4
67.3333333333333 388608
67.6666666666667 389120
68 388608
68.3333333333333 388096
68.6666666666667 387276.8
69 387788.8
69.3333333333333 388608
69.6666666666667 388812.8
70 388812.8
70.3333333333333 389734.4
70.6666666666667 389632
71 388812.8
71.3333333333333 389120
71.6666666666667 389017.6
72 388403.2
72.3333333333333 388198.4
72.6666666666667 388505.6
73 389427.2
73.3333333333333 389120
73.6666666666667 389632
74 387891.2
74.3333333333333 390656
74.6666666666667 388403.2
75 387686.4
75.3333333333333 387584
75.6666666666667 389632
76 389120
76.3333333333333 388403.2
76.6666666666667 387686.4
77 389120
77.3333333333333 388608
77.6666666666667 390348.8
78 389222.4
78.3333333333333 388812.8
78.6666666666667 390144
79 388300.8
79.3333333333333 389017.6
79.6666666666667 388300.8
80 388300.8
80.3333333333333 390348.8
80.6666666666667 387891.2
81 388915.2
81.3333333333333 387481.6
81.6666666666667 388608
82 388812.8
82.3333333333333 388198.4
82.6666666666667 388403.2
83 389324.8
83.3333333333333 388505.6
83.6666666666667 386969.6
84 388608
84.3333333333333 389017.6
84.6666666666667 389222.4
85 387788.8
85.3333333333333 388812.8
85.6666666666667 390246.4
86 389427.2
86.3333333333333 388505.6
86.6666666666667 387481.6
87 387276.8
87.3333333333333 388710.4
87.6666666666667 387072
88 388403.2
88.3333333333333 388608
88.6666666666667 387788.8
89 388403.2
89.3333333333333 389222.4
89.6666666666667 388300.8
90 389529.6
90.3333333333333 390758.4
90.6666666666667 388710.4
91 388608
91.3333333333333 389017.6
91.6666666666667 387276.8
92 386867.2
92.3333333333333 388403.2
92.6666666666667 388096
93 387993.6
93.3333333333333 388608
93.6666666666667 388198.4
94 388915.2
94.3333333333333 389120
94.6666666666667 390553.6
95 389324.8
95.3333333333333 388608
95.6666666666667 389529.6
96 388915.2
96.3333333333333 389939.2
96.6666666666667 389324.8
97 389427.2
97.3333333333333 389120
97.6666666666667 389324.8
98 389939.2
98.3333333333333 389632
98.6666666666667 388096
99 388608
99.3333333333333 388096
99.6666666666667 388300.8
100 390246.4
100.333333333333 390758.4
100.666666666667 388198.4
101 386560
101.333333333333 389529.6
101.666666666667 389324.8
102 389120
102.333333333333 387686.4
102.666666666667 388710.4
103 390246.4
103.333333333333 389632
103.666666666667 389120
104 389120
104.333333333333 387993.6
104.666666666667 389120
105 389632
105.333333333333 388812.8
105.666666666667 390758.4
106 388608
106.333333333333 390553.6
106.666666666667 388403.2
107 389427.2
107.333333333333 386662.4
107.666666666667 387891.2
108 388403.2
108.333333333333 388505.6
108.666666666667 390656
109 386048
109.333333333333 388198.4
109.666666666667 390144
110 389836.8
110.333333333333 389734.4
110.666666666667 389427.2
111 387072
111.333333333333 388198.4
111.666666666667 389324.8
112 387993.6
112.333333333333 389222.4
112.666666666667 390451.2
113 387686.4
113.333333333333 389222.4
113.666666666667 388608
114 388403.2
114.333333333333 388812.8
114.666666666667 388812.8
115 389427.2
115.333333333333 388403.2
115.666666666667 388300.8
116 19353.6
};
\addlegendentry{\sysKTwo}
\addplot [semithick, color4,mark=diamond*, mark size=2.0, mark options={solid,fill=white}, mark repeat=30,mark phase=15]
table {%
0 386560
0.333333333333333 388915.2
0.666666666666667 388608
1 392499.2
1.33333333333333 388608
1.66666666666667 389324.8
2 389222.4
2.33333333333333 386150.4
2.66666666666667 387788.8
3 391372.8
3.33333333333333 391372.8
3.66666666666667 391987.2
4 393728
4.33333333333333 389632
4.66666666666667 392499.2
5 388608
5.33333333333333 388915.2
5.66666666666667 389120
6 387584
6.33333333333333 386252.8
6.66666666666667 387788.8
7 387993.6
7.33333333333333 387481.6
7.66666666666667 390758.4
8 390758.4
8.33333333333333 389017.6
8.66666666666667 390041.6
9 386560
9.33333333333333 386662.4
9.66666666666667 389324.8
10 0
10.3333333333333 282419.2
10.6666666666667 369152
11 359526.4
11.3333333333333 357683.2
11.6666666666667 354304
12 348876.8
12.3333333333333 347340.8
12.6666666666667 347955.2
13 353075.2
13.3333333333333 351027.2
13.6666666666667 346112
14 343961.6
14.3333333333333 342220.8
14.6666666666667 343449.6
15 344064
15.3333333333333 341913.6
15.6666666666667 340787.2
16 346009.6
16.3333333333333 343859.2
16.6666666666667 342016
17 342016
17.3333333333333 342835.2
17.6666666666667 338636.8
18 337612.8
18.3333333333333 341708.8
18.6666666666667 337715.2
19 336896
19.3333333333333 342323.2
19.6666666666667 342323.2
20 341606.4
20.3333333333333 342732.8
20.6666666666667 343142.4
21 335769.6
21.3333333333333 335360
21.6666666666667 335155.2
22 339763.2
22.3333333333333 339251.2
22.6666666666667 347852.8
23 343142.4
23.3333333333333 343244.8
23.6666666666667 346009.6
24 345907.2
24.3333333333333 342425.6
24.6666666666667 341913.6
25 342220.8
25.3333333333333 339251.2
25.6666666666667 338944
26 338534.4
26.3333333333333 339865.6
26.6666666666667 338227.2
27 338329.6
27.3333333333333 338329.6
27.6666666666667 336588.8
28 340377.6
28.3333333333333 339046.4
28.6666666666667 340787.2
29 365260.8
29.3333333333333 389017.6
29.6666666666667 387276.8
30 391884.8
30.3333333333333 391884.8
30.6666666666667 393011.2
31 388608
31.3333333333333 388710.4
31.6666666666667 387686.4
32 387379.2
32.3333333333333 389324.8
32.6666666666667 391372.8
33 392089.6
33.3333333333333 392089.6
33.6666666666667 392908.8
34 390553.6
34.3333333333333 390553.6
34.6666666666667 388300.8
35 388915.2
35.3333333333333 388608
35.6666666666667 392499.2
36 388608
36.3333333333333 389324.8
36.6666666666667 389222.4
37 386150.4
37.3333333333333 387481.6
37.6666666666667 389632
38 389632
38.3333333333333 386969.6
38.6666666666667 389120
39 387993.6
39.3333333333333 388915.2
39.6666666666667 388096
40 387993.6
40.3333333333333 388710.4
40.6666666666667 389734.4
41 388403.2
41.3333333333333 388608
41.6666666666667 389120
42 387891.2
42.3333333333333 389427.2
42.6666666666667 389324.8
43 390451.2
43.3333333333333 389427.2
43.6666666666667 389222.4
44 388710.4
44.3333333333333 389427.2
44.6666666666667 388096
45 389120
45.3333333333333 388710.4
45.6666666666667 388403.2
46 388812.8
46.3333333333333 388915.2
46.6666666666667 389836.8
47 389324.8
47.3333333333333 389632
47.6666666666667 389427.2
48 389529.6
48.3333333333333 387072
48.6666666666667 388915.2
49 389120
49.3333333333333 389734.4
49.6666666666667 388300.8
50 390451.2
50.3333333333333 390451.2
50.6666666666667 388915.2
51 389939.2
51.3333333333333 388505.6
51.6666666666667 387481.6
52 388300.8
52.3333333333333 389017.6
52.6666666666667 388403.2
53 389836.8
53.3333333333333 389836.8
53.6666666666667 390553.6
54 387993.6
54.3333333333333 388812.8
54.6666666666667 389222.4
55 389529.6
55.3333333333333 388915.2
55.6666666666667 389324.8
56 389427.2
56.3333333333333 388915.2
56.6666666666667 388608
57 389427.2
57.3333333333333 387072
57.6666666666667 387993.6
58 389222.4
58.3333333333333 389324.8
58.6666666666667 388198.4
59 388403.2
59.3333333333333 388812.8
59.6666666666667 389836.8
60 388300.8
60.3333333333333 389222.4
60.6666666666667 388505.6
61 388812.8
61.3333333333333 390451.2
61.6666666666667 390758.4
62 388608
62.3333333333333 387788.8
62.6666666666667 388915.2
63 389324.8
63.3333333333333 388505.6
63.6666666666667 388505.6
64 387481.6
64.3333333333333 390656
64.6666666666667 387379.2
65 389222.4
65.3333333333333 388608
65.6666666666667 388608
66 389222.4
66.3333333333333 388710.4
66.6666666666667 387788.8
67 388915.2
67.3333333333333 388608
67.6666666666667 388812.8
68 387584
68.3333333333333 389427.2
68.6666666666667 388300.8
69 389734.4
69.3333333333333 388915.2
69.6666666666667 387993.6
70 386662.4
70.3333333333333 388505.6
70.6666666666667 387788.8
71 388710.4
71.3333333333333 387686.4
71.6666666666667 389734.4
72 388198.4
72.3333333333333 389632
72.6666666666667 389324.8
73 386867.2
73.3333333333333 386764.8
73.6666666666667 388300.8
74 387686.4
74.3333333333333 387993.6
74.6666666666667 389632
75 389120
75.3333333333333 389734.4
75.6666666666667 388403.2
76 388710.4
76.3333333333333 388403.2
76.6666666666667 388505.6
77 388505.6
77.3333333333333 388710.4
77.6666666666667 389734.4
78 388915.2
78.3333333333333 388505.6
78.6666666666667 386764.8
79 390041.6
79.3333333333333 388608
79.6666666666667 387891.2
80 389836.8
80.3333333333333 389939.2
80.6666666666667 389222.4
81 389222.4
81.3333333333333 389529.6
81.6666666666667 387174.4
82 386867.2
82.3333333333333 388300.8
82.6666666666667 388915.2
83 388505.6
83.3333333333333 389734.4
83.6666666666667 388403.2
84 390553.6
84.3333333333333 388608
84.6666666666667 387686.4
85 386969.6
85.3333333333333 389120
85.6666666666667 388505.6
86 388812.8
86.3333333333333 388710.4
86.6666666666667 388710.4
87 388403.2
87.3333333333333 388096
87.6666666666667 388915.2
88 388403.2
88.3333333333333 387481.6
88.6666666666667 388505.6
89 388505.6
89.3333333333333 389427.2
89.6666666666667 387686.4
90 387481.6
90.3333333333333 388505.6
90.6666666666667 388300.8
91 389222.4
91.3333333333333 387584
91.6666666666667 389324.8
92 388505.6
92.3333333333333 388505.6
92.6666666666667 388608
93 388300.8
93.3333333333333 388096
93.6666666666667 390553.6
94 388505.6
94.3333333333333 388198.4
94.6666666666667 388403.2
95 387993.6
95.3333333333333 388300.8
95.6666666666667 389120
96 389017.6
96.3333333333333 388096
96.6666666666667 389120
97 387686.4
97.3333333333333 387788.8
97.6666666666667 388710.4
98 387993.6
98.3333333333333 388198.4
98.6666666666667 389836.8
99 389529.6
99.3333333333333 388915.2
99.6666666666667 389734.4
100 390553.6
100.333333333333 387788.8
100.666666666667 389324.8
101 389939.2
101.333333333333 389120
101.666666666667 389529.6
102 388608
102.333333333333 389324.8
102.666666666667 389017.6
103 389120
103.333333333333 386764.8
103.666666666667 387584
};
\addlegendentry{\sysKFour}
